A mathematical framework to study organising principles in graphical representations of biochemical processes

The complexity of molecular and cellular processes forces experimental studies to focus on subsystems. To study the functioning of biological systems across levels of structural and functional organisation, we require tools to compose and organise networks with different levels of detail and abstraction. Systems Biology Graphical Notation (SBGN) is a standardised notational system that visualises biochemical processes as networks. Despite their widespread adoption, SBGN languages remain purely visual and lack an underlying mathematical framework, limiting their compositional analysis, abstraction, and integration with formal modelling approaches. SBGN comprises three complementary visual languages-Process Description (SBGN-PD), Activity Flow (SBGN-AF), and Entity Relationship (SBGN-ER)-each operating at a different level of abstraction. In this manuscript, we introduce a category-theoretic formalism for SBGN-PD, a visual language to describe biochemical processes as biochemical reaction networks. Using the theory of structured cospans, we construct a symmetric monoidal double category whose horizontal 1-morphisms correspond to SBGN-PD diagrams. We also analyse how a designated subnetwork influences the surrounding network and how external entities, in turn, affect the internal reactions of the subnetwork. Our work addresses a key gap between biological visualisation and mathematical structure. It provides precise organising principles for SBGN-PD, including compositionality, enabling the construction of large biochemical reaction networks from smaller ones, and zooming out, allowing the abstraction of detailed biochemical mechanisms while preserving their functional interfaces. Throughout the paper, the proposed framework is illustrated using standard SBGN-PD examples, demonstrating its applicability to large-scale biochemical reaction networks.

==> tikzlibrarysbgn.code.tex <==
%Copyright 2018 by Adrien Rougny
%This file may be distributed and/or modified under the terms of the GNU General Public License version 3
%See the file LICENSE.txt
\usetikzlibrary{arrows.meta, shapes, fit, backgrounds, intersections, fpu}

%include macros
\input{tikzlibrarysbgn.macros.tex}

%include shapes
\input{tikzlibrarysbgn.shapes.tex}
% %processes
% \input{genericprocess.tex}
% \input{uncertainprocess.tex}
% \input{association.tex}
% \input{dissociation.tex}
% \input{omittedprocess.tex}
%
% %epns
% \input{unspecifiedentity.tex}
% \input{emptyset.tex}
% \input{simplechemical.tex}
% \input{simplechemicalmultimer.tex}
% \input{complex.tex}
% \input{complexmultimer.tex}
% \input{macromolecule.tex}
% \input{macromoleculemultimer.tex}
% \input{nucleicacidfeature.tex}
% \input{nucleicacidfeaturemultimer.tex}
%
% %special svs
% \input{svexistence.tex}
% \input{svlocation.tex}
% \input{sv.tex}
%
% %los
% \input{and.tex}
% \input{or.tex}
% \input{not.tex}
% \input{delay.tex}
% \input{equivalence.tex}
%
% %tag
% \input{tag.tex}

%styles
\tikzset{sbgn/.style={execute at begin picture={
    \pgfdeclarelayer{background}
    \pgfdeclarelayer{compartments}
    \pgfdeclarelayer{nodes}
    \pgfdeclarelayer{arcs}
    \pgfdeclarelayer{subcomplexes}
    \pgfdeclarelayer{subunits}
    \pgfdeclarelayer{attributes}
    \pgfsetlayers{background,compartments,nodes,arcs,main,subcomplexes,subunits,attributes}},
    font=\huge\sffamily,
    node distance = 2cm}
}

\tikzset{macromolecule/.style={draw = black, fill = white, shape = macromolecule, minimum height = 60pt, minimum width = 108pt, line width = 1pt, inner xsep = 6pt, inner ysep = 6pt, node layer = nodes}}
\tikzset{macromolecule subunit/.style={draw = black, fill = white, shape = macromolecule, minimum height = 60pt, minimum width = 108pt, line width = 1pt, inner xsep = 6pt, inner ysep = 6pt, node layer = subunits}}
\tikzset{macromolecule multimer/.style={draw = black, fill = white, shape = macromoleculemultimer, minimum height = 60pt, minimum width = 108pt, line width = 1pt, inner xsep = 6pt, inner ysep = 6pt, node layer = nodes}}
\tikzset{macromolecule multimer subunit/.style={draw = black, fill = white, shape = macromoleculemultimer, minimum height = 60pt, minimum width = 108pt, line width = 1pt, inner xsep = 6pt, inner ysep = 6pt, node layer = subunits}}
\tikzset{unspecified entity/.style={draw = black, fill = white, shape = unspecifiedentity, minimum height = 60pt, minimum width = 108pt, line width = 1pt, inner xsep = 6pt, inner ysep = 6pt, node layer = nodes}}
\tikzset{unspecified entity subunit/.style={draw = black, fill = white, shape = unspecifiedentity, minimum height = 60pt, minimum width = 108pt, line width = 1pt, inner xsep = 6pt, inner ysep = 6pt, node layer = subunits}}
\tikzset{nucleic acid feature/.style={draw = black, fill = white, shape = nucleicacidfeature, minimum height = 60pt, minimum width = 108pt, line width = 1pt, inner xsep = 6pt, inner ysep = 6pt, node layer = nodes}}
\tikzset{nucleic acid feature subunit/.style={draw = black, fill = white, shape = nucleicacidfeature, minimum height = 60pt, minimum width = 108pt, line width = 1pt, inner xsep = 6pt, inner ysep = 6pt, node layer = subunits}}
\tikzset{nucleic acid feature multimer/.style={draw = black, fill = white, shape = nucleicacidfeaturemultimer, minimum height = 60pt, minimum width = 108pt, line width = 1pt, inner xsep = 6pt, inner ysep = 6pt, node layer = nodes}}
\tikzset{nucleic acid feature multimer subunit/.style={draw = black, fill = white, shape = nucleicacidfeaturemultimer, minimum height = 60pt, minimum width = 108pt, line width = 1pt, inner xsep = 6pt, inner ysep = 6pt, node layer = subunits}}
\tikzset{perturbation/.style={draw = black, fill = white, shape = signal, signal to = nowhere, signal from = east and west, signal pointer angle = 110, minimum height = 60pt, minimum width = 108pt, line width = 1pt, inner xsep = 6pt, inner ysep = 6pt, node layer = nodes}}
\tikzset{simple chemical/.style={draw = black, fill = white, shape = simplechemical, minimum height = 60pt, minimum width = 60pt, line width = 1pt, inner xsep = 6pt, inner ysep = 6pt, node layer = nodes}}
\tikzset{simple chemical subunit/.style={draw = black, fill = white, shape = simplechemical, minimum height = 60pt, minimum width = 60pt, line width = 1pt, inner xsep = 6pt, inner ysep = 6pt, node layer = subunits}}
\tikzset{simple chemical multimer/.style={draw = black, fill = white, shape = simplechemicalmultimer, minimum height = 60pt, minimum width = 60pt, line width = 1pt, inner xsep = 6pt, inner ysep = 6pt, node layer = nodes}}
\tikzset{simple chemical multimer subunit/.style={draw = black, fill = white, shape = simplechemicalmultimer, minimum height = 60pt, minimum width = 60pt, line width = 1pt, inner xsep = 6pt, inner ysep = 6pt, node layer = subunits}}
\tikzset{complex/.style={draw = black, shape = complex, fill = white, minimum height = 60pt, minimum width = 108pt, line width = 1pt, inner xsep = 6pt, inner ysep = 6pt, node layer = nodes}}
\tikzset{complex subunit/.style={draw = black, fill = white, shape = complex, minimum height = 60pt, minimum width = 108pt, line width = 1pt, inner xsep = 6pt, inner ysep = 6pt, node layer = subcomplexes}}
\tikzset{complex multimer/.style={draw = black, fill = white, shape = complexmultimer, minimum height = 60pt, minimum width = 108pt, line width = 1pt, inner xsep = 6pt, inner ysep = 6pt, node layer = nodes}}
\tikzset{complex multimer subunit/.style={draw = black, fill = white, shape = complexmultimer, minimum height = 60pt, minimum width = 108pt, line width = 1pt, inner xsep = 6pt, inner ysep = 6pt, node layer = nodes}}
\tikzset{empty set/.style={draw = black, fill = white, shape = emptyset, minimum height = 60pt, minimum width = 60pt, line width = 1pt, node layer = subunits}}
\tikzset{biological activity/.style={draw = black, fill = white, shape = rectangle, minimum height = 60pt, minimum width = 108pt, line width = 1pt, inner xsep = 6pt, inner ysep = 6pt, node layer = nodes}}
\tikzset{entity/.style={draw = black, fill = white, shape = macromolecule, minimum height = 60pt, minimum width = 108pt, line width = 1pt, inner xsep = 6pt, inner ysep = 6pt, node layer = nodes}}
\tikzset{outcome/.style={draw = black, fill = black, shape = circle, inner xsep = 0pt, inner ysep = 0pt, minimum height = 12pt, minimum width = 12pt, node layer = attributes}}
\tikzset{sv/.style={draw = black, fill = white, shape = sv, minimum height = 22pt, inner xsep = 6pt, inner ysep = 6pt, line width = 1pt, font = {\large\sffamily}, node layer = attributes}}
\tikzset{value/.style={draw = black, fill = white, shape = sv, minimum height = 22pt, inner xsep = 2pt, inner ysep = 2pt, line width = 1pt, inner xsep = 6pt, inner ysep = 6pt, font = {\normalsize\sffamily}, node layer = attributes}}
\tikzset{sv existence/.style={draw = black, fill = white, shape = svexistence, minimum width = 22pt, minimum height = 22pt, line width = 1pt, node layer = attributes}}
\tikzset{sv location/.style={draw = black, fill = white, shape = svlocation, minimum width = 22pt, minimum height = 22pt, line width = 1pt, node layer = attributes}}
\tikzset{ui/.style={draw = black, fill = white, shape = rectangle, line width = 1pt, inner xsep = 6pt, inner ysep = 6pt, font = {\large\sffamily}, node layer = attributes}}
\tikzset{ui macromolecule/.style={draw = black, shape = macromolecule, fill = white, line width = 1pt, inner xsep = 6pt, inner ysep = 6pt, minimum width = 30pt, minimum height = 20pt, font = {\normalsize\sffamily}, node layer = attributes}}
\tikzset{ui complex/.style={draw = black, shape = complex, fill = white, line width = 1pt, inner xsep = 6pt, inner ysep = 6pt, minimum width = 30pt, minimum height = 20pt, font = {\normalsize\sffamily}, node layer = attributes}}
\tikzset{ui perturbation/.style={draw = black, shape = signal, signal to = nowhere, signal from = east and west, signal pointer angle = 110, fill = white, line width = 1pt, inner xsep = 6pt, inner ysep = 6pt, minimum width = 30pt, minimum height = 20pt, font = {\normalsize\sffamily}, node layer = attributes}}
\tikzset{ui simple chemical/.style={draw = black, shape = simplechemical, fill = white, line width = 1pt, inner xsep = 6pt, inner ysep = 6pt, minimum width = 30pt, minimum height = 20pt, font = {\normalsize\sffamily}, node layer = attributes}}
\tikzset{ui nucleic acid feature/.style={draw = black, shape = nucleicacidfeature, fill = white, line width = 1pt, inner xsep = 6pt, inner ysep = 6pt, minimum width = 30pt, minimum height = 20pt, font = {\normalsize\sffamily}, node layer = attributes}}
\tikzset{ui unspecified entity/.style={draw = black, shape = unspecifiedentity, fill = white, line width = 1pt, inner xsep = 6pt, inner ysep = 6pt, minimum width = 30pt, minimum height = 20pt, font = {\normalsize\sffamily}, node layer = attributes}}
\tikzset{compartment/.style={draw = black, line width = 6pt, fill = white}, compartment/.append code={
    \pgfkeysgetvalue{/tikz/isnode}{\isnode}
    \ifx\isnode\true
        \pgfkeys{/tikz/node layer=compartments}
    \else
        \pgfkeys{/tikz/draw layer=compartments}
    \fi}
}
\tikzset{submap/.style={draw = black, fill = white, shape = rectangle, minimum height = 60pt, minimum width = 108pt, line width = 1pt, inner xsep = 6pt, inner ysep = 6pt, outer xsep = 0pt, outer ysep = 0pt, node layer = nodes}}
\tikzset{tag/.style={draw = black, fill = white, shape = tag, minimum height = 40pt, minimum width = 60pt, line width = 1pt, inner xsep = 6pt, inner ysep = 6pt, node layer = nodes}}
\tikzset{and/.style={draw = black, fill = white, shape = and, minimum height = 42pt, minimum width = 42pt, line width = 1pt, node layer = nodes}}
\tikzset{or/.style={draw = black, fill = white, shape = or, minimum height = 42pt, minimum width = 42pt, line width = 1pt, node layer = nodes}}
\tikzset{not/.style={draw = black, fill = white, shape = not, minimum height = 42pt, minimum width = 42pt, line width = 1pt, node layer = nodes}}
\tikzset{delay/.style={draw = black, fill = white, shape = delay, minimum height = 42pt, minimum width = 42pt, line width = 1pt, node layer = nodes}}
\tikzset{equivalence/.style={draw = black, fill = white, shape = equivalence, minimum height = 42pt, minimum width = 42pt, line width = 1pt, node layer = nodes}}
\tikzset{generic process/.style={draw = black, fill = white, shape = genericprocess, minimum height = 26pt, minimum width = 26pt, line width = 1pt, node layer = nodes}}
\tikzset{omitted process/.style={draw = black, fill = white, shape = omittedprocess, minimum height = 26pt, minimum width = 26pt, line width = 1pt, node layer = nodes}}
\tikzset{uncertain process/.style={draw = black, fill = white, shape = uncertainprocess, minimum height = 26pt, minimum width = 26pt, line width = 1pt, node layer = nodes}}
\tikzset{association/.style={draw = black, fill = black, shape = association, minimum height = 26pt, minimum width = 26pt, line width = 1pt, node layer = nodes}}
\tikzset{dissociation/.style={draw = black, fill = white, shape = dissociation, minimum height = 26pt, minimum width = 26pt, line width = 1pt, node layer = nodes}}
\tikzset{phenotype/.style={draw = black, fill = white, shape = signal, signal to = east and west, signal pointer angle = 110, minimum height = 60pt, minimum width = 108pt, line width = 1pt, inner xsep = 6pt, inner ysep = 6pt, node layer = nodes}}
\tikzset{logic arc/.style={line width = 1pt, draw layer = arcs}}
\tikzset{equivalence arc/.style={line width = 1pt, draw layer = arcs}}
\tikzset{consumption/.style={line width = 1pt, draw layer = arcs}}
\tikzset{production/.style={line width = 1pt, -{Triangle[length=16pt, width=16pt]}, draw layer = arcs}}
\tikzset{reversible/.style={line width = 1pt, {Triangle[length=16pt, width=16pt]}-, draw layer = arcs}}
\tikzset{modulation/.style={line width = 1pt, -{Diamond[fill=#1, length=16pt, width=16pt]}, draw layer = arcs}, modulation/.default=white}
\tikzset{stimulation/.style={line width = 1pt, -{Triangle[fill=#1, length=16pt, width=16pt]}, draw layer = arcs}, stimulation/.default=white}
\tikzset{catalysis/.style={line width = 1pt, -{Circle[fill=#1, length = 12pt, width=12pt]}, draw layer = arcs}, catalysis/.default=white}
\tikzset{inhibition/.style={line width = 1pt, -{Bar[width = 16pt]}, draw layer = arcs, shorten >= 0.05cm}}
\tikzset{absolute inhibition/.style={line width = 1pt, -{Bar[sep=1, width = 16pt] Bar[width = 16pt]}, draw layer = arcs, shorten >= 0.05cm}}
\tikzset{necessary stimulation/.style={line width = 1pt, -{Bar[width = 16pt, sep=2] Triangle[fill=#1, length=16pt, width=16pt]}, draw layer = arcs}, necessary stimulation/.default=white}
\tikzset{absolute stimulation/.style={line width = 1pt, -{Triangle[fill=#1, length=16pt, width=16pt, sep=-3] Triangle[fill=#1, length=16pt, width=16pt]}, draw layer = arcs}, absolute stimulation/.default=white}
\tikzset{assignment/.style={line width = 1pt, -{Stealth[length=16pt, width=12pt]}, draw layer = arcs}}
\tikzset{interaction/.style={line width = 1pt, {Stealth[length=16pt, width=12pt]}-{Stealth[length=16pt, width=12pt]}, draw layer = arcs}}
\tikzset{nary/.style={draw = black, fill = white, shape = circle, minimum height = 42pt, minimum width = 42pt, line width = 1pt, node layer = attributes}}
\tikzset{anchor point/.style={shape = circle, inner xsep = 0pt, inner ysep = 0pt, outer xsep = 0pt, outer ysep = 0pt, node layer = nodes}}
\tikzset{implicit xor/.style={draw = black, shape = circle, inner xsep = 0pt, inner ysep = 0pt, minimum width = 1pt, minimum height = 1pt, node layer = nodes}}
\tikzset{annotation/.style={draw = black, fill = white, shape = rectangle callout, line width = 1pt, minimum height = 50pt, inner xsep = 6pt, inner ysep = 6pt, node layer = nodes}}

% \tikzset{macromolecule/.style={draw = black, fill = white, shape = macromolecule, minimum height = 60pt, minimum width = 108pt, line width = 1pt, node layer = nodes}}


==> tikzlibrarysbgn.macros.tex <==
%Copyright 2018 by Adrien Rougny
%This file may be distributed and/or modified under the terms of the GNU General Public License version 3
%See the file LICENSE.txt
\def\true{true}
\def\false{false}
\def\vertical{vertical}
\def\horizontal{horizontal}
\def\oup{up}
\def\odown{down}
\def\oright{right}
\def\oleft{left}

\def\pointborderrectanglecorners#1#2#3{%point, southwest, northeast
    \pgf@process{#2}
    \pgf@xa = \pgf@x
    \pgf@ya = \pgf@y
    \pgf@process{#3}
    \pgf@xb = \pgf@x
    \pgf@yb = \pgf@y
    \pgf@xc = 0.5\pgf@xa
    \advance\pgf@xc by 0.5\pgf@xb
    \pgf@yc = 0.5\pgf@ya
    \advance\pgf@yc by 0.5\pgf@yb
    \advance\pgf@xb by -\pgf@xc
    \advance\pgf@yb by -\pgf@yc
    \pgf@process{#1}
    \pgf@xa = \pgf@x
    \pgf@ya = \pgf@y
    \advance\pgf@xa by -\pgf@xc
    \advance\pgf@ya by -\pgf@yc
    \edef\pgf@marshal{
        \noexpand\pgfpointborderrectangle{\noexpand\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}{\noexpand\pgfpoint{\the\pgf@xb}{\the\pgf@yb}}
    }
    \pgf@process{\pgf@marshal}
    \advance\pgf@x by \pgf@xc
    \advance\pgf@y by \pgf@yc
}

\def\pointbordercircle#1#2#3{%point, center, radius
    \pgf@process{#2}
    \pgf@xc = \pgf@x
    \pgf@yc = \pgf@y
    \pgf@process{#1}
    \pgf@xa = \pgf@x
    \pgf@ya = \pgf@y
    \pgf@xb = #3
    \pgf@yb = #3
    \edef\pgf@marshal{%
        \noexpand\pgfpointborderellipse
        {\noexpand\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}
        {\noexpand\pgfpoint{\the\pgf@xb}{\the\pgf@yb}}%
    }
    \pgf@process{\pgf@marshal}
    \advance\pgf@x by \pgf@xc
    \advance\pgf@y by \pgf@yc
}

\def\circlefindx#1#2#3#4{%center, radius, y, sol
    \pgf@process{#1}
    \@tempdima=\pgf@x
    \@tempdimb=\pgf@y
    \pgf@xb=#2
    \pgf@y=#3
    \advance\pgf@y by -\@tempdimb
    \pgfmathsetlength{\pgf@x}{sqrt(\pgf@xb^2-\pgf@y^2)}
    \ifnum #4=1
        \pgf@x=-\pgf@x
    \fi
    \advance\pgf@x by \@tempdima
}

\def\circlefindangle#1#2#3#4{%center, radius, y, sol
    \pgf@process{#1}
    \@tempdima=\pgf@x
    \@tempdimb=\pgf@y
    \pgf@xb=#2
    \pgf@y=#3
    \advance\pgf@y by -\@tempdimb
    \pgfmathsetlength{\pgf@x}{sqrt(\pgf@xb^2-\pgf@y^2)}
    \ifnum #4=1
        \pgf@x=-\pgf@x
    \fi
    % \pgfmathsetlength{\pgf@x}{atan2(\pgf@y,\pgf@x)}
    \pgfmathsetlength{\pgf@x}{atan2(\pgf@y,\pgf@x)}
}

\def\belongstocone#1#2#3#4{%center, point1, point2, point
    % \global\if@tempswa
    \pgf@process{#1}
    \pgf@xc=\pgf@x
    \pgf@yc=\pgf@y
    \pgf@process{#2}
    \advance\pgf@x by -\pgf@xc
    \advance\pgf@y by -\pgf@yc
    \ifdim\pgf@y=0pt
        \ifdim\pgf@x>0pt
            \pgf@xa=0pt
        \else
            \pgf@xa=180pt
        \fi
    \else
        \pgfmathsetlength{\pgf@xa}{atan2(\pgf@y,\pgf@x)}
    \fi
    % \ifdim\pgf@xa<0pt
    %     \advance\pgf@xa by 360pt
    % \fi
    \pgf@process{#3}
    \advance\pgf@x by -\pgf@xc
    \advance\pgf@y by -\pgf@yc
    \ifdim\pgf@y=0pt
        \ifdim\pgf@x>0pt
            \pgf@xb=0pt
        \else
            \pgf@xb=180pt
        \fi
    \else
        \pgfmathsetlength{\pgf@xb}{atan2(\pgf@y,\pgf@x)}
    \fi
    % \ifdim\pgf@xb<0pt
    %     \advance\pgf@xb by 360pt
    % \fi
    \pgf@process{#4}
    \advance\pgf@x by -\pgf@xc
    \advance\pgf@y by -\pgf@yc
    \ifdim\pgf@y=0pt
        \ifdim\pgf@x>0pt
            \pgf@ya=0pt
        \else
            \pgf@ya=180pt
        \fi
    \else
        \pgfmathsetlength{\pgf@ya}{atan2(\pgf@y,\pgf@x)}
    \fi
    % \ifdim\pgf@ya<0pt
    %     \advance\pgf@ya by 360pt
    % \fi
    \ifdim\pgf@xa<0pt
        \advance\pgf@xa by 360pt
        \ifdim\pgf@xb<0pt
            \advance\pgf@xb by 360pt
        \fi
        \ifdim\pgf@ya<0pt
            \advance\pgf@ya by 360pt
        \fi
    \fi
    \ifdim\pgf@ya>\pgf@xa
        \global\@tempswafalse
    \else
        \ifdim\pgf@ya<\pgf@xb
            \global\@tempswafalse
        \else
            \global\@tempswatrue
        \fi
    \fi
}

\def\intersectionlinecircle#1#2#3#4#5{% point1, point2, center, radius, solution
    \pgf@process{#1}
    \pgf@xa = \pgf@x
    \pgf@ya = \pgf@y
    \pgf@process{#2}
    \pgf@xb = \pgf@x
    \pgf@yb = \pgf@y
    \pgf@process{#3}
    \pgf@xc = \pgf@x
    \pgf@yc = \pgf@y
    \newdimen\rad
    \rad = #4
    \c@pgf@counta=#5
    \advance\pgf@xa by -\pgf@xc
    \advance\pgf@xb by -\pgf@xc
    \advance\pgf@ya by -\pgf@yc
    \advance\pgf@yb by -\pgf@yc
    \ifdim\pgf@xa=\pgf@xb % infinite slope set to max dimen
        \ifnum\c@pgf@counta=1
            \pgfmathsetlength{\pgf@y}{-sqrt(\rad^2-\pgf@xa^2)}
        \else
            \pgfmathsetlength{\pgf@y}{sqrt(\rad^2-\pgf@xa^2)}
        \fi
        \pgf@x=\pgf@xa
    \else
        \pgfmathsetlength{\@tempdima}{(\pgf@yb-\pgf@ya)/(\pgf@xb-\pgf@xa)}
        \pgfmathsetlength{\@tempdimb}{\pgf@yb-\pgf@xb*\@tempdima}
        \pgfkeys{/pgf/fpu} % for bigger dimen
        \ifnum\c@pgf@counta=1

            % \pgfmathsetlength{\pgf@x}{(-sqrt(\rad^2*\@tempdima^2+\rad^2-\@tempdimb^2) - \@tempdimb*\@tempdima)/(\@tempdima^2+1)}
            \pgfmathparse{(-sqrt(\rad^2*\@tempdima^2+\rad^2-\@tempdimb^2) - \@tempdimb*\@tempdima)/(\@tempdima^2+1)}
            \pgfmathfloattofixed{\pgfmathresult}
            \pgf@x=\pgfmathresult pt
        \else
            % \pgftext{\the\@tempdimb}
            \pgfmathparse{(sqrt(\rad^2*\@tempdima^2+\rad^2-\@tempdimb^2) - \@tempdimb*\@tempdima)/(\@tempdima^2+1)}
            \pgfmathfloattofixed{\pgfmathresult}
            \pgf@x=\pgfmathresult pt

        \fi
        \pgfkeys{/pgf/fpu=false} % for bigger dimen
        \pgfmathsetlength{\pgf@y}{\@tempdima*\pgf@x+\@tempdimb}
    \fi
    \advance\pgf@x by \pgf@xc
    \advance\pgf@y by \pgf@yc
}

\def\sbgn@subunits#1{
    \pgfkeysalso{/tikz/fit=#1}
    \pgfkeysalso{
        /tikz/text width/.expand once=\tikz@text@width+20pt,
        /tikz/text height/.expand once=\tikz@text@height+16pt,
        /tikz/text depth/.expand once=\tikz@text@depth+20pt
    }
}

\pgfkeys{/tikz/isnode/.initial=false, /tikz/every node/.style={/tikz/isnode=true}}
\pgfkeys{/pgf/.cd, clone/.initial/.expanded=false, clone/.default/.expanded=\true}
\pgfkeys{/pgf/.cd, connectors/.initial=none}
\pgfkeys{/pgf/.cd, left connector length/.initial=8pt}
\pgfkeys{/pgf/.cd, right connector length/.initial=8pt}
\pgfkeys{/pgf/.cd, orientation/.initial=right}
\pgfkeys{/tikz/subunits/.code=\sbgn@subunits{#1}}
% this awesome piece of code was written by Loop Space and taken from https://tex.stackexchange.com/questions/20425/z-level-in-tikz/20426#20426
\pgfkeys{/tikz/draw layer/.code={
    \pgfonlayer{#1}\begingroup
    \aftergroup\endpgfonlayer
    \aftergroup\endgroup
    }
}

\pgfkeys{/tikz/node layer/.code={%
    \gdef\node@@layer{%
      \setbox\tikz@tempbox=\hbox\bgroup\pgfonlayer{#1}\unhbox\tikz@tempbox\endpgfonlayer\egroup}
    \aftergroup\node@layer
  }
}

\def\node@layer{\aftergroup\node@@layer}


==> tikzlibrarysbgn.shapes.tex <==
\pgfdeclareshape{dissociation}{
    % \savedmacro\lanchor{0.75}
    \inheritsavedanchors[from=circle]
    \inheritanchorborder[from=circle]
    \foreach \a in {center, south east, south west, north east, north west}
    {
        \inheritanchor[from=circle]{\a}
    }

    \savedanchor\connectoreast{
        \pgfkeysgetvalue{/pgf/connectors}{\connectors}
        %compute width and height without taking into account outer sep
        \pgf@x=\wd\pgfnodeparttextbox
        \pgf@xc=\pgfkeysvalueof{/pgf/inner xsep}
        \advance\pgf@x by 2\pgf@xc
        \pgf@xc=\pgfkeysvalueof{/pgf/minimum width}
        \ifdim\pgf@xc>\pgf@x
            \pgf@x=\pgf@xc
        \fi
        \pgf@y=\ht\pgfnodeparttextbox
        \advance\pgf@y by \dp\pgfnodeparttextbox
        \pgf@yc=\pgfkeysvalueof{/pgf/inner ysep}
        \advance\pgf@y by 2\pgf@yc
        \pgf@yc=\pgfkeysvalueof{/pgf/minimum height}
        \ifdim\pgf@yc>\pgf@y
            \pgf@y=\pgf@yc
        \fi
        %store south west in xa,ya and north east in xb,yb
        \pgf@xa=-0.5\pgf@x
        \advance\pgf@xa by 0.5\wd\pgfnodeparttextbox
        \pgf@ya=-0.5\pgf@y
        \advance\pgf@ya by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@ya by -0.5\dp\pgfnodeparttextbox
        \pgf@xb=0.5\pgf@x
        \advance\pgf@xb by 0.5\wd\pgfnodeparttextbox
        \pgf@yb=0.5\pgf@y
        \advance\pgf@yb by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@yb by -0.5\dp\pgfnodeparttextbox
        %compute anchor
        \pgf@y=0.5\pgf@yb
        \advance\pgf@y by 0.5\pgf@ya
        \pgf@x=\pgf@xb
        \ifx\connectors\horizontal
            \pgfkeysgetvalue{/pgf/right connector length}{\lconnector}
            \advance\pgf@x by \lconnector
        \fi
    }

    \savedanchor\connectorwest{
        \pgfkeysgetvalue{/pgf/connectors}{\connectors}
        %compute width and height without taking into account outer sep
        \pgf@x=\wd\pgfnodeparttextbox
        \pgf@xc=\pgfkeysvalueof{/pgf/inner xsep}
        \advance\pgf@x by 2\pgf@xc
        \pgf@xc=\pgfkeysvalueof{/pgf/minimum width}
        \ifdim\pgf@xc>\pgf@x
            \pgf@x=\pgf@xc
        \fi
        \pgf@y=\ht\pgfnodeparttextbox
        \advance\pgf@y by \dp\pgfnodeparttextbox
        \pgf@yc=\pgfkeysvalueof{/pgf/inner ysep}
        \advance\pgf@y by 2\pgf@yc
        \pgf@yc=\pgfkeysvalueof{/pgf/minimum height}
        \ifdim\pgf@yc>\pgf@y
            \pgf@y=\pgf@yc
        \fi
        %store south west in xa,ya and north east in xb,yb
        \pgf@xa=-0.5\pgf@x
        \advance\pgf@xa by 0.5\wd\pgfnodeparttextbox
        \pgf@ya=-0.5\pgf@y
        \advance\pgf@ya by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@ya by -0.5\dp\pgfnodeparttextbox
        \pgf@xb=0.5\pgf@x
        \advance\pgf@xb by 0.5\wd\pgfnodeparttextbox
        \pgf@yb=0.5\pgf@y
        \advance\pgf@yb by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@yb by -0.5\dp\pgfnodeparttextbox
        %compute anchor
        \pgf@y=0.5\pgf@yb
        \advance\pgf@y by 0.5\pgf@ya
        \pgf@x=\pgf@xa
        \ifx\connectors\horizontal
            \pgfkeysgetvalue{/pgf/left connector length}{\lconnector}
            \advance\pgf@x by -\lconnector
        \fi
    }

    \savedanchor\connectornorth{
        \pgfkeysgetvalue{/pgf/connectors}{\connectors}
        %compute width and height without taking into account outer sep
        \pgf@x=\wd\pgfnodeparttextbox
        \pgf@xc=\pgfkeysvalueof{/pgf/inner xsep}
        \advance\pgf@x by 2\pgf@xc
        \pgf@xc=\pgfkeysvalueof{/pgf/minimum width}
        \ifdim\pgf@xc>\pgf@x
            \pgf@x=\pgf@xc
        \fi
        \pgf@y=\ht\pgfnodeparttextbox
        \advance\pgf@y by \dp\pgfnodeparttextbox
        \pgf@yc=\pgfkeysvalueof{/pgf/inner ysep}
        \advance\pgf@y by 2\pgf@yc
        \pgf@yc=\pgfkeysvalueof{/pgf/minimum height}
        \ifdim\pgf@yc>\pgf@y
            \pgf@y=\pgf@yc
        \fi
        %store south west in xa,ya and north east in xb,yb
        \pgf@xa=-0.5\pgf@x
        \advance\pgf@xa by 0.5\wd\pgfnodeparttextbox
        \pgf@ya=-0.5\pgf@y
        \advance\pgf@ya by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@ya by -0.5\dp\pgfnodeparttextbox
        \pgf@xb=0.5\pgf@x
        \advance\pgf@xb by 0.5\wd\pgfnodeparttextbox
        \pgf@yb=0.5\pgf@y
        \advance\pgf@yb by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@yb by -0.5\dp\pgfnodeparttextbox
        %compute anchor
        \pgf@x=0.5\pgf@xb
        \advance\pgf@x by 0.5\pgf@xa
        \pgf@y=\pgf@yb
        \ifx\connectors\vertical
            \pgfkeysgetvalue{/pgf/left connector length}{\lconnector}
            \advance\pgf@y by \lconnector
        \fi
    }

    \savedanchor\connectorsouth{
        \pgfkeysgetvalue{/pgf/connectors}{\connectors}
        %compute width and height without taking into account outer sep
        \pgf@x=\wd\pgfnodeparttextbox
        \pgf@xc=\pgfkeysvalueof{/pgf/inner xsep}
        \advance\pgf@x by 2\pgf@xc
        \pgf@xc=\pgfkeysvalueof{/pgf/minimum width}
        \ifdim\pgf@xc>\pgf@x
            \pgf@x=\pgf@xc
        \fi
        \pgf@y=\ht\pgfnodeparttextbox
        \advance\pgf@y by \dp\pgfnodeparttextbox
        \pgf@yc=\pgfkeysvalueof{/pgf/inner ysep}
        \advance\pgf@y by 2\pgf@yc
        \pgf@yc=\pgfkeysvalueof{/pgf/minimum height}
        \ifdim\pgf@yc>\pgf@y
            \pgf@y=\pgf@yc
        \fi
        %store south west in xa,ya and north east in xb,yb
        \pgf@xa=-0.5\pgf@x
        \advance\pgf@xa by 0.5\wd\pgfnodeparttextbox
        \pgf@ya=-0.5\pgf@y
        \advance\pgf@ya by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@ya by -0.5\dp\pgfnodeparttextbox
        \pgf@xb=0.5\pgf@x
        \advance\pgf@xb by 0.5\wd\pgfnodeparttextbox
        \pgf@yb=0.5\pgf@y
        \advance\pgf@yb by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@yb by -0.5\dp\pgfnodeparttextbox
        %compute anchor
        \pgf@x=0.5\pgf@xb
        \advance\pgf@x by 0.5\pgf@xa
        \pgf@y=\pgf@ya
        \ifx\connectors\vertical
            \pgfkeysgetvalue{/pgf/right connector length}{\lconnector}
            \advance\pgf@y by -\lconnector
        \fi
    }

    \anchor{west}{\connectorwest}
    \anchor{east}{\connectoreast}
    \anchor{north}{\connectornorth}
    \anchor{south}{\connectorsouth}

    \backgroundpath{
        \pgfpathcircle{\centerpoint}{\radius}
        \pgfpathcircle{\centerpoint}{0.6*\radius}
        \pgfkeysgetvalue{/pgf/connectors}{\connectors}
        \ifx\connectors\horizontal
            \pgfkeysgetvalue{/pgf/left connector length}{\lconnector}
            \pgfkeysgetvalue{/pgf/right connector length}{\rconnector}
            \pgf@process{\centerpoint}
            \pgf@xc=\pgf@x
            \pgf@yc=\pgf@y
            \pgf@xb = \radius
            \advance\pgf@xc by \pgf@xb
            \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@xc by \rconnector
            \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@xc by -\rconnector
            \advance\pgf@xc by -2\pgf@xb
            \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@xc by -\lconnector
            \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
        \fi
        \ifx\connectors\vertical
            \pgfkeysgetvalue{/pgf/left connector length}{\lconnector}
            \pgfkeysgetvalue{/pgf/right connector length}{\rconnector}
            \pgf@process{\centerpoint}
            \pgf@xc=\pgf@x
            \pgf@yc=\pgf@y
            \pgf@xb = \radius
            \advance\pgf@yc by \pgf@xb
            \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@yc by \lconnector
            \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@yc by -\lconnector
            \advance\pgf@yc by -2\pgf@xb
            \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@yc by -\rconnector
            \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
        \fi
    }
}
\pgfdeclareshape{phenotype}{
    \inheritsavedanchors[from=rectangle] % this is nearly a rectangle
    \inheritanchorborder[from=rectangle]

    \foreach \a in {center, north, south, west, east, south east, south west, north east, north west}
    {
        \inheritanchor[from=rectangle]{\a}
    }

    \backgroundpath{
        \pgf@process{\southwest}
        \pgfgetlastxy{\xa}{\ya}
        \pgf@process{\northeast}
        \pgfgetlastxy{\xb}{\yb}
        \pgf@yc = \yb
        \pgfmathsetlength{\pgf@xc}{\xa+0.20*(\xb-\xa)}
        \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc}}
        \pgfmathsetlength{\pgf@xc}{\xb-0.20*(\xb-\xa)}
        \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
        \pgfmathsetlength{\pgf@yc}{\ya+0.5*(\yb-\ya)}
        \pgf@xc = \xb
        \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
        \pgfmathsetlength{\pgf@xc}{\xb-0.20*(\xb-\xa)}
        \pgf@yc = \ya
        \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
        \pgfmathsetlength{\pgf@xc}{\xa+0.20*(\xb-\xa)}
        \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
        \pgfmathsetlength{\pgf@yc}{\ya+0.5*(\yb-\ya)}
        \pgf@xc = \xa
        \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
        \pgfclosepath
    }
}
\pgfdeclareshape{sv}{

    \savedanchor\northeast{
        \pgf@x = \wd\pgfnodeparttextbox
        \pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/pgf/inner xsep}}
        \advance\pgf@x by 2\pgf@xa
        \pgf@xb=\pgfkeysvalueof{/pgf/minimum width}
        \ifdim\pgf@xb>\pgf@x
            \pgf@x=\pgf@xb
        \fi
        \pgf@y = \ht\pgfnodeparttextbox
        \advance\pgf@y by \dp\pgfnodeparttextbox
        \pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/pgf/inner ysep}}
        \advance\pgf@y by 2\pgf@xa
        \pgf@yb=\pgfkeysvalueof{/pgf/minimum height}
        \ifdim\pgf@yb>\pgf@y
            \pgf@y=\pgf@yb
        \fi
        \ifdim\pgf@y>\pgf@x
            \pgf@x=\pgf@y
        \fi
        \pgf@x = 0.5\pgf@x
        \advance\pgf@x by 0.5\wd\pgfnodeparttextbox
        \pgf@y = 0.5\pgf@y
        \advance\pgf@y by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@y by -0.5\dp\pgfnodeparttextbox
    }

    \savedanchor\southwest{
        \pgf@x = \wd\pgfnodeparttextbox
        \pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/pgf/inner xsep}}
        \advance\pgf@x by 2\pgf@xa
        \pgf@xb=\pgfkeysvalueof{/pgf/minimum width}
        \ifdim\pgf@xb>\pgf@x
            \pgf@x=\pgf@xb
        \fi
        \pgf@y = \ht\pgfnodeparttextbox
        \advance\pgf@y by \dp\pgfnodeparttextbox
        \pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/pgf/inner ysep}}
        \advance\pgf@y by 2\pgf@xa
        \pgf@yb=\pgfkeysvalueof{/pgf/minimum height}
        \ifdim\pgf@yb>\pgf@y
            \pgf@y=\pgf@yb
        \fi
        \ifdim\pgf@y>\pgf@x
            \pgf@x=\pgf@y
        \fi
        \pgf@x = -0.5\pgf@x
        \advance\pgf@x by 0.5\wd\pgfnodeparttextbox
        \pgf@y = -0.5\pgf@y
        \advance\pgf@y by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@y by -0.5\dp\pgfnodeparttextbox
    }

    \foreach \a in {center, north, south, west, east, south west, south east, north east, north west}
    {
        \inheritanchor[from=rectangle]{\a}
    }

    \anchorborder{
        %we put the center of shape at \pgfpointorigin!
        \@tempdima = \pgf@x
        \@tempdimb = \pgf@y
        \pgf@process{\southwest}
        \pgf@xa=\pgf@x
        \pgf@ya=\pgf@y
        \pgf@process{\northeast}
        \pgf@xb=\pgf@x
        \pgf@yb=\pgf@y
        \newdimen\radius
        \radius = 0.5\pgf@yb
        \advance\radius by -0.5\pgf@ya
        \advance\pgf@xa by \radius
        \advance\pgf@xb by -\radius
        \pgf@xc = 0.5\pgf@xa
        \advance\pgf@xc by 0.5\pgf@xb
        \pgf@yc = 0.5\pgf@ya
        \advance\pgf@yc by 0.5\pgf@yb
        \advance\pgf@xa by -\pgf@xc
        \advance\pgf@xb by -\pgf@xc
        \advance\pgf@ya by -\pgf@yc
        \advance\pgf@yb by -\pgf@yc
        \edef\pgf@marshal{%
            \noexpand\belongstocone
            {\pgfpointorigin}%
            {\noexpand\pgfpoint{\the\pgf@xa}{\the\pgf@yb}}%
            {\noexpand\pgfpoint{\the\pgf@xb}{\the\pgf@yb}}%
            {\noexpand\pgfpoint{\the\@tempdima}{\the\@tempdimb}}%
        }
        \pgf@process{\pgf@marshal}
        \if@tempswa
            % \pgftext{a}
            \edef\pgf@marshal{
                \noexpand\pgfpointborderrectangle{\noexpand\pgfpoint{\the\@tempdima}{\the\@tempdimb}}{\noexpand\pgfpoint{\the\pgf@xb}{\the\pgf@yb}}
            }
            \pgf@process{\pgf@marshal}
        \else
            \edef\pgf@marshal{%
                \noexpand\belongstocone
                {\pgfpointorigin}%
                {\noexpand\pgfpoint{\the\pgf@xb}{\the\pgf@ya}}%
                {\noexpand\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}%
                {\noexpand\pgfpoint{\the\@tempdima}{\the\@tempdimb}}%
            }
            \pgf@process{\pgf@marshal}
            \if@tempswa
                % \pgftext{b}
                \edef\pgf@marshal{%
                    \noexpand\pgfpointborderrectangle{\noexpand\pgfpoint{\the\@tempdima}{\the\@tempdimb}}{\noexpand\pgfpoint{\the\pgf@xb}{\the\pgf@yb}}
                }
                \pgf@process{\pgf@marshal}
            \else
                \edef\pgf@marshal{%
                    \noexpand\belongstocone
                    {\pgfpointorigin}%
                    {\noexpand\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}%
                    {\noexpand\pgfpoint{\the\pgf@xa}{\the\pgf@yb}}%
                    {\noexpand\pgfpoint{\the\@tempdima}{\the\@tempdimb}}%
                }
                \pgf@process{\pgf@marshal}
                \if@tempswa
                    % \pgftext{c}
                    \edef\pgf@marshal{
                        \noexpand\intersectionlinecircle{\noexpand\pgfpointorigin}{\noexpand\pgfpoint{\the\@tempdima}{\the\@tempdimb}}{\noexpand\pgfpoint{\the\pgf@xa}{0pt}}{\the\radius}{1}
                    }
                    \pgf@process{\pgf@marshal}
                \else
                    % \pgftext{d}
                    \edef\pgf@marshal{
                        \noexpand\intersectionlinecircle{\noexpand\pgfpointorigin}{\noexpand\pgfpoint{\the\@tempdima}{\the\@tempdimb}}{\noexpand\pgfpoint{\the\pgf@xb}{0pt}}{\the\radius}{2}
                    }
                    \pgf@process{\pgf@marshal}
                \fi
            \fi
        \fi
        \advance\pgf@x by \pgf@xc
        \advance\pgf@y by \pgf@yc
    }

    \backgroundpath{
        \pgf@process{\southwest}
        \pgf@xa=\pgf@x
        \pgf@ya=\pgf@y
        % \pgfmathsetlength{\pgf@xc}{\pgfkeysvalueof{/pgf/outer xsep}}
        % \pgfmathsetlength{\pgf@yc}{\pgfkeysvalueof{/pgf/outer ysep}}
        % \advance\pgf@xa by \pgf@xc
        % \advance\pgf@ya by \pgf@yc
        \pgf@process{\northeast}
        \pgf@xb=\pgf@x
        \pgf@yb=\pgf@y
        \newdimen\radius
        \radius = 0.5\pgf@yb
        \advance\radius by -0.5\pgf@ya
        \advance\pgf@xa by \radius
        \advance\pgf@xb by -\radius
        \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@yb}}
        \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
        \pgf@process{\pgfpatharc{90}{-90}{\radius}}
        \pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@ya}}
        \pgf@process{\pgfpatharc{270}{90}{\radius}}
        \pgfpathclose
    }
}
\pgfdeclareshape{nucleicacidfeature}{

    \savedmacro{\scarceratio}{\def\scarceratio{0.15}}

    \savedmacro\computecoordinates{%
        \pgf@yb = \ht\pgfnodeparttextbox
        \advance\pgf@yb by \dp\pgfnodeparttextbox
        \pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/pgf/inner ysep}}
        \advance\pgf@yb by 2\pgf@xa
        \pgf@yc=\pgfkeysvalueof{/pgf/minimum height}
        \ifdim\pgf@yc>\pgf@yb
            \pgf@yb=\pgf@yc
        \fi
        \pgf@xb=\wd\pgfnodeparttextbox
        \pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/pgf/inner xsep}}
        \advance\pgf@xb by 2\pgf@xa
        \pgf@xc=\pgfkeysvalueof{/pgf/minimum width}
        \ifdim\pgf@xc>\pgf@xb
            \pgf@xb=\pgf@xc
        \fi
        \ifdim\pgf@yb>\pgf@xb
            \pgfmathsetlengthmacro\scarceoffset{\scarceratio*\pgf@xb}
        \else
            \pgfmathsetlengthmacro\scarceoffset{\scarceratio*\pgf@yb}
        \fi
        \addtosavedmacro\scarceoffset
        \pgf@xa=-0.5\pgf@xb
        \advance\pgf@xa by 0.5\wd\pgfnodeparttextbox
        \pgf@xc=\pgf@xa %saving for later
        \pgf@ya=0.5\pgf@yb
        \advance\pgf@ya by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@ya by -0.5\dp\pgfnodeparttextbox
        \pgfextract@process\northwest{\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}
        \addtosavedmacro{\northwest}
        \advance\pgf@xa by \pgf@xb
        \pgfextract@process\northeast{\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}
        \addtosavedmacro{\northeast}
        \advance\pgf@ya by -\pgf@yb
        \advance\pgf@ya by \scarceoffset
        \pgfextract@process\eastsouthjoin{\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}
        \addtosavedmacro{\eastsouthjoin}
        \advance\pgf@ya by -\scarceoffset
        \advance\pgf@xa by -\scarceoffset
        \pgfextract@process\southeastjoin{\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}
        \addtosavedmacro{\southeastjoin}
        \pgf@xa=\pgf@xc
        \advance\pgf@xa by \scarceoffset
        \pgfextract@process\southwestjoin{\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}
        \addtosavedmacro{\southwestjoin}
        \advance\pgf@xa by -\scarceoffset
        \advance\pgf@ya by \scarceoffset
        \pgfextract@process\westsouthjoin{\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}
        \addtosavedmacro{\westsouthjoin}
    }

    \savedanchor{\southwest}{
        \northwest
        \pgf@xc=\pgf@x
        \southwestjoin
        \pgf@x=\pgf@xc
    }

    \savedanchor{\northeast}{
        \northeast
    }

    \anchor{south west}{
        \southwest
    }

    \anchor{north east}{
        \northeast
    }


    \anchor{south east}{
        \northeast
        \pgf@xc=\pgf@x
        \southwest
        \pgf@x=\pgf@xc
    }

    \anchor{north west}{
        \southwest
        \pgf@xc=\pgf@x
        \northeast
        \pgf@x=\pgf@xc
    }

    \inheritanchorborder[from=rectangle]

    \foreach \a in {center, north, south, west, east}
    {
        \inheritanchor[from=rectangle]{\a}
    }

    \backgroundpath{
        \computecoordinates
        \pgfpathmoveto{\northwest}
        \pgfpathlineto{\northeast}
        \pgfpathlineto{\eastsouthjoin}
        \pgfpatharc{0}{-90}{\scarceoffset}
        \pgfpathlineto{\southwestjoin}
        \pgfpatharc{-90}{-180}{\scarceoffset}
        \pgfpathclose
    }

    \foregroundpath{
        \pgfkeysgetvalue{/pgf/clone}{\clone}
        \ifx\clone\true
            \def\cloneoffsetratio{0.25}
            \computecoordinates
            \northwest
            \pgf@ya=\pgf@y
            \pgf@xc=\pgf@x
            \southwestjoin
            \advance\pgf@ya by -\pgf@y
            \newdimen\cloneoffset
            \cloneoffset=\cloneoffsetratio\pgf@ya
            \pgf@yc=\pgf@y
            \advance\pgf@yc by \cloneoffset
            \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \northeast
            \pgf@xc=\pgf@x
            \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \pgfpathlineto{\eastsouthjoin}
            \pgfpatharc{0}{-90}{\scarceoffset}
            \pgfpathlineto{\southwestjoin}
            \pgfpatharc{-90}{-180}{\scarceoffset}
            \pgfpathclose
            \pgfsetfillcolor{\tikz@strokecolor}
            \pgfusepath{fill, stroke}
        \fi
    }
}
\pgfdeclareshape{svexistence}{
    \inheritsavedanchors[from=circle]
    \inheritanchorborder[from=circle]
    \foreach \a in {center, east, south, north, west, south east, south west, north east, north west}
    {
        \inheritanchor[from=circle]{\a}
    }
    \backgroundpath{
        \@tempdima = \radius
        \pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/pgf/outer xsep}}
        \advance\@tempdima by -\pgf@xa
        \pgfpathcircle{\centerpoint}{\@tempdima}
        \pgfusepath{stroke, fill}
        \centerpoint
        \pgf@xc = \pgf@x
        \pgf@yc = \pgf@y
        \advance\pgf@y by \@tempdima
        \pgfpathmoveto{\pgfpoint{\pgf@x}{\pgf@y}}
        \pgfpatharc{90}{-90}{\@tempdima}
        \pgfclosepath
        \pgfsetfillcolor{\tikz@strokecolor}
        \pgfusepath{stroke, fill}
    }
}
\pgfdeclareshape{uncertainprocess}{
    % \savedmacro\lanchor{0.75}
    \inheritsavedanchors[from=rectangle]
    \inheritanchorborder[from=rectangle]
    \foreach \a in {center, south east, south west, north east, north west}
    {
        \inheritanchor[from=rectangle]{\a}
    }

    \savedanchor\connectoreast{
        \pgfkeysgetvalue{/pgf/connectors}{\connectors}
        %compute width and height without taking into account outer sep
        \pgf@x=\wd\pgfnodeparttextbox
        \pgf@xc=\pgfkeysvalueof{/pgf/inner xsep}
        \advance\pgf@x by 2\pgf@xc
        \pgf@xc=\pgfkeysvalueof{/pgf/minimum width}
        \ifdim\pgf@xc>\pgf@x
            \pgf@x=\pgf@xc
        \fi
        \pgf@y=\ht\pgfnodeparttextbox
        \advance\pgf@y by \dp\pgfnodeparttextbox
        \pgf@yc=\pgfkeysvalueof{/pgf/inner ysep}
        \advance\pgf@y by 2\pgf@yc
        \pgf@yc=\pgfkeysvalueof{/pgf/minimum height}
        \ifdim\pgf@yc>\pgf@y
            \pgf@y=\pgf@yc
        \fi
        %store south west in xa,ya and north east in xb,yb
        \pgf@xa=-0.5\pgf@x
        \advance\pgf@xa by 0.5\wd\pgfnodeparttextbox
        \pgf@ya=-0.5\pgf@y
        \advance\pgf@ya by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@ya by -0.5\dp\pgfnodeparttextbox
        \pgf@xb=0.5\pgf@x
        \advance\pgf@xb by 0.5\wd\pgfnodeparttextbox
        \pgf@yb=0.5\pgf@y
        \advance\pgf@yb by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@yb by -0.5\dp\pgfnodeparttextbox
        %compute anchor
        \pgf@y=0.5\pgf@yb
        \advance\pgf@y by 0.5\pgf@ya
        \pgf@x=\pgf@xb
        \ifx\connectors\horizontal
            \pgfkeysgetvalue{/pgf/right connector length}{\lconnector}
            \advance\pgf@x by \lconnector
        \fi
    }

    \savedanchor\connectorwest{
        \pgfkeysgetvalue{/pgf/connectors}{\connectors}
        %compute width and height without taking into account outer sep
        \pgf@x=\wd\pgfnodeparttextbox
        \pgf@xc=\pgfkeysvalueof{/pgf/inner xsep}
        \advance\pgf@x by 2\pgf@xc
        \pgf@xc=\pgfkeysvalueof{/pgf/minimum width}
        \ifdim\pgf@xc>\pgf@x
            \pgf@x=\pgf@xc
        \fi
        \pgf@y=\ht\pgfnodeparttextbox
        \advance\pgf@y by \dp\pgfnodeparttextbox
        \pgf@yc=\pgfkeysvalueof{/pgf/inner ysep}
        \advance\pgf@y by 2\pgf@yc
        \pgf@yc=\pgfkeysvalueof{/pgf/minimum height}
        \ifdim\pgf@yc>\pgf@y
            \pgf@y=\pgf@yc
        \fi
        %store south west in xa,ya and north east in xb,yb
        \pgf@xa=-0.5\pgf@x
        \advance\pgf@xa by 0.5\wd\pgfnodeparttextbox
        \pgf@ya=-0.5\pgf@y
        \advance\pgf@ya by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@ya by -0.5\dp\pgfnodeparttextbox
        \pgf@xb=0.5\pgf@x
        \advance\pgf@xb by 0.5\wd\pgfnodeparttextbox
        \pgf@yb=0.5\pgf@y
        \advance\pgf@yb by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@yb by -0.5\dp\pgfnodeparttextbox
        %compute anchor
        \pgf@y=0.5\pgf@yb
        \advance\pgf@y by 0.5\pgf@ya
        \pgf@x=\pgf@xa
        \ifx\connectors\horizontal
            \pgfkeysgetvalue{/pgf/left connector length}{\lconnector}
            \advance\pgf@x by -\lconnector
        \fi
    }

    \savedanchor\connectornorth{
        \pgfkeysgetvalue{/pgf/connectors}{\connectors}
        %compute width and height without taking into account outer sep
        \pgf@x=\wd\pgfnodeparttextbox
        \pgf@xc=\pgfkeysvalueof{/pgf/inner xsep}
        \advance\pgf@x by 2\pgf@xc
        \pgf@xc=\pgfkeysvalueof{/pgf/minimum width}
        \ifdim\pgf@xc>\pgf@x
            \pgf@x=\pgf@xc
        \fi
        \pgf@y=\ht\pgfnodeparttextbox
        \advance\pgf@y by \dp\pgfnodeparttextbox
        \pgf@yc=\pgfkeysvalueof{/pgf/inner ysep}
        \advance\pgf@y by 2\pgf@yc
        \pgf@yc=\pgfkeysvalueof{/pgf/minimum height}
        \ifdim\pgf@yc>\pgf@y
            \pgf@y=\pgf@yc
        \fi
        %store south west in xa,ya and north east in xb,yb
        \pgf@xa=-0.5\pgf@x
        \advance\pgf@xa by 0.5\wd\pgfnodeparttextbox
        \pgf@ya=-0.5\pgf@y
        \advance\pgf@ya by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@ya by -0.5\dp\pgfnodeparttextbox
        \pgf@xb=0.5\pgf@x
        \advance\pgf@xb by 0.5\wd\pgfnodeparttextbox
        \pgf@yb=0.5\pgf@y
        \advance\pgf@yb by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@yb by -0.5\dp\pgfnodeparttextbox
        %compute anchor
        \pgf@x=0.5\pgf@xb
        \advance\pgf@x by 0.5\pgf@xa
        \pgf@y=\pgf@yb
        \ifx\connectors\vertical
            \pgfkeysgetvalue{/pgf/left connector length}{\lconnector}
            \advance\pgf@y by \lconnector
        \fi
    }

    \savedanchor\connectorsouth{
        \pgfkeysgetvalue{/pgf/connectors}{\connectors}
        %compute width and height without taking into account outer sep
        \pgf@x=\wd\pgfnodeparttextbox
        \pgf@xc=\pgfkeysvalueof{/pgf/inner xsep}
        \advance\pgf@x by 2\pgf@xc
        \pgf@xc=\pgfkeysvalueof{/pgf/minimum width}
        \ifdim\pgf@xc>\pgf@x
            \pgf@x=\pgf@xc
        \fi
        \pgf@y=\ht\pgfnodeparttextbox
        \advance\pgf@y by \dp\pgfnodeparttextbox
        \pgf@yc=\pgfkeysvalueof{/pgf/inner ysep}
        \advance\pgf@y by 2\pgf@yc
        \pgf@yc=\pgfkeysvalueof{/pgf/minimum height}
        \ifdim\pgf@yc>\pgf@y
            \pgf@y=\pgf@yc
        \fi
        %store south west in xa,ya and north east in xb,yb
        \pgf@xa=-0.5\pgf@x
        \advance\pgf@xa by 0.5\wd\pgfnodeparttextbox
        \pgf@ya=-0.5\pgf@y
        \advance\pgf@ya by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@ya by -0.5\dp\pgfnodeparttextbox
        \pgf@xb=0.5\pgf@x
        \advance\pgf@xb by 0.5\wd\pgfnodeparttextbox
        \pgf@yb=0.5\pgf@y
        \advance\pgf@yb by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@yb by -0.5\dp\pgfnodeparttextbox
        %compute anchor
        \pgf@x=0.5\pgf@xb
        \advance\pgf@x by 0.5\pgf@xa
        \pgf@y=\pgf@ya
        \ifx\connectors\vertical
            \pgfkeysgetvalue{/pgf/right connector length}{\lconnector}
            \advance\pgf@y by -\lconnector
        \fi
    }

    \anchor{west}{\connectorwest}
    \anchor{east}{\connectoreast}
    \anchor{north}{\connectornorth}
    \anchor{south}{\connectorsouth}

    \backgroundpath{
        \pgfpathrectanglecorners{\southwest}{\northeast}
        \pgfkeysgetvalue{/pgf/connectors}{\connectors}
        \ifx\connectors\horizontal
            \pgfkeysgetvalue{/pgf/left connector length}{\lconnector}
            \pgfkeysgetvalue{/pgf/right connector length}{\rconnector}
            \pgf@process{\southwest}
            \pgf@xa = \pgf@x
            \pgf@ya = \pgf@y
            \pgf@process{\northeast}
            \pgf@xb = \pgf@x
            \pgf@yb = \pgf@y
            \pgf@xc=\pgf@x
            \pgf@yc=\pgf@y
            \advance\pgf@yc by -0.5\pgf@yb
            \advance\pgf@yc by 0.5\pgf@ya
            \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@xc by \rconnector
            \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \pgf@xc=\pgf@xa
            \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@xc by -\lconnector
            \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
        \fi
        \ifx\connectors\vertical
            \pgfkeysgetvalue{/pgf/left connector length}{\lconnector}
            \pgfkeysgetvalue{/pgf/right connector length}{\rconnector}
            \pgf@process{\southwest}
            \pgf@xa = \pgf@x
            \pgf@ya = \pgf@y
            \pgf@process{\northeast}
            \pgf@xb = \pgf@x
            \pgf@yb = \pgf@y
            \pgf@xc=\pgf@x
            \pgf@yc=\pgf@y
            \advance\pgf@xc by -0.5\pgf@xb
            \advance\pgf@xc by 0.5\pgf@xa
            \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@yc by \rconnector
            \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \pgf@yc=\pgf@ya
            \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@yc by -\lconnector
            \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
        \fi
    }

    \foregroundpath{
        \pgf@process{\southwest}
        \pgf@ya = \pgf@y
        \pgf@process{\northeast}
        \pgf@yb = \pgf@y
        \pgf@x = \pgf@yb
        \advance\pgf@x by -\pgf@ya
        \pgftext{\fontsize{\pgf@x}{\pgf@x}\selectfont\sffamily\textcolor{\tikz@strokecolor}{?}}
    }
}
\pgfdeclareshape{simplechemical}{

    \savedanchor\northeast{
        \pgf@x = \wd\pgfnodeparttextbox
        \pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/pgf/inner xsep}}
        \advance\pgf@x by 2\pgf@xa
        \pgf@xb=\pgfkeysvalueof{/pgf/minimum width}
        \ifdim\pgf@xb>\pgf@x
            \pgf@x=\pgf@xb
        \fi
        \pgf@y = \ht\pgfnodeparttextbox
        \advance\pgf@y by \dp\pgfnodeparttextbox
        \pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/pgf/inner ysep}}
        \advance\pgf@y by 2\pgf@xa
        \pgf@yb=\pgfkeysvalueof{/pgf/minimum height}
        \ifdim\pgf@yb>\pgf@y
            \pgf@y=\pgf@yb
        \fi
        \ifdim\pgf@y>\pgf@x
            \pgf@x=\pgf@y
        \fi
        \pgf@x = 0.5\pgf@x
        \advance\pgf@x by 0.5\wd\pgfnodeparttextbox
        \pgf@y = 0.5\pgf@y
        \advance\pgf@y by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@y by -0.5\dp\pgfnodeparttextbox
    }

    \savedanchor\southwest{
        \pgf@x = \wd\pgfnodeparttextbox
        \pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/pgf/inner xsep}}
        \advance\pgf@x by 2\pgf@xa
        \pgf@xb=\pgfkeysvalueof{/pgf/minimum width}
        \ifdim\pgf@xb>\pgf@x
            \pgf@x=\pgf@xb
        \fi
        \pgf@y = \ht\pgfnodeparttextbox
        \advance\pgf@y by \dp\pgfnodeparttextbox
        \pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/pgf/inner ysep}}
        \advance\pgf@y by 2\pgf@xa
        \pgf@yb=\pgfkeysvalueof{/pgf/minimum height}
        \ifdim\pgf@yb>\pgf@y
            \pgf@y=\pgf@yb
        \fi
        \ifdim\pgf@y>\pgf@x
            \pgf@x=\pgf@y
        \fi
        \pgf@x = -0.5\pgf@x
        \advance\pgf@x by 0.5\wd\pgfnodeparttextbox
        \pgf@y = -0.5\pgf@y
        \advance\pgf@y by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@y by -0.5\dp\pgfnodeparttextbox
    }

    \foreach \a in {center, north, south, west, east, south west, south east, north east, north west}
    {
        \inheritanchor[from=rectangle]{\a}
    }

    \anchorborder{
        %we put the center of shape at \pgfpointorigin!
        \@tempdima = \pgf@x
        \@tempdimb = \pgf@y
        \pgf@process{\southwest}
        \pgf@xa=\pgf@x
        \pgf@ya=\pgf@y
        \pgf@process{\northeast}
        \pgf@xb=\pgf@x
        \pgf@yb=\pgf@y
        \newdimen\radius
        \radius = 0.5\pgf@yb
        \advance\radius by -0.5\pgf@ya
        \advance\pgf@xa by \radius
        \advance\pgf@xb by -\radius
        \pgf@xc = 0.5\pgf@xa
        \advance\pgf@xc by 0.5\pgf@xb
        \pgf@yc = 0.5\pgf@ya
        \advance\pgf@yc by 0.5\pgf@yb
        \advance\pgf@xa by -\pgf@xc
        \advance\pgf@xb by -\pgf@xc
        \advance\pgf@ya by -\pgf@yc
        \advance\pgf@yb by -\pgf@yc
        \edef\pgf@marshal{%
            \noexpand\belongstocone
            {\pgfpointorigin}%
            {\noexpand\pgfpoint{\the\pgf@xa}{\the\pgf@yb}}%
            {\noexpand\pgfpoint{\the\pgf@xb}{\the\pgf@yb}}%
            {\noexpand\pgfpoint{\the\@tempdima}{\the\@tempdimb}}%
        }
        \pgf@process{\pgf@marshal}
        \if@tempswa
            % \pgftext{a}
            \edef\pgf@marshal{
                \noexpand\pgfpointborderrectangle{\noexpand\pgfpoint{\the\@tempdima}{\the\@tempdimb}}{\noexpand\pgfpoint{\the\pgf@xb}{\the\pgf@yb}}
            }
            \pgf@process{\pgf@marshal}
        \else
            \edef\pgf@marshal{%
                \noexpand\belongstocone
                {\pgfpointorigin}%
                {\noexpand\pgfpoint{\the\pgf@xb}{\the\pgf@ya}}%
                {\noexpand\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}%
                {\noexpand\pgfpoint{\the\@tempdima}{\the\@tempdimb}}%
            }
            \pgf@process{\pgf@marshal}
            \if@tempswa
                % \pgftext{b}
                \edef\pgf@marshal{%
                    \noexpand\pgfpointborderrectangle{\noexpand\pgfpoint{\the\@tempdima}{\the\@tempdimb}}{\noexpand\pgfpoint{\the\pgf@xb}{\the\pgf@yb}}
                }
                \pgf@process{\pgf@marshal}
            \else
                \edef\pgf@marshal{%
                    \noexpand\belongstocone
                    {\pgfpointorigin}%
                    {\noexpand\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}%
                    {\noexpand\pgfpoint{\the\pgf@xa}{\the\pgf@yb}}%
                    {\noexpand\pgfpoint{\the\@tempdima}{\the\@tempdimb}}%
                }
                \pgf@process{\pgf@marshal}
                \if@tempswa
                    % \pgftext{c}
                    \edef\pgf@marshal{
                        \noexpand\intersectionlinecircle{\noexpand\pgfpointorigin}{\noexpand\pgfpoint{\the\@tempdima}{\the\@tempdimb}}{\noexpand\pgfpoint{\the\pgf@xa}{0pt}}{\the\radius}{1}
                    }
                    \pgf@process{\pgf@marshal}
                \else
                    % \pgftext{d}
                    \edef\pgf@marshal{
                        \noexpand\intersectionlinecircle{\noexpand\pgfpointorigin}{\noexpand\pgfpoint{\the\@tempdima}{\the\@tempdimb}}{\noexpand\pgfpoint{\the\pgf@xb}{0pt}}{\the\radius}{2}
                    }
                    \pgf@process{\pgf@marshal}
                \fi
            \fi
        \fi
        \advance\pgf@x by \pgf@xc
        \advance\pgf@y by \pgf@yc
    }

    \backgroundpath{
        \pgf@process{\southwest}
        \pgf@xa=\pgf@x
        \pgf@ya=\pgf@y
        % \pgfmathsetlength{\pgf@xc}{\pgfkeysvalueof{/pgf/outer xsep}}
        % \pgfmathsetlength{\pgf@yc}{\pgfkeysvalueof{/pgf/outer ysep}}
        % \advance\pgf@xa by \pgf@xc
        % \advance\pgf@ya by \pgf@yc
        \pgf@process{\northeast}
        \pgf@xb=\pgf@x
        \pgf@yb=\pgf@y
        \newdimen\radius
        \radius = 0.5\pgf@yb
        \advance\radius by -0.5\pgf@ya
        \advance\pgf@xa by \radius
        \advance\pgf@xb by -\radius
        \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@yb}}
        \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
        \pgf@process{\pgfpatharc{90}{-90}{\radius}}
        \pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@ya}}
        \pgf@process{\pgfpatharc{270}{90}{\radius}}
        \pgfpathclose
    }

    \foregroundpath{
        \pgfkeysgetvalue{/pgf/clone}{\clone}
        \ifx\clone\true
            \def\cloneoffset{0.25}
            \pgf@process{\southwest}
            \pgf@xa=\pgf@x
            \pgf@ya=\pgf@y
            \advance\pgf@xa by 0.5\pgflinewidth
            \advance\pgf@ya by 0.5\pgflinewidth
            \pgf@process{\northeast}
            \pgf@xb=\pgf@x
            \pgf@yb=\pgf@y
            \advance\pgf@xb by -0.5\pgflinewidth
            \advance\pgf@yb by -0.5\pgflinewidth
            \newdimen\radius
            \radius = 0.5\pgf@yb
            \advance\radius by -0.5\pgf@ya
            \pgfmathsetlength{\pgf@yc}{2*\cloneoffset*\radius-\radius}
            \pgfmathsetlength{\pgf@xc}{sqrt(\radius^2-\pgf@yc^2)}
            \pgfmathsetlength{\pgf@yc}{\pgf@ya+\cloneoffset*(\pgf@yb-\pgf@ya)}
            \pgfmathsetlength{\pgf@x}{\pgf@xa+\radius-\pgf@xc}
            \pgfpathmoveto{\pgfpoint{\pgf@x}{\pgf@yc}}
            \pgfmathsetlength{\pgf@x}{\pgf@xb-\radius+\pgf@xc}
            \pgfpathlineto{\pgfpoint{\pgf@x}{\pgf@yc}}
            \pgfmathsetlength{\pgf@xc}{round(atan2(2*\cloneoffset*\radius-\radius,sqrt(\radius^2-(2*\cloneoffset*\radius-\radius)^2))}
            \pgfpatharc{\pgf@xc}{-90}{\radius}
            \pgfmathsetlength{\pgf@x}{\pgf@xa+\radius}
            \pgfpathlineto{\pgfpoint{\pgf@x}{\pgf@ya}}
            \pgfmathsetlength{\pgf@xc}{-180-\pgf@xc}
            \pgfpatharc{-90}{\pgf@xc}{\radius}
            \pgfpathclose
            \pgfsetfillcolor{\tikz@strokecolor}
            \pgfusepath{stroke, fill}
        \fi
    }
}
\pgfdeclareshape{not}{

    \inheritsavedanchors[from=circle]
    \inheritanchorborder[from=circle]
    \foreach \a in {center, south east, south west, north east, north west}
    {
        \inheritanchor[from=circle]{\a}
    }

    \savedanchor\connectoreast{
        \pgfkeysgetvalue{/pgf/connectors}{\connectors}
        %compute width and height without taking into account outer sep
        \pgf@x=\wd\pgfnodeparttextbox
        \pgf@xc=\pgfkeysvalueof{/pgf/inner xsep}
        \advance\pgf@x by 2\pgf@xc
        \pgf@xc=\pgfkeysvalueof{/pgf/minimum width}
        \ifdim\pgf@xc>\pgf@x
            \pgf@x=\pgf@xc
        \fi
        \pgf@y=\ht\pgfnodeparttextbox
        \advance\pgf@y by \dp\pgfnodeparttextbox
        \pgf@yc=\pgfkeysvalueof{/pgf/inner ysep}
        \advance\pgf@y by 2\pgf@yc
        \pgf@yc=\pgfkeysvalueof{/pgf/minimum height}
        \ifdim\pgf@yc>\pgf@y
            \pgf@y=\pgf@yc
        \fi
        %store south west in xa,ya and north east in xb,yb
        \pgf@xa=-0.5\pgf@x
        \advance\pgf@xa by 0.5\wd\pgfnodeparttextbox
        \pgf@ya=-0.5\pgf@y
        \advance\pgf@ya by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@ya by -0.5\dp\pgfnodeparttextbox
        \pgf@xb=0.5\pgf@x
        \advance\pgf@xb by 0.5\wd\pgfnodeparttextbox
        \pgf@yb=0.5\pgf@y
        \advance\pgf@yb by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@yb by -0.5\dp\pgfnodeparttextbox
        %compute anchor
        \pgf@y=0.5\pgf@yb
        \advance\pgf@y by 0.5\pgf@ya
        \pgf@x=\pgf@xb
        \ifx\connectors\horizontal
            \pgfkeysgetvalue{/pgf/right connector length}{\lconnector}
            \advance\pgf@x by \lconnector
        \fi
    }

    \savedanchor\connectorwest{
        \pgfkeysgetvalue{/pgf/connectors}{\connectors}
        %compute width and height without taking into account outer sep
        \pgf@x=\wd\pgfnodeparttextbox
        \pgf@xc=\pgfkeysvalueof{/pgf/inner xsep}
        \advance\pgf@x by 2\pgf@xc
        \pgf@xc=\pgfkeysvalueof{/pgf/minimum width}
        \ifdim\pgf@xc>\pgf@x
            \pgf@x=\pgf@xc
        \fi
        \pgf@y=\ht\pgfnodeparttextbox
        \advance\pgf@y by \dp\pgfnodeparttextbox
        \pgf@yc=\pgfkeysvalueof{/pgf/inner ysep}
        \advance\pgf@y by 2\pgf@yc
        \pgf@yc=\pgfkeysvalueof{/pgf/minimum height}
        \ifdim\pgf@yc>\pgf@y
            \pgf@y=\pgf@yc
        \fi
        %store south west in xa,ya and north east in xb,yb
        \pgf@xa=-0.5\pgf@x
        \advance\pgf@xa by 0.5\wd\pgfnodeparttextbox
        \pgf@ya=-0.5\pgf@y
        \advance\pgf@ya by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@ya by -0.5\dp\pgfnodeparttextbox
        \pgf@xb=0.5\pgf@x
        \advance\pgf@xb by 0.5\wd\pgfnodeparttextbox
        \pgf@yb=0.5\pgf@y
        \advance\pgf@yb by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@yb by -0.5\dp\pgfnodeparttextbox
        %compute anchor
        \pgf@y=0.5\pgf@yb
        \advance\pgf@y by 0.5\pgf@ya
        \pgf@x=\pgf@xa
        \ifx\connectors\horizontal
            \pgfkeysgetvalue{/pgf/left connector length}{\lconnector}
            \advance\pgf@x by -\lconnector
        \fi
    }

    \savedanchor\connectornorth{
        \pgfkeysgetvalue{/pgf/connectors}{\connectors}
        %compute width and height without taking into account outer sep
        \pgf@x=\wd\pgfnodeparttextbox
        \pgf@xc=\pgfkeysvalueof{/pgf/inner xsep}
        \advance\pgf@x by 2\pgf@xc
        \pgf@xc=\pgfkeysvalueof{/pgf/minimum width}
        \ifdim\pgf@xc>\pgf@x
            \pgf@x=\pgf@xc
        \fi
        \pgf@y=\ht\pgfnodeparttextbox
        \advance\pgf@y by \dp\pgfnodeparttextbox
        \pgf@yc=\pgfkeysvalueof{/pgf/inner ysep}
        \advance\pgf@y by 2\pgf@yc
        \pgf@yc=\pgfkeysvalueof{/pgf/minimum height}
        \ifdim\pgf@yc>\pgf@y
            \pgf@y=\pgf@yc
        \fi
        %store south west in xa,ya and north east in xb,yb
        \pgf@xa=-0.5\pgf@x
        \advance\pgf@xa by 0.5\wd\pgfnodeparttextbox
        \pgf@ya=-0.5\pgf@y
        \advance\pgf@ya by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@ya by -0.5\dp\pgfnodeparttextbox
        \pgf@xb=0.5\pgf@x
        \advance\pgf@xb by 0.5\wd\pgfnodeparttextbox
        \pgf@yb=0.5\pgf@y
        \advance\pgf@yb by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@yb by -0.5\dp\pgfnodeparttextbox
        %compute anchor
        \pgf@x=0.5\pgf@xb
        \advance\pgf@x by 0.5\pgf@xa
        \pgf@y=\pgf@yb
        \ifx\connectors\vertical
            \pgfkeysgetvalue{/pgf/left connector length}{\lconnector}
            \advance\pgf@y by \lconnector
        \fi
    }

    \savedanchor\connectorsouth{
        \pgfkeysgetvalue{/pgf/connectors}{\lconnectors}
        %compute width and height without taking into account outer sep
        \pgf@x=\wd\pgfnodeparttextbox
        \pgf@xc=\pgfkeysvalueof{/pgf/inner xsep}
        \advance\pgf@x by 2\pgf@xc
        \pgf@xc=\pgfkeysvalueof{/pgf/minimum width}
        \ifdim\pgf@xc>\pgf@x
            \pgf@x=\pgf@xc
        \fi
        \pgf@y=\ht\pgfnodeparttextbox
        \advance\pgf@y by \dp\pgfnodeparttextbox
        \pgf@yc=\pgfkeysvalueof{/pgf/inner ysep}
        \advance\pgf@y by 2\pgf@yc
        \pgf@yc=\pgfkeysvalueof{/pgf/minimum height}
        \ifdim\pgf@yc>\pgf@y
            \pgf@y=\pgf@yc
        \fi
        %store south west in xa,ya and north east in xb,yb
        \pgf@xa=-0.5\pgf@x
        \advance\pgf@xa by 0.5\wd\pgfnodeparttextbox
        \pgf@ya=-0.5\pgf@y
        \advance\pgf@ya by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@ya by -0.5\dp\pgfnodeparttextbox
        \pgf@xb=0.5\pgf@x
        \advance\pgf@xb by 0.5\wd\pgfnodeparttextbox
        \pgf@yb=0.5\pgf@y
        \advance\pgf@yb by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@yb by -0.5\dp\pgfnodeparttextbox
        %compute anchor
        \pgf@x=0.5\pgf@xb
        \advance\pgf@x by 0.5\pgf@xa
        \pgf@y=\pgf@ya
        \ifx\connectors\vertical
            \pgfkeysgetvalue{/pgf/right connector length}{\lconnector}
            \advance\pgf@y by -\lconnector
        \fi
    }

    \anchor{west}{\connectorwest}
    \anchor{east}{\connectoreast}
    \anchor{north}{\connectornorth}
    \anchor{south}{\connectorsouth}

    \backgroundpath{
        \pgfpathcircle{\centerpoint}{\radius}
        \pgfkeysgetvalue{/pgf/connectors}{\connectors}
        \ifx\connectors\horizontal
            \pgfkeysgetvalue{/pgf/left connector length}{\lconnector}
            \pgfkeysgetvalue{/pgf/right connector length}{\rconnector}
            \pgf@process{\centerpoint}
            \pgf@xc=\pgf@x
            \pgf@yc=\pgf@y
            \pgf@xb = \radius
            \advance\pgf@xc by \pgf@xb
            \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@xc by \rconnector
            \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@xc by -\rconnector
            \advance\pgf@xc by -2\pgf@xb
            \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@xc by -\lconnector
            \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
        \fi
        \ifx\connectors\vertical
            \pgfkeysgetvalue{/pgf/left connector length}{\lconnector}
            \pgfkeysgetvalue{/pgf/right connector length}{\rconnector}
            \pgf@process{\centerpoint}
            \pgf@xc=\pgf@x
            \pgf@yc=\pgf@y
            \pgf@xb = \radius
            \advance\pgf@yc by \pgf@xb
            \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@yc by \lconnector
            \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@yc by -\lconnector
            \advance\pgf@yc by -2\pgf@xb
            \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@yc by -\rconnector
            \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
        \fi
    }

    \foregroundpath{
        \pgf@xa = \radius
        \advance\pgf@xa by -0.2\pgf@xa
        \pgftext{\fontsize{\pgf@xa}{\pgf@xa}\selectfont\sffamily\textcolor{\tikz@strokecolor}{NOT}}
    }
}
\pgfdeclareshape{emptyset}{
    \inheritsavedanchors[from=circle]
    \inheritanchorborder[from=circle]
    \foreach \a in {center, east, north, west, south, south east, south west, north east, north west}
    {
        \inheritanchor[from=circle]{\a}
    }
    \backgroundpath{
        \pgfpathcircle{\centerpoint}{\radius}
        \pgf@process{\centerpoint}
        \pgf@xa = \pgf@x
        \pgf@ya = \pgf@y
        \pgfpathmoveto{\pgfpoint{\pgf@xa-\radius}{\pgf@ya-\radius}}
        \pgfpathlineto{\pgfpoint{\pgf@xa+\radius}{\pgf@ya+\radius}}
    }
}
\pgfdeclareshape{macromoleculemultimer}{

    \inheritsavedanchors[from=rectangle] % this is nearly a rectangle

    \savedmacro{\scarceratio}{\def\scarceratio{0.15}}

    \savedmacro{\offsetratio}{\def\offsetratio{0.1}}

    \savedmacro\computecoordinates{%
        \pgf@yb = \ht\pgfnodeparttextbox
        \advance\pgf@yb by \dp\pgfnodeparttextbox
        \pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/pgf/inner ysep}}
        \advance\pgf@yb by 2\pgf@xa
        \pgfmathsetlength{\pgf@yb}{\pgf@yb/(1-\offsetratio)}
        \pgf@yc=\pgfkeysvalueof{/pgf/minimum height}
        \ifdim\pgf@yc>\pgf@yb
            \pgf@yb=\pgf@yc
        \fi
        \pgfmathsetlengthmacro\offset{\offsetratio*\pgf@yb}
        \addtosavedmacro\offset
        \pgf@xb=\wd\pgfnodeparttextbox
        \pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/pgf/inner xsep}}
        \advance\pgf@xb by 2\pgf@xa
        \pgf@xc=\pgfkeysvalueof{/pgf/minimum width}
        \advance\pgf@xb by \offset
        \ifdim\pgf@xc>\pgf@xb
            \pgf@xb=\pgf@xc
        \fi
        % \pgfmathsetlength{\pgf@xb}{\pgf@xb -0.5*\offset}
        \advance\pgf@xb by -\offset
        \advance\pgf@yb by -\offset
        \ifdim\pgf@yb>\pgf@xb
            \pgfmathsetlengthmacro\scarceoffset{\scarceratio*\pgf@xb}
        \else
            \pgfmathsetlengthmacro\scarceoffset{\scarceratio*\pgf@yb}
        \fi
        \addtosavedmacro\scarceoffset
        \pgf@xa=-0.5\pgf@xb
        \advance\pgf@xa by 0.5\wd\pgfnodeparttextbox
        \pgfmathsetlength{\pgf@xa}{\pgf@xa - 0.5*\offset}
        \pgf@xc=\pgf@xa %saving for later
        \pgf@ya=0.5\pgf@yb
        \advance\pgf@ya by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@ya by -0.5\dp\pgfnodeparttextbox
        \pgfmathsetlength{\pgf@ya}{\pgf@ya + 0.5*\offset}
        \advance\pgf@ya by -\scarceoffset
        \pgfextract@process\upperwestnorthjoin{\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}
        \addtosavedmacro{\upperwestnorthjoin}
        \advance\pgf@ya by \scarceoffset
        \advance\pgf@xa by \scarceoffset
        \pgfextract@process\uppernorthwestjoin{\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}
        \addtosavedmacro{\uppernorthwestjoin}
        \advance\pgf@xa by \pgf@xb
        \pgfmathaddtolength{\pgf@xa}{-2*\scarceoffset}
        \pgfextract@process\uppernortheastjoin{\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}
        \addtosavedmacro{\uppernortheastjoin}
        \advance\pgf@ya by -\scarceoffset
        \advance\pgf@xa by \scarceoffset
        \pgfextract@process\uppereastnorthjoin{\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}
        \addtosavedmacro{\uppereastnorthjoin}
        \advance\pgf@ya by -\pgf@yb
        \pgfmathaddtolength{\pgf@ya}{2*\scarceoffset}
        \pgfextract@process\uppereastsouthjoin{\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}
        \addtosavedmacro{\uppereastsouthjoin}
        \advance\pgf@ya by -\scarceoffset
        \advance\pgf@xa by -\scarceoffset
        \pgfextract@process\uppersoutheastjoin{\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}
        \addtosavedmacro{\uppersoutheastjoin}
        \pgf@xa=\pgf@xc
        \advance\pgf@xa by \scarceoffset
        \pgfextract@process\uppersouthwestjoin{\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}
        \addtosavedmacro{\uppersouthwestjoin}
        \advance\pgf@xa by -\scarceoffset
        \advance\pgf@ya by \scarceoffset
        \pgfextract@process\upperwestsouthjoin{\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}
        \addtosavedmacro{\upperwestsouthjoin}
        \upperwestnorthjoin
        \advance\pgf@x by \offset
        \advance\pgf@y by -\offset
        \pgfextract@process\lowerwestnorthjoin{\pgfpoint{\the\pgf@x}{\the\pgf@y}}
        \addtosavedmacro{\lowerwestnorthjoin}
        \uppernorthwestjoin
        \advance\pgf@x by \offset
        \advance\pgf@y by -\offset
        \pgfextract@process\lowernorthwestjoin{\pgfpoint{\the\pgf@x}{\the\pgf@y}}
        \addtosavedmacro{\lowernorthwestjoin}
        \uppernortheastjoin
        \advance\pgf@x by \offset
        \advance\pgf@y by -\offset
        \pgfextract@process\lowernortheastjoin{\pgfpoint{\the\pgf@x}{\the\pgf@y}}
        \addtosavedmacro{\lowernortheastjoin}
        \uppereastnorthjoin
        \advance\pgf@x by \offset
        \advance\pgf@y by -\offset
        \pgfextract@process\lowereastnorthjoin{\pgfpoint{\the\pgf@x}{\the\pgf@y}}
        \addtosavedmacro{\lowereastnorthjoin}
        \uppereastsouthjoin
        \advance\pgf@x by \offset
        \advance\pgf@y by -\offset
        \pgfextract@process\lowereastsouthjoin{\pgfpoint{\the\pgf@x}{\the\pgf@y}}
        \addtosavedmacro{\lowereastsouthjoin}
        \uppersoutheastjoin
        \advance\pgf@x by \offset
        \advance\pgf@y by -\offset
        \pgfextract@process\lowersoutheastjoin{\pgfpoint{\the\pgf@x}{\the\pgf@y}}
        \addtosavedmacro{\lowersoutheastjoin}
        \uppersouthwestjoin
        \advance\pgf@x by \offset
        \advance\pgf@y by -\offset
        \pgfextract@process\lowersouthwestjoin{\pgfpoint{\the\pgf@x}{\the\pgf@y}}
        \addtosavedmacro{\lowersouthwestjoin}
        \upperwestsouthjoin
        \advance\pgf@x by \offset
        \advance\pgf@y by -\offset
        \pgfextract@process\lowerwestsouthjoin{\pgfpoint{\the\pgf@x}{\the\pgf@y}}
        \addtosavedmacro{\lowerwestsouthjoin}
        \pgf@xa=\offset
        \pgf@xb=\scarceoffset\relax
        \ifdim\pgf@xa>\pgf@xb
            \lowerwestsouthjoin
            \pgf@xc=\pgf@x
            \uppersouthwestjoin
            \pgfextract@process\leftintersection{\pgfpoint{\the\pgf@xc}{\the\pgf@y}}
            \addtosavedmacro{\leftintersection}
            \uppereastnorthjoin
            \pgf@xc=\pgf@x
            \lowernortheastjoin
            \pgfextract@process\rightintersection{\pgfpoint{\the\pgf@xc}{\the\pgf@y}}
            \addtosavedmacro{\rightintersection}
        \else
            \upperwestsouthjoin
            \advance\pgf@x by \scarceoffset
            \pgfextract@process\uppersouthwestcenter{\pgfpoint{\the\pgf@x}{\the\pgf@y}}
            \addtosavedmacro{\uppersouthwestcenter}
            \advance\pgf@x by \offset
            \advance\pgf@y by -\offset
            \pgfextract@process\lowersouthwestcenter{\pgfpoint{\the\pgf@x}{\the\pgf@y}}
            \addtosavedmacro{\lowersouthwestcenter}
            \uppernortheastjoin
            \advance\pgf@y by -\scarceoffset
            \pgfextract@process\uppernortheastcenter{\pgfpoint{\the\pgf@x}{\the\pgf@y}}
            \addtosavedmacro{\uppernortheastcenter}
            \advance\pgf@x by \offset
            \advance\pgf@y by -\offset
            \pgfextract@process\lowernortheastcenter{\pgfpoint{\the\pgf@x}{\the\pgf@y}}
            \addtosavedmacro{\lowernortheastcenter}
            % \uppersouthwestjoin
            % \pgf@yc=\pgf@y
            \pgf@process{\pgfpointintersectionofcircles{\uppersouthwestcenter}{\lowersouthwestcenter}{\scarceoffset}{\scarceoffset}{1}}
            \pgfextract@process\leftintersection{\pgfpoint{\the\pgf@x}{\the\pgf@y}}
            \addtosavedmacro{\leftintersection}
            \pgf@process{\pgfpointintersectionofcircles{\uppernortheastcenter}{\lowernortheastcenter}{\scarceoffset}{\scarceoffset}{2}}
            \pgfextract@process\rightintersection{\pgfpoint{\the\pgf@x}{\the\pgf@y}}
            \addtosavedmacro{\rightintersection}
        \fi
    }

    \inheritanchorborder[from=rectangle]

    \foreach \a in {center, north, south, west, east, south east, south west, north east, north west}
    {
        \inheritanchor[from=rectangle]{\a}
    }

    \backgroundpath{
        \computecoordinates
        \pgfpathmoveto{\uppernorthwestjoin}
        \pgfpathlineto{\uppernortheastjoin}
        \pgfpatharc{90}{0}{\scarceoffset}
        \pgfpathlineto{\uppereastsouthjoin}
        \pgfpatharc{0}{-90}{\scarceoffset}
        \pgfpathlineto{\uppersouthwestjoin}
        \pgfpatharc{-90}{-180}{\scarceoffset}
        \pgfpathlineto{\upperwestnorthjoin}
        \pgfpatharc{-180}{-270}{\scarceoffset}
        \pgfpathclose

        \pgf@xa=\offset
        \pgf@xb=\scarceoffset
        \ifdim\pgf@xa>\pgf@xb
            \pgfpathmoveto{\leftintersection}
            \pgfpathlineto{\uppersoutheastjoin}
            \pgfpatharc{-90}{0}{\scarceoffset}
            \pgfpathlineto{\rightintersection}
            \pgfpathlineto{\lowernortheastjoin}
            \pgfpatharc{90}{0}{\scarceoffset}
            \pgfpathlineto{\lowereastsouthjoin}
            \pgfpatharc{0}{-90}{\scarceoffset}
            \pgfpathlineto{\lowersouthwestjoin}
            \pgfpatharc{-90}{-180}{\scarceoffset}
            \pgfpathclose
        \else
            \pgfpathmoveto{\uppersouthwestjoin}
            \pgfpathlineto{\uppersoutheastjoin}
            \pgfpatharc{-90}{0}{\scarceoffset}
            \pgfpathlineto{\uppereastnorthjoin}
            \rightintersection
            \pgf@ya=\pgf@y
            \pgf@process{\circlefindangle{\uppernortheastcenter}{\scarceoffset}{\pgf@ya}{2}}
            \pgfpatharc{0}{\pgf@x}{\scarceoffset}
            \circlefindangle{\lowernortheastcenter}{\scarceoffset}{\pgf@ya}{2}
            \pgfpatharc{\pgf@x}{0}{\scarceoffset}
            \pgfpathlineto{\lowereastsouthjoin}
            \pgfpatharc{0}{-90}{\scarceoffset}
            \pgfpathlineto{\lowersouthwestjoin}
            \leftintersection
            \pgf@ya=\pgf@y
            \pgf@process{\circlefindangle{\lowersouthwestcenter}{\scarceoffset}{\pgf@ya}{1}}
            \pgfpatharc{-90}{\pgf@x}{\scarceoffset}
            \pgf@process{\circlefindangle{\uppersouthwestcenter}{\scarceoffset}{\pgf@ya}{1}}
            \pgfpatharc{\pgf@x}{-90}{\scarceoffset}
            \pgfpathclose
        \fi
    }

    \foregroundpath{
        \pgfkeysgetvalue{/pgf/clone}{\clone}
        \ifx\clone\true
            \def\cloneoffsetratio{0.25}
            \computecoordinates
            \uppernorthwestjoin
            \pgf@ya=\pgf@y
            \lowersouthwestjoin
            \advance\pgf@ya by -\pgf@y
            \newdimen\cloneoffset
            \pgfmathsetlength{\cloneoffset}{(\cloneoffsetratio - \offsetratio)* \pgf@ya}
            \uppersouthwestjoin
            \pgf@yc=\pgf@y
            \upperwestsouthjoin
            \pgf@xc=\pgf@x
            \advance\pgf@yc by \cloneoffset
            \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \uppereastnorthjoin
            \pgf@xc=\pgf@x
            \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \lowersoutheastjoin
            \pgf@yc=\pgf@y
            \advance\pgf@yc by \cloneoffset
            \pgf@xb=\offset
            \advance\pgf@xb by \scarceoffset\relax
            \ifdim\cloneoffset>\pgf@xb
                \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \else
                \pgfpathlineto{\uppereastsouthjoin}
                \uppereastsouthjoin
                \advance\pgf@x by -\scarceoffset
                \pgf@process{\circlefindangle{\pgfpoint{\pgf@x}{\pgf@y}}{\scarceoffset}{\pgf@yc}{2}}
                \pgfpatharc{0}{\pgf@x}{\scarceoffset}
            \fi
            \lowereastsouthjoin
            \pgf@xc=\pgf@x
            \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \pgfpathlineto{\lowereastsouthjoin}
            \pgfpatharc{0}{-90}{\scarceoffset}
            \pgfpathlineto{\lowersouthwestjoin}
            \pgf@xa=\offset
            \pgf@xb=\scarceoffset\relax
            \ifdim\pgf@xa>\pgf@xb
                \pgfpatharc{-90}{-180}{\scarceoffset}
                \pgfpathlineto{\leftintersection}
                \pgfpathlineto{\uppersouthwestjoin}
                \pgfpatharc{-90}{-180}{\scarceoffset}
            \else
                \leftintersection
                \pgf@yc=\pgf@y
                \pgf@process{\circlefindangle{\lowersouthwestcenter}{\scarceoffset}{\pgf@yc}{1}}
                \pgfpatharc{-90}{\pgf@x}{\scarceoffset}
                \pgf@process{\circlefindangle{\uppersouthwestcenter}{\scarceoffset}{\pgf@yc}{1}}
                \pgfpatharc{\pgf@x}{-180}{\scarceoffset}
            \fi
            \pgfpathclose
            \pgfsetfillcolor{\tikz@strokecolor}
            \pgfusepath{fill, stroke}
        \fi
    }
}
\pgfdeclareshape{perturbation}{
    \inheritsavedanchors[from=rectangle] % this is nearly a rectangle
    \inheritanchorborder[from=rectangle]

    \foreach \a in {center, north, south, west, east, south east, south west, north east, north west}
    {
        \inheritanchor[from=rectangle]{\a}
    }

    \backgroundpath{
        \pgf@process{\southwest}
        \pgfgetlastxy{\xa}{\ya}
        \pgf@process{\northeast}
        \pgfgetlastxy{\xb}{\yb}
        \pgf@xc = \xa \pgf@yc = \yb
        \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc}}
        \pgf@xc = \xb
        \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
        \pgfmathsetlength{\pgf@yc}{\ya+0.5*(\yb-\ya)}
        \pgfmathsetlength{\pgf@xc}{\xb-0.20*(\xb-\xa)}
        \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
        \pgf@xc = \xb \pgf@yc = \ya
        \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
        \pgf@xc = \xa \pgf@yc = \ya
        \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
        \pgfmathsetlength{\pgf@yc}{\ya+0.5*(\yb-\ya)}
        \pgfmathsetlength{\pgf@xc}{\xa+0.20*(\xb-\xa)}
        \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
        \pgfclosepath
    }
}
\pgfdeclareshape{nucleicacidfeaturemultimer}{

    \inheritsavedanchors[from=rectangle] % this is nearly a rectangle

    \savedmacro{\scarceratio}{\def\scarceratio{0.15}}

    \savedmacro{\offsetratio}{\def\offsetratio{0.1}}

    \savedmacro\computecoordinates{%
        \pgf@yb = \ht\pgfnodeparttextbox
        \advance\pgf@yb by \dp\pgfnodeparttextbox
        \pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/pgf/inner ysep}}
        \advance\pgf@yb by 2\pgf@xa
        \pgfmathsetlength{\pgf@yb}{\pgf@yb/(1-\offsetratio)}
        \pgf@yc=\pgfkeysvalueof{/pgf/minimum height}
        \ifdim\pgf@yc>\pgf@yb
            \pgf@yb=\pgf@yc
        \fi
        \pgfmathsetlengthmacro\offset{\offsetratio*\pgf@yb}
        \addtosavedmacro\offset
        \pgf@xb=\wd\pgfnodeparttextbox
        \pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/pgf/inner xsep}}
        \advance\pgf@xb by 2\pgf@xa
        \pgf@xc=\pgfkeysvalueof{/pgf/minimum width}
        \advance\pgf@xb by \offset
        \ifdim\pgf@xc>\pgf@xb
            \pgf@xb=\pgf@xc
        \fi
        \advance\pgf@xb by -\offset
        \advance\pgf@yb by -\offset
        \ifdim\pgf@yb>\pgf@xb
            \pgfmathsetlengthmacro\scarceoffset{\scarceratio*\pgf@xb}
        \else
            \pgfmathsetlengthmacro\scarceoffset{\scarceratio*\pgf@yb}
        \fi
        \addtosavedmacro\scarceoffset
        \pgf@xa=-0.5\pgf@xb
        \advance\pgf@xa by 0.5\wd\pgfnodeparttextbox
        \pgf@xc=\pgf@xa %saving for later
        \pgf@ya=0.5\pgf@yb
        \advance\pgf@ya by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@ya by -0.5\dp\pgfnodeparttextbox
        \pgfextract@process\uppernorthwest{\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}
        \addtosavedmacro{\uppernorthwest}
        \advance\pgf@xa by \pgf@xb
        \pgfextract@process\uppernortheast{\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}
        \addtosavedmacro{\uppernortheast}
        \advance\pgf@ya by -\pgf@yb
        \advance\pgf@ya by \scarceoffset
        \pgfextract@process\uppereastsouthjoin{\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}
        \addtosavedmacro{\uppereastsouthjoin}
        \advance\pgf@ya by -\scarceoffset
        \advance\pgf@xa by -\scarceoffset
        \pgfextract@process\uppersoutheastjoin{\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}
        \addtosavedmacro{\uppersoutheastjoin}
        \pgf@xa=\pgf@xc
        \advance\pgf@xa by \scarceoffset
        \pgfextract@process\uppersouthwestjoin{\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}
        \addtosavedmacro{\uppersouthwestjoin}
        \advance\pgf@xa by -\scarceoffset
        \advance\pgf@ya by \scarceoffset
        \pgfextract@process\upperwestsouthjoin{\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}
        \addtosavedmacro{\upperwestsouthjoin}
        \uppernorthwest
        \advance\pgf@x by \offset
        \advance\pgf@y by -\offset
        \pgfextract@process\lowernorthwest{\pgfpoint{\the\pgf@x}{\the\pgf@y}}
        \uppernortheast
        \advance\pgf@x by \offset
        \advance\pgf@y by -\offset
        \pgfextract@process\lowernortheast{\pgfpoint{\the\pgf@x}{\the\pgf@y}}
        \addtosavedmacro{\lowernortheast}
        \uppereastsouthjoin
        \addtosavedmacro{\lowernorthwest}
        \uppereastsouthjoin
        \advance\pgf@x by \offset
        \advance\pgf@y by -\offset
        \pgfextract@process\lowereastsouthjoin{\pgfpoint{\the\pgf@x}{\the\pgf@y}}
        \addtosavedmacro{\lowereastsouthjoin}
        \uppersoutheastjoin
        \advance\pgf@x by \offset
        \advance\pgf@y by -\offset
        \pgfextract@process\lowersoutheastjoin{\pgfpoint{\the\pgf@x}{\the\pgf@y}}
        \addtosavedmacro{\lowersoutheastjoin}
        \uppersouthwestjoin
        \advance\pgf@x by \offset
        \advance\pgf@y by -\offset
        \pgfextract@process\lowersouthwestjoin{\pgfpoint{\the\pgf@x}{\the\pgf@y}}
        \addtosavedmacro{\lowersouthwestjoin}
        \upperwestsouthjoin
        \advance\pgf@x by \offset
        \advance\pgf@y by -\offset
        \pgfextract@process\lowerwestsouthjoin{\pgfpoint{\the\pgf@x}{\the\pgf@y}}
        \addtosavedmacro{\lowerwestsouthjoin}
        \pgf@xa=\offset
        \pgf@xb=\scarceoffset\relax
        \uppernortheast
        \pgf@xc=\pgf@x
        \lowernortheast
        \pgfextract@process\rightintersection{\pgfpoint{\the\pgf@xc}{\the\pgf@y}}
        \addtosavedmacro{\rightintersection}
        \ifdim\pgf@xa>\pgf@xb
            \lowerwestsouthjoin
            \pgf@xc=\pgf@x
            \uppersouthwestjoin
            \pgfextract@process\leftintersection{\pgfpoint{\the\pgf@xc}{\the\pgf@y}}
            \addtosavedmacro{\leftintersection}
        \else
            \upperwestsouthjoin
            \advance\pgf@x by \scarceoffset
            \pgfextract@process\uppersouthwestcenter{\pgfpoint{\the\pgf@x}{\the\pgf@y}}
            \addtosavedmacro{\uppersouthwestcenter}
            \advance\pgf@x by \offset
            \advance\pgf@y by -\offset
            \pgfextract@process\lowersouthwestcenter{\pgfpoint{\the\pgf@x}{\the\pgf@y}}
            \addtosavedmacro{\lowersouthwestcenter}
            \pgf@process{\pgfpointintersectionofcircles{\uppersouthwestcenter}{\lowersouthwestcenter}{\scarceoffset}{\scarceoffset}{1}}
            \pgfextract@process\leftintersection{\pgfpoint{\the\pgf@x}{\the\pgf@y}}
            \addtosavedmacro{\leftintersection}
        \fi
    }

    \inheritanchorborder[from=rectangle]

    \foreach \a in {center, north, south, west, east, south east, south west, north east, north west}
    {
        \inheritanchor[from=rectangle]{\a}
    }

    \backgroundpath{
        \computecoordinates
        \pgfpathmoveto{\uppernorthwest}
        \pgfpathlineto{\uppernortheast}
        \pgfpathlineto{\uppereastsouthjoin}
        \pgfpatharc{0}{-90}{\scarceoffset}
        \pgfpathlineto{\uppersouthwestjoin}
        \pgfpatharc{-90}{-180}{\scarceoffset}
        \pgfpathclose

        \pgf@xa=\offset
        \pgf@xb=\scarceoffset
        \ifdim\pgf@xa>\pgf@xb
            \pgfpathmoveto{\leftintersection}
            \pgfpathlineto{\uppersoutheastjoin}
            \pgfpatharc{-90}{0}{\scarceoffset}
            \pgfpathlineto{\rightintersection}
            \pgfpathlineto{\lowernortheast}
            \pgfpathlineto{\lowereastsouthjoin}
            \pgfpatharc{0}{-90}{\scarceoffset}
            \pgfpathlineto{\lowersouthwestjoin}
            \pgfpatharc{-90}{-180}{\scarceoffset}
            \pgfpathclose
        \else
            \pgfpathmoveto{\uppersouthwestjoin}
            \pgfpathlineto{\uppersoutheastjoin}
            \pgfpatharc{-90}{0}{\scarceoffset}
            \pgfpathlineto{\rightintersection}
            \pgfpathlineto{\lowernortheast}
            \pgfpathlineto{\lowereastsouthjoin}
            \pgfpatharc{0}{-90}{\scarceoffset}
            \pgfpathlineto{\lowersouthwestjoin}
            \leftintersection
            \pgf@ya=\pgf@y
            \pgf@process{\circlefindangle{\lowersouthwestcenter}{\scarceoffset}{\pgf@ya}{1}}
            \pgfpatharc{-90}{\pgf@x}{\scarceoffset}
            \pgf@process{\circlefindangle{\uppersouthwestcenter}{\scarceoffset}{\pgf@ya}{1}}
            \pgfpatharc{\pgf@x}{-90}{\scarceoffset}
            \pgfpathclose
        \fi
    }

    \foregroundpath{
        \pgfkeysgetvalue{/pgf/clone}{\clone}
        \ifx\clone\true
            \def\cloneoffsetratio{0.25}
            \computecoordinates
            \uppernorthwest
            \pgf@xc=\pgf@x
            \pgf@ya=\pgf@y
            \uppersouthwestjoin
            \advance\pgf@ya by -\pgf@y
            \newdimen\cloneoffset
            \cloneoffset=\cloneoffsetratio\pgf@ya
            \pgf@yc=\pgf@y
            \advance\pgf@yc by \cloneoffset
            \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \uppernortheast
            \pgf@xc=\pgf@x
            \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \lowersoutheastjoin
            \pgf@yc=\pgf@y
            \advance\pgf@yc by \cloneoffset
            \pgf@xb=\offset
            \advance\pgf@xb by \scarceoffset\relax
            \ifdim\cloneoffset>\pgf@xb
                \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \else
                \pgfpathlineto{\uppereastsouthjoin}
                \uppereastsouthjoin
                \advance\pgf@x by -\scarceoffset
                \pgf@process{\circlefindangle{\pgfpoint{\pgf@x}{\pgf@y}}{\scarceoffset}{\pgf@yc}{2}}
                \pgfpatharc{0}{\pgf@x}{\scarceoffset}
            \fi
            \lowereastsouthjoin
            \pgf@xc=\pgf@x
            \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \pgfpathlineto{\lowereastsouthjoin}
            \pgfpatharc{0}{-90}{\scarceoffset}
            \pgfpathlineto{\lowersouthwestjoin}
            \pgf@xa=\offset
            \pgf@xb=\scarceoffset\relax
            \ifdim\pgf@xa>\pgf@xb
                \pgfpatharc{-90}{-180}{\scarceoffset}
                \pgfpathlineto{\leftintersection}
                \pgfpathlineto{\uppersouthwestjoin}
                \pgfpatharc{-90}{-180}{\scarceoffset}
            \else
                \leftintersection
                \pgf@yc=\pgf@y
                \pgf@process{\circlefindangle{\lowersouthwestcenter}{\scarceoffset}{\pgf@yc}{1}}
                \pgfpatharc{-90}{\pgf@x}{\scarceoffset}
                \pgf@process{\circlefindangle{\uppersouthwestcenter}{\scarceoffset}{\pgf@yc}{1}}
                \pgfpatharc{\pgf@x}{-180}{\scarceoffset}
            \fi
            \pgfpathclose
            \pgfsetfillcolor{\tikz@strokecolor}
            \pgfusepath{fill, stroke}
        \fi
   }
}
%Copyright 2018 by Adrien Rougny
%This file may be distributed and/or modified under the terms of the GNU General Public License version 3
%See the file LICENSE.txt
\pgfdeclareshape{genericprocess}{
    % \savedmacro\lanchor{0.75}
    \inheritsavedanchors[from=rectangle]
    \inheritanchorborder[from=rectangle]
    \foreach \a in {center, south east, south west, north east, north west}
    {
        \inheritanchor[from=rectangle]{\a}
    }

    \savedanchor\connectoreast{
        \pgfkeysgetvalue{/pgf/connectors}{\connectors}
        %compute width and height without taking into account outer sep
        \pgf@x=\wd\pgfnodeparttextbox
        \pgf@xc=\pgfkeysvalueof{/pgf/inner xsep}
        \advance\pgf@x by 2\pgf@xc
        \pgf@xc=\pgfkeysvalueof{/pgf/minimum width}
        \ifdim\pgf@xc>\pgf@x
            \pgf@x=\pgf@xc
        \fi
        \pgf@y=\ht\pgfnodeparttextbox
        \advance\pgf@y by \dp\pgfnodeparttextbox
        \pgf@yc=\pgfkeysvalueof{/pgf/inner ysep}
        \advance\pgf@y by 2\pgf@yc
        \pgf@yc=\pgfkeysvalueof{/pgf/minimum height}
        \ifdim\pgf@yc>\pgf@y
            \pgf@y=\pgf@yc
        \fi
        %store south west in xa,ya and north east in xb,yb
        \pgf@xa=-0.5\pgf@x
        \advance\pgf@xa by 0.5\wd\pgfnodeparttextbox
        \pgf@ya=-0.5\pgf@y
        \advance\pgf@ya by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@ya by -0.5\dp\pgfnodeparttextbox
        \pgf@xb=0.5\pgf@x
        \advance\pgf@xb by 0.5\wd\pgfnodeparttextbox
        \pgf@yb=0.5\pgf@y
        \advance\pgf@yb by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@yb by -0.5\dp\pgfnodeparttextbox
        %compute anchor
        \pgf@y=0.5\pgf@yb
        \advance\pgf@y by 0.5\pgf@ya
        \pgf@x=\pgf@xb
        \ifx\connectors\horizontal
            \pgfkeysgetvalue{/pgf/right connector length}{\lconnector}
            \advance\pgf@x by \lconnector
        \fi
    }

    \savedanchor\connectorwest{
        \pgfkeysgetvalue{/pgf/connectors}{\connectors}
        %compute width and height without taking into account outer sep
        \pgf@x=\wd\pgfnodeparttextbox
        \pgf@xc=\pgfkeysvalueof{/pgf/inner xsep}
        \advance\pgf@x by 2\pgf@xc
        \pgf@xc=\pgfkeysvalueof{/pgf/minimum width}
        \ifdim\pgf@xc>\pgf@x
            \pgf@x=\pgf@xc
        \fi
        \pgf@y=\ht\pgfnodeparttextbox
        \advance\pgf@y by \dp\pgfnodeparttextbox
        \pgf@yc=\pgfkeysvalueof{/pgf/inner ysep}
        \advance\pgf@y by 2\pgf@yc
        \pgf@yc=\pgfkeysvalueof{/pgf/minimum height}
        \ifdim\pgf@yc>\pgf@y
            \pgf@y=\pgf@yc
        \fi
        %store south west in xa,ya and north east in xb,yb
        \pgf@xa=-0.5\pgf@x
        \advance\pgf@xa by 0.5\wd\pgfnodeparttextbox
        \pgf@ya=-0.5\pgf@y
        \advance\pgf@ya by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@ya by -0.5\dp\pgfnodeparttextbox
        \pgf@xb=0.5\pgf@x
        \advance\pgf@xb by 0.5\wd\pgfnodeparttextbox
        \pgf@yb=0.5\pgf@y
        \advance\pgf@yb by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@yb by -0.5\dp\pgfnodeparttextbox
        %compute anchor
        \pgf@y=0.5\pgf@yb
        \advance\pgf@y by 0.5\pgf@ya
        \pgf@x=\pgf@xa
        \ifx\connectors\horizontal
            \pgfkeysgetvalue{/pgf/left connector length}{\lconnector}
            \advance\pgf@x by -\lconnector
        \fi
    }

    \savedanchor\connectornorth{
        \pgfkeysgetvalue{/pgf/connectors}{\connectors}
        %compute width and height without taking into account outer sep
        \pgf@x=\wd\pgfnodeparttextbox
        \pgf@xc=\pgfkeysvalueof{/pgf/inner xsep}
        \advance\pgf@x by 2\pgf@xc
        \pgf@xc=\pgfkeysvalueof{/pgf/minimum width}
        \ifdim\pgf@xc>\pgf@x
            \pgf@x=\pgf@xc
        \fi
        \pgf@y=\ht\pgfnodeparttextbox
        \advance\pgf@y by \dp\pgfnodeparttextbox
        \pgf@yc=\pgfkeysvalueof{/pgf/inner ysep}
        \advance\pgf@y by 2\pgf@yc
        \pgf@yc=\pgfkeysvalueof{/pgf/minimum height}
        \ifdim\pgf@yc>\pgf@y
            \pgf@y=\pgf@yc
        \fi
        %store south west in xa,ya and north east in xb,yb
        \pgf@xa=-0.5\pgf@x
        \advance\pgf@xa by 0.5\wd\pgfnodeparttextbox
        \pgf@ya=-0.5\pgf@y
        \advance\pgf@ya by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@ya by -0.5\dp\pgfnodeparttextbox
        \pgf@xb=0.5\pgf@x
        \advance\pgf@xb by 0.5\wd\pgfnodeparttextbox
        \pgf@yb=0.5\pgf@y
        \advance\pgf@yb by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@yb by -0.5\dp\pgfnodeparttextbox
        %compute anchor
        \pgf@x=0.5\pgf@xb
        \advance\pgf@x by 0.5\pgf@xa
        \pgf@y=\pgf@yb
        \ifx\connectors\vertical
            \pgfkeysgetvalue{/pgf/left connector length}{\lconnector}
            \advance\pgf@y by \lconnector
        \fi
    }

    \savedanchor\connectorsouth{
        \pgfkeysgetvalue{/pgf/connectors}{\connectors}
        %compute width and height without taking into account outer sep
        \pgf@x=\wd\pgfnodeparttextbox
        \pgf@xc=\pgfkeysvalueof{/pgf/inner xsep}
        \advance\pgf@x by 2\pgf@xc
        \pgf@xc=\pgfkeysvalueof{/pgf/minimum width}
        \ifdim\pgf@xc>\pgf@x
            \pgf@x=\pgf@xc
        \fi
        \pgf@y=\ht\pgfnodeparttextbox
        \advance\pgf@y by \dp\pgfnodeparttextbox
        \pgf@yc=\pgfkeysvalueof{/pgf/inner ysep}
        \advance\pgf@y by 2\pgf@yc
        \pgf@yc=\pgfkeysvalueof{/pgf/minimum height}
        \ifdim\pgf@yc>\pgf@y
            \pgf@y=\pgf@yc
        \fi
        %store south west in xa,ya and north east in xb,yb
        \pgf@xa=-0.5\pgf@x
        \advance\pgf@xa by 0.5\wd\pgfnodeparttextbox
        \pgf@ya=-0.5\pgf@y
        \advance\pgf@ya by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@ya by -0.5\dp\pgfnodeparttextbox
        \pgf@xb=0.5\pgf@x
        \advance\pgf@xb by 0.5\wd\pgfnodeparttextbox
        \pgf@yb=0.5\pgf@y
        \advance\pgf@yb by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@yb by -0.5\dp\pgfnodeparttextbox
        %compute anchor
        \pgf@x=0.5\pgf@xb
        \advance\pgf@x by 0.5\pgf@xa
        \pgf@y=\pgf@ya
        \ifx\connectors\vertical
            \pgfkeysgetvalue{/pgf/right connector length}{\lconnector}
            \advance\pgf@y by -\lconnector
        \fi
    }

    \anchor{west}{\connectorwest}
    \anchor{east}{\connectoreast}
    \anchor{north}{\connectornorth}
    \anchor{south}{\connectorsouth}

    \backgroundpath{
        \pgfpathrectanglecorners{\southwest}{\northeast}
        \pgfkeysgetvalue{/pgf/connectors}{\connectors}
        \ifx\connectors\horizontal
            \pgfkeysgetvalue{/pgf/left connector length}{\lconnector}
            \pgfkeysgetvalue{/pgf/right connector length}{\rconnector}
            \pgf@process{\southwest}
            \pgf@xa = \pgf@x
            \pgf@ya = \pgf@y
            \pgf@process{\northeast}
            \pgf@xb = \pgf@x
            \pgf@yb = \pgf@y
            \pgf@xc=\pgf@x
            \pgf@yc=\pgf@y
            \advance\pgf@yc by -0.5\pgf@yb
            \advance\pgf@yc by 0.5\pgf@ya
            \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@xc by \rconnector
            \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \pgf@xc=\pgf@xa
            \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@xc by -\lconnector
            \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
        \fi
        \ifx\connectors\vertical
            \pgfkeysgetvalue{/pgf/left connector length}{\lconnector}
            \pgfkeysgetvalue{/pgf/right connector length}{\rconnector}
            \pgf@process{\southwest}
            \pgf@xa = \pgf@x
            \pgf@ya = \pgf@y
            \pgf@process{\northeast}
            \pgf@xb = \pgf@x
            \pgf@yb = \pgf@y
            \pgf@xc=\pgf@x
            \pgf@yc=\pgf@y
            \advance\pgf@xc by -0.5\pgf@xb
            \advance\pgf@xc by 0.5\pgf@xa
            \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@yc by \rconnector
            \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \pgf@yc=\pgf@ya
            \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@yc by -\lconnector
            \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
        \fi
    }
}
\pgfdeclareshape{unspecifiedentity}{
    \inheritsavedanchors[from=ellipse]
    \inheritanchorborder[from=ellipse]
    \foreach \a in {center, south, north, east, west, south east, south west, north east, north west}
    {
        \inheritanchor[from=ellipse]{\a}
    }
    \inheritbackgroundpath[from=ellipse]
    \foregroundpath{
        \pgfkeysgetvalue{/pgf/clone}{\clone}
        \ifx\clone\true
            \def\cloneoffset{0.25}
            \newdimen\xa
            \newdimen\ya
            \pgf@process{\centerpoint}
            \xa=\pgf@x
            \ya=\pgf@y
            \newdimen\xb
            \newdimen\yb
            \pgf@process{\radius}
            \xb=\pgf@x
            \yb=\pgf@y
            \advance\xb by -0.5\pgflinewidth
            \advance\yb by -0.5\pgflinewidth
            \newdimen\yc
            \pgfmathsetlength{\yc}{-2*\cloneoffset)*\yb}
            \newdimen\xc
            \pgfmathsetlength{\xc}{sqrt(\xb^2-(\xb*\yc/\yb)^2)}
            \newdimen\anglea
            \pgfmathsetmacro{\anglea}{asin(\yc/\yb)}
            \newdimen\angleb
            \pgfmathsetlength{\angleb}{-180-\anglea}
            \pgf@xa = -\xc
            \advance\pgf@xa by \xa
            \pgf@xb = \xc
            \advance\pgf@xb by \xa
            \advance\yc by \ya
            \pgfpathmoveto{\pgfpoint{\pgf@xa}{\yc}}
            \pgfpathlineto{\pgfpoint{\pgf@xb}{\yc}}
            \pgfpatharc{\anglea}{\angleb}{\xb and \yb}
            \pgfpathclose
            \pgfsetfillcolor{\tikz@strokecolor}
            \pgfusepath{stroke, fill}
        \fi
    }
}
\pgfdeclareshape{association}{
    % \savedmacro\lanchor{0.75}
    \inheritsavedanchors[from=circle]
    \inheritanchorborder[from=circle]
    \foreach \a in {center, south east, south west, north east, north west}
    {
        \inheritanchor[from=circle]{\a}
    }

    \savedanchor\connectoreast{
        \pgfkeysgetvalue{/pgf/connectors}{\connectors}
        %compute width and height without taking into account outer sep
        \pgf@x=\wd\pgfnodeparttextbox
        \pgf@xc=\pgfkeysvalueof{/pgf/inner xsep}
        \advance\pgf@x by 2\pgf@xc
        \pgf@xc=\pgfkeysvalueof{/pgf/minimum width}
        \ifdim\pgf@xc>\pgf@x
            \pgf@x=\pgf@xc
        \fi
        \pgf@y=\ht\pgfnodeparttextbox
        \advance\pgf@y by \dp\pgfnodeparttextbox
        \pgf@yc=\pgfkeysvalueof{/pgf/inner ysep}
        \advance\pgf@y by 2\pgf@yc
        \pgf@yc=\pgfkeysvalueof{/pgf/minimum height}
        \ifdim\pgf@yc>\pgf@y
            \pgf@y=\pgf@yc
        \fi
        %store south west in xa,ya and north east in xb,yb
        \pgf@xa=-0.5\pgf@x
        \advance\pgf@xa by 0.5\wd\pgfnodeparttextbox
        \pgf@ya=-0.5\pgf@y
        \advance\pgf@ya by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@ya by -0.5\dp\pgfnodeparttextbox
        \pgf@xb=0.5\pgf@x
        \advance\pgf@xb by 0.5\wd\pgfnodeparttextbox
        \pgf@yb=0.5\pgf@y
        \advance\pgf@yb by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@yb by -0.5\dp\pgfnodeparttextbox
        %compute anchor
        \pgf@y=0.5\pgf@yb
        \advance\pgf@y by 0.5\pgf@ya
        \pgf@x=\pgf@xb
        \ifx\connectors\horizontal
            \pgfkeysgetvalue{/pgf/right connector length}{\lconnector}
            \advance\pgf@x by \lconnector
        \fi
    }

    \savedanchor\connectorwest{
        \pgfkeysgetvalue{/pgf/connectors}{\connectors}
        %compute width and height without taking into account outer sep
        \pgf@x=\wd\pgfnodeparttextbox
        \pgf@xc=\pgfkeysvalueof{/pgf/inner xsep}
        \advance\pgf@x by 2\pgf@xc
        \pgf@xc=\pgfkeysvalueof{/pgf/minimum width}
        \ifdim\pgf@xc>\pgf@x
            \pgf@x=\pgf@xc
        \fi
        \pgf@y=\ht\pgfnodeparttextbox
        \advance\pgf@y by \dp\pgfnodeparttextbox
        \pgf@yc=\pgfkeysvalueof{/pgf/inner ysep}
        \advance\pgf@y by 2\pgf@yc
        \pgf@yc=\pgfkeysvalueof{/pgf/minimum height}
        \ifdim\pgf@yc>\pgf@y
            \pgf@y=\pgf@yc
        \fi
        %store south west in xa,ya and north east in xb,yb
        \pgf@xa=-0.5\pgf@x
        \advance\pgf@xa by 0.5\wd\pgfnodeparttextbox
        \pgf@ya=-0.5\pgf@y
        \advance\pgf@ya by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@ya by -0.5\dp\pgfnodeparttextbox
        \pgf@xb=0.5\pgf@x
        \advance\pgf@xb by 0.5\wd\pgfnodeparttextbox
        \pgf@yb=0.5\pgf@y
        \advance\pgf@yb by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@yb by -0.5\dp\pgfnodeparttextbox
        %compute anchor
        \pgf@y=0.5\pgf@yb
        \advance\pgf@y by 0.5\pgf@ya
        \pgf@x=\pgf@xa
        \ifx\connectors\horizontal
            \pgfkeysgetvalue{/pgf/left connector length}{\lconnector}
            \advance\pgf@x by -\lconnector
        \fi
    }

    \savedanchor\connectornorth{
        \pgfkeysgetvalue{/pgf/connectors}{\connectors}
        %compute width and height without taking into account outer sep
        \pgf@x=\wd\pgfnodeparttextbox
        \pgf@xc=\pgfkeysvalueof{/pgf/inner xsep}
        \advance\pgf@x by 2\pgf@xc
        \pgf@xc=\pgfkeysvalueof{/pgf/minimum width}
        \ifdim\pgf@xc>\pgf@x
            \pgf@x=\pgf@xc
        \fi
        \pgf@y=\ht\pgfnodeparttextbox
        \advance\pgf@y by \dp\pgfnodeparttextbox
        \pgf@yc=\pgfkeysvalueof{/pgf/inner ysep}
        \advance\pgf@y by 2\pgf@yc
        \pgf@yc=\pgfkeysvalueof{/pgf/minimum height}
        \ifdim\pgf@yc>\pgf@y
            \pgf@y=\pgf@yc
        \fi
        %store south west in xa,ya and north east in xb,yb
        \pgf@xa=-0.5\pgf@x
        \advance\pgf@xa by 0.5\wd\pgfnodeparttextbox
        \pgf@ya=-0.5\pgf@y
        \advance\pgf@ya by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@ya by -0.5\dp\pgfnodeparttextbox
        \pgf@xb=0.5\pgf@x
        \advance\pgf@xb by 0.5\wd\pgfnodeparttextbox
        \pgf@yb=0.5\pgf@y
        \advance\pgf@yb by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@yb by -0.5\dp\pgfnodeparttextbox
        %compute anchor
        \pgf@x=0.5\pgf@xb
        \advance\pgf@x by 0.5\pgf@xa
        \pgf@y=\pgf@yb
        \ifx\connectors\vertical
            \pgfkeysgetvalue{/pgf/left connector length}{\lconnector}
            \advance\pgf@y by \lconnector
        \fi
    }

    \savedanchor\connectorsouth{
        \pgfkeysgetvalue{/pgf/connectors}{\connectors}
        %compute width and height without taking into account outer sep
        \pgf@x=\wd\pgfnodeparttextbox
        \pgf@xc=\pgfkeysvalueof{/pgf/inner xsep}
        \advance\pgf@x by 2\pgf@xc
        \pgf@xc=\pgfkeysvalueof{/pgf/minimum width}
        \ifdim\pgf@xc>\pgf@x
            \pgf@x=\pgf@xc
        \fi
        \pgf@y=\ht\pgfnodeparttextbox
        \advance\pgf@y by \dp\pgfnodeparttextbox
        \pgf@yc=\pgfkeysvalueof{/pgf/inner ysep}
        \advance\pgf@y by 2\pgf@yc
        \pgf@yc=\pgfkeysvalueof{/pgf/minimum height}
        \ifdim\pgf@yc>\pgf@y
            \pgf@y=\pgf@yc
        \fi
        %store south west in xa,ya and north east in xb,yb
        \pgf@xa=-0.5\pgf@x
        \advance\pgf@xa by 0.5\wd\pgfnodeparttextbox
        \pgf@ya=-0.5\pgf@y
        \advance\pgf@ya by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@ya by -0.5\dp\pgfnodeparttextbox
        \pgf@xb=0.5\pgf@x
        \advance\pgf@xb by 0.5\wd\pgfnodeparttextbox
        \pgf@yb=0.5\pgf@y
        \advance\pgf@yb by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@yb by -0.5\dp\pgfnodeparttextbox
        %compute anchor
        \pgf@x=0.5\pgf@xb
        \advance\pgf@x by 0.5\pgf@xa
        \pgf@y=\pgf@ya
        \ifx\connectors\vertical
            \pgfkeysgetvalue{/pgf/right connector length}{\lconnector}
            \advance\pgf@y by -\lconnector
        \fi
    }

    \anchor{west}{\connectorwest}
    \anchor{east}{\connectoreast}
    \anchor{north}{\connectornorth}
    \anchor{south}{\connectorsouth}

    \backgroundpath{
        \pgfpathcircle{\centerpoint}{\radius}
        \pgfkeysgetvalue{/pgf/connectors}{\connectors}
        \ifx\connectors\horizontal
            \pgfkeysgetvalue{/pgf/left connector length}{\lconnector}
            \pgfkeysgetvalue{/pgf/right connector length}{\rconnector}
            \pgf@process{\centerpoint}
            \pgf@xc=\pgf@x
            \pgf@yc=\pgf@y
            \pgf@xb = \radius
            \advance\pgf@xc by \pgf@xb
            \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@xc by \rconnector
            \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@xc by -\rconnector
            \advance\pgf@xc by -2\pgf@xb
            \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@xc by -\lconnector
            \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
        \fi
        \ifx\connectors\vertical
            \pgfkeysgetvalue{/pgf/left connector length}{\lconnector}
            \pgfkeysgetvalue{/pgf/right connector length}{\rconnector}
            \pgf@process{\centerpoint}
            \pgf@xc=\pgf@x
            \pgf@yc=\pgf@y
            \pgf@xb = \radius
            \advance\pgf@yc by \pgf@xb
            \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@yc by \lconnector
            \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@yc by -\lconnector
            \advance\pgf@yc by -2\pgf@xb
            \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@yc by -\rconnector
            \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
        \fi
    }
}
\pgfdeclareshape{tag}{

    \inheritsavedanchors[from=rectangle] % this is nearly a rectangle

    \savedmacro{\pointratio}{\def\pointratio{0.25}}

    \savedmacro\computecoordinates{%
        \pgfkeysgetvalue{/pgf/orientation}{\orientation}
        \pgf@yb = \ht\pgfnodeparttextbox
        \advance\pgf@yb by \dp\pgfnodeparttextbox
        \pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/pgf/inner ysep}}
        \advance\pgf@yb by 2\pgf@xa
        \ifx\orientation\oup
            \pgfmathsetlength{\pgf@yb}{\pgf@yb/(1-\pointratio)}
        \fi
        \ifx\orientation\odown
            \pgfmathsetlength{\pgf@yb}{\pgf@yb/(1-\pointratio)}
        \fi
        \pgf@yc=\pgfkeysvalueof{/pgf/minimum height}
        \ifdim\pgf@yc>\pgf@yb
            \pgf@yb=\pgf@yc
        \fi
        \ifx\orientation\oup
            \pgfmathsetlengthmacro\pointoffset{\pointratio*\pgf@yb}
        \fi
        \ifx\orientation\odown
            \pgfmathsetlengthmacro\pointoffset{\pointratio*\pgf@yb}
        \fi
        \pgf@xb = \wd\pgfnodeparttextbox
        \pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/pgf/inner xsep}}
        \advance\pgf@xb by 2\pgf@xa
        \ifx\orientation\oleft
            \pgfmathsetlength{\pgf@xb}{\pgf@xb/(1-\pointratio)}
        \fi
        \ifx\orientation\oright
            \pgfmathsetlength{\pgf@xb}{\pgf@xb/(1-\pointratio)}
        \fi
        \pgf@xc=\pgfkeysvalueof{/pgf/minimum width}
        \ifdim\pgf@xc>\pgf@xb
            \pgf@xb=\pgf@xc
        \fi
        \ifx\orientation\oleft
            \pgfmathsetlengthmacro\pointoffset{\pointratio*\pgf@xb}
        \fi
        \ifx\orientation\oright
            \pgfmathsetlengthmacro\pointoffset{\pointratio*\pgf@xb}
        \fi
        \addtosavedmacro\pointoffset
        \pgf@xa=-0.5\pgf@xb
        \ifx\orientation\oright
            \pgfmathaddtolength{\pgf@xa}{0.5*\pointoffset}
        \fi
        \ifx\orientation\oleft
            \pgfmathaddtolength{\pgf@xa}{0.5*\pointoffset}
        \fi
        \advance\pgf@xa by 0.5\wd\pgfnodeparttextbox
        \pgf@ya=-0.5\pgf@yb
        \advance\pgf@ya by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@ya by -0.5\dp\pgfnodeparttextbox
        \ifx\orientation\oup
            \pgfmathaddtolength{\pgf@ya}{0.5*\pointoffset}
        \fi
        \ifx\orientation\odown
            \pgfmathaddtolength{\pgf@ya}{0.5*\pointoffset}
        \fi
        \pgfextract@process\southwest{\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}
        \addtosavedmacro\southwest
        \advance\pgf@xa by \pgf@xb
        \ifx\orientation\oright
            \advance\pgf@xa by -\pointoffset
        \fi
        \ifx\orientation\oleft
            \advance\pgf@xa by -\pointoffset
        \fi
        \advance\pgf@ya by \pgf@yb
        \ifx\orientation\oup
            \advance\pgf@ya by -\pointoffset
        \fi
        \ifx\orientation\odown
            \advance\pgf@ya by -\pointoffset
        \fi
        \pgfextract@process\northeast{\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}
        \addtosavedmacro\northeast
        \ifx\orientation\oright
            \advance\pgf@ya by -0.5\pgf@yb
            \advance\pgf@xa by \pointoffset
        \fi
        \ifx\orientation\oleft
            \advance\pgf@ya by -0.5\pgf@yb
            \advance\pgf@xa by -\pgf@xb
        \fi
        \ifx\orientation\odown
            \advance\pgf@ya by -\pgf@yb
            \advance\pgf@xa by -0.5\pgf@xb
        \fi
        \ifx\orientation\oup
            \advance\pgf@ya by \pointoffset
            \advance\pgf@xa by -0.5\pgf@xb
        \fi
        \pgfextract@process\pointangle{\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}
        \addtosavedmacro\pointangle
    }

    \anchor{south west}{
        \computecoordinates
        \southwest
    }

    \anchor{north east}{
        \computecoordinates
        \northeast
    }

    \anchor{south east}{
        \computecoordinates
        \northeast
        \pgf@xa=\pgf@x
        \southwest
        \pgf@x=\pgf@xa
    }

    \anchor{north west}{
        \computecoordinates
        \northeast
        \pgf@ya=\pgf@y
        \southwest
        \pgf@y=\pgf@ya
    }

    \anchor{north}{
        \computecoordinates
        \pointangle
        \pgf@ya=\pgf@y
        \northeast
        \ifdim\pgf@ya>\pgf@y
            \pointangle
        \else
            \pgf@ya=\pgf@y
            \pgf@xa=0.5\pgf@x
            \southwest
            \advance\pgf@xa by 0.5\pgf@x
            \pgf@x=\pgf@xa
            \pgf@y=\pgf@ya
        \fi
    }

    \anchor{south}{
        \computecoordinates
        \pointangle
        \pgf@ya=\pgf@y
        \southwest
        \ifdim\pgf@ya<\pgf@y
            \pointangle
        \else
            \pgf@ya=\pgf@y
            \pgf@xa=0.5\pgf@x
            \northeast
            \advance\pgf@xa by 0.5\pgf@x
            \pgf@x=\pgf@xa
            \pgf@y=\pgf@ya
        \fi
    }

    \anchor{east}{
        \computecoordinates
        \pointangle
        \pgf@xa=\pgf@x
        \northeast
        \ifdim\pgf@xa>\pgf@x
            \pointangle
        \else
            \pgf@xa=\pgf@x
            \pgf@ya=0.5\pgf@y
            \southwest
            \advance\pgf@ya by 0.5\pgf@y
            \pgf@x=\pgf@xa
            \pgf@y=\pgf@ya
        \fi
    }

    \anchor{west}{
        \computecoordinates
        \pointangle
        \pgf@xa=\pgf@x
        \southwest
        \ifdim\pgf@xa<\pgf@x
            \pointangle
        \else
            \pgf@xa=\pgf@x
            \pgf@ya=0.5\pgf@y
            \northeast
            \advance\pgf@ya by 0.5\pgf@y
            \pgf@x=\pgf@xa
            \pgf@y=\pgf@ya
        \fi
    }

    \anchor{center}{
        \computecoordinates
        \pgf@process{\southwest}
        \pgf@xa=0.5\pgf@x
        \pgf@ya=0.5\pgf@y
        \pgf@process{\northeast}
        \advance\pgf@xa by 0.5\pgf@x
        \advance\pgf@ya by 0.5\pgf@y
        \pgf@x=\pgf@xa
        \pgf@y=\pgf@ya
    }

    \anchorborder{
        \@tempdima=\pgf@x
        \@tempdimb=\pgf@y
        \pgf@sh@reanchor{tag}{center}
        \advance\@tempdima by \pgf@x
        \advance\@tempdimb by \pgf@y
        \computecoordinates
        \pointangle
        \pgf@xa=\pgf@x
        \pgf@ya=\pgf@y
        \northeast
        \ifdim\pgf@xa>\pgf@x
            \def\orientation{right}
        \fi
        \ifdim\pgf@ya>\pgf@y
            \def\orientation{up}
        \fi
        \southwest
        \ifdim\pgf@xa<\pgf@x
            \def\orientation{left}
        \fi
        \ifdim\pgf@ya<\pgf@y
            \def\orientation{down}
        \fi
        \ifx\orientation\oright
            \edef\pgf@marshal{%
                \noexpand\belongstocone
                {\noexpand\pgf@sh@reanchor{tag}{center}}
                {\noexpand\northeast}%
                {\noexpand\pointangle}%
                {\noexpand\pgfpoint{\the\@tempdima}{\the\@tempdimb}}%
            }
            \pgf@process{\pgf@marshal}
            \if@tempswa
                \pgfpointintersectionoflines{\pgfpoint{\@tempdima}{\@tempdimb}}{\pgf@sh@reanchor{tag}{center}}{\northeast}{\pointangle}
            \else
                \edef\pgf@marshal{%
                    \noexpand\belongstocone
                    {\noexpand\pgf@sh@reanchor{tag}{center}}
                    {\noexpand\pointangle}%
                    {\noexpand\pgf@sh@reanchor{tag}{south east}}
                    {\noexpand\pgfpoint{\the\@tempdima}{\the\@tempdimb}}%
                }
                \pgf@process{\pgf@marshal}
                \if@tempswa
                    \pgfpointintersectionoflines{\pgfpoint{\@tempdima}{\@tempdimb}}{\pgf@sh@reanchor{tag}{center}}{\pointangle}{\pgf@sh@reanchor{tag}{south east}}
                \else
                    \pointborderrectanglecorners{\pgfpoint{\@tempdima}{\@tempdimb}}{\southwest}{\northeast}
                \fi
            \fi
        \fi
        \ifx\orientation\oleft
            \edef\pgf@marshal{%
                \noexpand\belongstocone
                {\noexpand\pgf@sh@reanchor{tag}{center}}
                {\noexpand\southwest}%
                {\noexpand\pointangle}%
                {\noexpand\pgfpoint{\the\@tempdima}{\the\@tempdimb}}%
            }
            \pgf@process{\pgf@marshal}
            \if@tempswa
                \pgfpointintersectionoflines{\pgfpoint{\@tempdima}{\@tempdimb}}{\pgf@sh@reanchor{tag}{center}}{\southwest}{\pointangle}
            \else
                \edef\pgf@marshal{%
                    \noexpand\belongstocone
                    {\noexpand\pgf@sh@reanchor{tag}{center}}
                    {\noexpand\pointangle}%
                    {\noexpand\pgf@sh@reanchor{tag}{north west}}
                    {\noexpand\pgfpoint{\the\@tempdima}{\the\@tempdimb}}%
                }
                \pgf@process{\pgf@marshal}
                \if@tempswa
                    \pgfpointintersectionoflines{\pgfpoint{\@tempdima}{\@tempdimb}}{\pgf@sh@reanchor{tag}{center}}{\pointangle}{\pgf@sh@reanchor{tag}{north west}}
                \else
                    \pointborderrectanglecorners{\pgfpoint{\@tempdima}{\@tempdimb}}{\southwest}{\northeast}
                \fi
            \fi
        \fi
        \ifx\orientation\odown
            \edef\pgf@marshal{%
                \noexpand\belongstocone
                {\noexpand\pgf@sh@reanchor{tag}{center}}
                {\noexpand\pointangle}%
                {\noexpand\southwest}%
                {\noexpand\pgfpoint{\the\@tempdima}{\the\@tempdimb}}%
            }
            \pgf@process{\pgf@marshal}
            \if@tempswa
                \pgfpointintersectionoflines{\pgfpoint{\@tempdima}{\@tempdimb}}{\pgf@sh@reanchor{tag}{center}}{\southwest}{\pointangle}
            \else
                \edef\pgf@marshal{%
                    \noexpand\belongstocone
                    {\noexpand\pgf@sh@reanchor{tag}{center}}
                    {\noexpand\pgf@sh@reanchor{tag}{south east}}
                    {\noexpand\pointangle}%
                    {\noexpand\pgfpoint{\the\@tempdima}{\the\@tempdimb}}%
                }
                \pgf@process{\pgf@marshal}
                \if@tempswa
                    \pgfpointintersectionoflines{\pgfpoint{\@tempdima}{\@tempdimb}}{\pgf@sh@reanchor{tag}{center}}{\pointangle}{\pgf@sh@reanchor{tag}{south east}}
                \else
                    \pointborderrectanglecorners{\pgfpoint{\@tempdima}{\@tempdimb}}{\southwest}{\northeast}
                \fi
            \fi
        \fi
        \ifx\orientation\oup
            \edef\pgf@marshal{%
                \noexpand\belongstocone
                {\noexpand\pgf@sh@reanchor{tag}{center}}
                {\noexpand\pointangle}%
                {\noexpand\northeast}%
                {\noexpand\pgfpoint{\the\@tempdima}{\the\@tempdimb}}%
            }
            \pgf@process{\pgf@marshal}
            \if@tempswa
                \pgfpointintersectionoflines{\pgfpoint{\@tempdima}{\@tempdimb}}{\pgf@sh@reanchor{tag}{center}}{\northeast}{\pointangle}
            \else
                \edef\pgf@marshal{%
                    \noexpand\belongstocone
                    {\noexpand\pgf@sh@reanchor{tag}{center}}
                    {\noexpand\pgf@sh@reanchor{tag}{north west}}
                    {\noexpand\pointangle}%
                    {\noexpand\pgfpoint{\the\@tempdima}{\the\@tempdimb}}%
                }
                \pgf@process{\pgf@marshal}
                \if@tempswa
                    \pgfpointintersectionoflines{\pgfpoint{\@tempdima}{\@tempdimb}}{\pgf@sh@reanchor{tag}{center}}{\pointangle}{\pgf@sh@reanchor{tag}{north west}}
                \else
                    \pointborderrectanglecorners{\pgfpoint{\@tempdima}{\@tempdimb}}{\southwest}{\northeast}
                \fi
            \fi
        \fi
    }

    \backgroundpath{
        \computecoordinates
        \pgf@process{\southwest}
        \pgf@xa=\pgf@x
        \pgf@ya=\pgf@y
        \pgf@process{\northeast}
        \pgf@xb=\pgf@x
        \pgf@yb=\pgf@y
        \pgfkeysgetvalue{/pgf/orientation}{\orientation}
        \ifx\orientation\oright
            \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
            \pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@yb}}
            \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
            \pgfpathlineto{\pointangle}
            \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}
        \fi
        \ifx\orientation\oleft
            \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
            \pgfpathlineto{\pointangle}
            \pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@yb}}
            \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
            \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}
        \fi
        \ifx\orientation\odown
            \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
            \pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@yb}}
            \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
            \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}
            \pgfpathlineto{\pointangle}
        \fi
        \ifx\orientation\oup
            \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
            \pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@yb}}
            \pgfpathlineto{\pointangle}
            \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
            \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}
        \fi
        \pgfclosepath
    }
}
\pgfdeclareshape{complex}{

    \inheritsavedanchors[from=rectangle] % this is nearly a rectangle

    \savedmacro{\scarceratio}{\def\scarceratio{0.15}}

    \savedmacro\computecoordinates{%
        \pgf@yb = \ht\pgfnodeparttextbox
        \advance\pgf@yb by \dp\pgfnodeparttextbox
        \pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/pgf/inner ysep}}
        \advance\pgf@yb by 2\pgf@xa
        \pgf@yc=\pgfkeysvalueof{/pgf/minimum height}
        \ifdim\pgf@yc>\pgf@yb
            \pgf@yb=\pgf@yc
        \fi
        \pgf@xb=\wd\pgfnodeparttextbox
        \pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/pgf/inner xsep}}
        \advance\pgf@xb by 2\pgf@xa
        \pgf@xc=\pgfkeysvalueof{/pgf/minimum width}
        \ifdim\pgf@xc>\pgf@xb
            \pgf@xb=\pgf@xc
        \fi
        \ifdim\pgf@yb>\pgf@xb
            \pgfmathsetlengthmacro\scarceoffset{\scarceratio*\pgf@xb}
        \else
            \pgfmathsetlengthmacro\scarceoffset{\scarceratio*\pgf@yb}
        \fi
        \addtosavedmacro\scarceoffset
        \pgf@xa=-0.5\pgf@xb
        \advance\pgf@xa by 0.5\wd\pgfnodeparttextbox
        \pgf@xc=\pgf@xa %saving for later
        \pgf@ya=0.5\pgf@yb
        \advance\pgf@ya by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@ya by -0.5\dp\pgfnodeparttextbox
        \advance\pgf@ya by -\scarceoffset
        \pgfextract@process\westnorthjoin{\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}
        \addtosavedmacro{\westnorthjoin}
        \advance\pgf@ya by \scarceoffset
        \advance\pgf@xa by \scarceoffset
        \pgfextract@process\northwestjoin{\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}
        \addtosavedmacro{\northwestjoin}
        \advance\pgf@xa by \pgf@xb
        \pgfmathaddtolength{\pgf@xa}{-2*\scarceoffset}
        \pgfextract@process\northeastjoin{\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}
        \addtosavedmacro{\northeastjoin}
        \advance\pgf@ya by -\scarceoffset
        \advance\pgf@xa by \scarceoffset
        \pgfextract@process\eastnorthjoin{\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}
        \addtosavedmacro{\eastnorthjoin}
        \advance\pgf@ya by -\pgf@yb
        \pgfmathaddtolength{\pgf@ya}{2*\scarceoffset}
        \pgfextract@process\eastsouthjoin{\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}
        \addtosavedmacro{\eastsouthjoin}
        \advance\pgf@ya by -\scarceoffset
        \advance\pgf@xa by -\scarceoffset
        \pgfextract@process\southeastjoin{\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}
        \addtosavedmacro{\southeastjoin}
        \pgf@xa=\pgf@xc
        \advance\pgf@xa by \scarceoffset
        \pgfextract@process\southwestjoin{\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}
        \addtosavedmacro{\southwestjoin}
        \advance\pgf@xa by -\scarceoffset
        \advance\pgf@ya by \scarceoffset
        \pgfextract@process\westsouthjoin{\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}
        \addtosavedmacro{\westsouthjoin}
    }

    \inheritanchorborder[from=rectangle]

    \foreach \a in {center, north, south, west, east, south east, south west, north east, north west}
    {
        \inheritanchor[from=rectangle]{\a}
    }

    \backgroundpath{
        \pgfpathmoveto{\northwestjoin}
        \pgfpathlineto{\northeastjoin}
        \pgfpathlineto{\eastnorthjoin}
        \pgfpathlineto{\eastsouthjoin}
        \pgfpathlineto{\southeastjoin}
        \pgfpathlineto{\southwestjoin}
        \pgfpathlineto{\westsouthjoin}
        \pgfpathlineto{\westnorthjoin}
        \pgfpathclose
    }

    \foregroundpath{
        \pgfkeysgetvalue{/pgf/clone}{\clone}
        \ifx\clone\true
            \def\cloneoffsetratio{0.25}
            \computecoordinates
            \northwestjoin
            \pgf@ya=\pgf@y
            \southwestjoin
            \advance\pgf@ya by -\pgf@y
            \newdimen\cloneoffset
            \cloneoffset=\cloneoffsetratio\pgf@ya
            \pgf@yc=\pgf@y
            \advance\pgf@yc by \cloneoffset
            \westsouthjoin
            \pgf@xc=\pgf@x
            \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \eastnorthjoin
            \pgf@xc=\pgf@x
            \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \pgfpathlineto{\eastsouthjoin}
            \pgfpathlineto{\southeastjoin}
            \pgfpathlineto{\southwestjoin}
            \pgfpathlineto{\westsouthjoin}
            \pgfpathclose
            \pgfsetfillcolor{\tikz@strokecolor}
            \pgfusepath{fill, stroke}
        \fi
    }
}
\pgfdeclareshape{svlocation}{
    \inheritsavedanchors[from=circle]
    \inheritanchorborder[from=circle]
    \foreach \a in {center, east, south, north, west, south east, south west, north east, north west}
    {
        \inheritanchor[from=circle]{\a}
    }
    \backgroundpath{
        \pgf@xa = \radius
        \pgfmathsetlength{\pgf@xb}{\pgfkeysvalueof{/pgf/outer xsep}}
        \advance\pgf@xa by -\pgf@xb
        \pgf@process{\pgfpathcircle{\centerpoint}{\pgf@xa}}
        \pgf@process{\centerpoint}
        \@tempdimb = \pgf@y
        \advance\@tempdimb by -0.6\pgf@xa
        \advance\@tempdimb by 0.5\pgflinewidth
        \edef\pgf@marshal{
            \noexpand\circlefindx
            {\noexpand\centerpoint}
            {\the\pgf@xa}
            {\the\@tempdimb}
            {1}
        }
        \pgf@process{\pgf@marshal}
        \@tempdima = \pgf@x
        \pgfpathmoveto{\pgfpoint{\@tempdima}{\@tempdimb}}
        \pgfpathlineto{\pgfpoint{-\@tempdimb}{-\@tempdima}}
        \pgf@xc = 0.5\@tempdima
        \advance\pgf@xc by -0.5\@tempdimb
        \pgf@ya = 0.5\@tempdimb
        \advance\pgf@ya by -0.5\@tempdima
        \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@ya}}
        \pgf@process{\centerpoint}
        \pgf@xb = \pgf@x
        \pgf@yb = \pgf@y
        \advance\pgf@xb by 0.7072\pgf@xa
        \advance\pgf@yb by -0.7072\pgf@xa
        \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
    }
}
\pgfdeclareshape{simplechemicalmultimer}{

    \inheritsavedanchors[from=rectangle] % this is nearly a rectangle

    \savedmacro{\offsetratio}{\def\offsetratio{0.1}}

    \savedmacro\computecoordinates{%
        \pgf@y = \ht\pgfnodeparttextbox
        \advance\pgf@y by \dp\pgfnodeparttextbox
        \pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/pgf/inner ysep}}
        \advance\pgf@y by 2\pgf@xa
        \pgfmathsetlength{\pgf@y}{\pgf@y/(1-\offsetratio)}
        \pgf@yb=\pgfkeysvalueof{/pgf/minimum height}
        \ifdim\pgf@yb>\pgf@y
            \pgf@y=\pgf@yb
        \fi
        \pgf@yb=\offsetratio\pgf@y
        \pgfmathsetlengthmacro\offset{\pgf@yb}
        \addtosavedmacro\offset
        \pgf@x=\wd\pgfnodeparttextbox
        \pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/pgf/inner xsep}}
        \advance\pgf@x by 2\pgf@xa
        \pgf@xb=\pgfkeysvalueof{/pgf/minimum width}
        \advance\pgf@x by \offset
        \ifdim\pgf@xb>\pgf@x
            \pgf@x=\pgf@xb
        \fi
        \ifdim\pgf@y>\pgf@x
            \pgf@x=\pgf@y
        \fi
        \@tempdima=\pgf@x
        \@tempdimb=\pgf@y
        \pgf@yc=\@tempdimb
        \advance\pgf@yc by -\offset
        \pgf@yc=0.5\pgf@yc
        \pgfmathsetlengthmacro{\radius}{\the\pgf@yc}
        \addtosavedmacro{\radius}
        \pgf@xa=-0.5\@tempdima
        \pgfmathaddtolength{\pgf@xa}{0.5*\offset}
        \advance\pgf@xa 0.5\wd\pgfnodeparttextbox
        \pgfmathaddtolength{\pgf@xa}{\radius}
        \pgf@ya=0.5\ht\pgfnodeparttextbox
        \advance\pgf@ya by -0.5\dp\pgfnodeparttextbox
        \pgfextract@process\upperleftcenter{\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}
        \addtosavedmacro{\upperleftcenter}
        \pgf@xc=\pgf@xa
        \pgf@yc=\pgf@ya
        \advance\pgf@yc by \radius
        \pgfextract@process\upperleftjoin{\pgfpoint{\the\pgf@xc}{\the\pgf@yc}}
        \addtosavedmacro{\upperleftjoin}
        \pgf@yc=\pgf@ya
        \advance\pgf@yc by -\radius
        \pgfextract@process\middleleftjoin{\pgfpoint{\the\pgf@xc}{\the\pgf@yc}}
        \addtosavedmacro{\middleleftjoin}
        \pgf@xc=\pgf@xa
        \advance\pgf@xc by \offset
        \pgf@yc=\pgf@ya
        \advance\pgf@yc by -\offset
        \pgfextract@process\lowerleftcenter{\pgfpoint{\the\pgf@xc}{\the\pgf@yc}}
        \addtosavedmacro{\lowerleftcenter}
        \advance\pgf@yc by -\radius
        \pgfextract@process\lowerleftjoin{\pgfpoint{\the\pgf@xc}{\the\pgf@yc}}
        \addtosavedmacro{\lowerleftjoin}
        \pgf@xc=\pgf@xa
        \advance\pgf@xc by \@tempdima
        \pgfmathaddtolength{\pgf@xc}{-2*\radius}
        \advance\pgf@xc by -\offset
        \pgf@yc=\pgf@ya
        \pgfextract@process\upperrightcenter{\pgfpoint{\the\pgf@xc}{\the\pgf@yc}}
        \addtosavedmacro{\upperrightcenter}
        \advance\pgf@yc by \radius
        \pgfextract@process\upperrightjoin{\pgfpoint{\the\pgf@xc}{\the\pgf@yc}}
        \addtosavedmacro{\upperrightjoin}
        \pgf@yc=\pgf@ya
        \advance\pgf@yc by -\radius
        \pgfextract@process\middlerightjoin{\pgfpoint{\the\pgf@xc}{\the\pgf@yc}}
        \addtosavedmacro{\middlerightjoin}
        \advance\pgf@xc by \offset
        \pgf@yc=\pgf@ya
        \advance\pgf@yc by -\offset
        \pgfextract@process\lowerrightcenter{\pgfpoint{\the\pgf@xc}{\the\pgf@yc}}
        \addtosavedmacro{\lowerrightcenter}
        \advance\pgf@yc by -\radius
        \pgfextract@process\lowerrightjoin{\pgfpoint{\the\pgf@xc}{\the\pgf@yc}}
        \addtosavedmacro{\lowerrightjoin}
        \pgf@process{\pgfpointintersectionofcircles{\upperleftcenter}{\lowerleftcenter}{\radius}{\radius}{1}}
        \pgfextract@process\leftintersection{\noexpand\pgfpoint{\the\pgf@x}{\the\pgf@y}}
        \addtosavedmacro{\leftintersection}
        \pgf@process{\pgfpointintersectionofcircles{\upperrightcenter}{\lowerrightcenter}{\radius}{\radius}{2}}
        \pgfextract@process\rightintersection{\noexpand\pgfpoint{\the\pgf@x}{\the\pgf@y}}
        \addtosavedmacro{\rightintersection}
    }
    %

    \anchor{center}{
        \computecoordinates
        \pgf@process{\lowerrightcenter}
        \pgf@xa=\pgf@x
        \pgf@process{\upperleftcenter}
        \pgf@x=0.5\pgf@x
        \advance\pgf@x by 0.5\pgf@xa
        \pgfmathaddtolength{\pgf@y}{-0.5*\offset}
    }

    % \anchor{north}{
    %     \computecoordinates
    %     \lowerrightcenter
    %     \pgf@xa=\pgf@x
    %     \upperleftcenter
    %     \pgf@x=-0.5\pgf@x
    %     \pgf@x=0.5\pgf@xa
    %     \pgfmathaddtolength{\pgf@x}{0.5*\pgf@xa}
    %     \pgfmathaddtolength{\pgf@x}{0.5*\offset}
    %     \advance\pgf@y by \radius
    % }

    \foreach \a in {north, west, east, south, north east, south west, north west, south east}
    {
        \inheritanchor[from=rectangle]{\a}
    }

    \anchorborder{
        \@tempdima=\pgf@x
        \@tempdimb=\pgf@y
        \pgf@sh@reanchor{simplechemicalmultimer}{center}
        \advance\@tempdima by \pgf@x
        \advance\@tempdimb by \pgf@y
        \computecoordinates
        \edef\pgf@marshal{
            \noexpand\belongstocone
            {\noexpand\pgf@sh@reanchor{simplechemicalmultimer}{center}}
            {\noexpand\upperleftjoin}%
            {\noexpand\upperrightjoin}%
            {\noexpand\pgfpoint{\the\@tempdima}{\the\@tempdimb}}%
        }
        \pgf@process{\pgf@marshal}
        \if@tempswa
            \edef\pgf@marshal{
                \noexpand\pointborderrectanglecorners
                {\noexpand\pgfpoint{\the\@tempdima}{\the\@tempdimb}}
                {\noexpand\pgfpointadd{\middleleftjoin}{\noexpand\pgfpoint{0}{-\offset}}}
                {\noexpand\pgfpointadd{\upperrightjoin}{\noexpand\pgfpoint{\offset}{0}}}
            }
            \pgf@process{\pgf@marshal}
        \else
            \edef\pgf@marshal{
                \noexpand\belongstocone
                {\noexpand\pgf@sh@reanchor{simplechemicalmultimer}{center}}
                {\upperrightjoin}
                {\rightintersection}
                {\noexpand\pgfpoint{\the\@tempdima}{\the\@tempdimb}}
            }
            \pgf@process{\pgf@marshal}
            \if@tempswa
                \pgf@sh@reanchor{simplechemicalmultimer}{center}
                \ifdim\@tempdima<\pgf@x
                    \c@pgf@counta=1
                \else
                    \c@pgf@counta=2
                \fi
                \edef\pgf@marshal{
                    \noexpand\intersectionlinecircle
                    {\noexpand\pgf@sh@reanchor{simplechemicalmultimer}{center}}
                    {\noexpand\pgfpoint{\the\@tempdima}{\the\@tempdimb}}
                    {\upperrightcenter}
                    {\radius}
                    {\the\c@pgf@counta}
                }
                \pgf@process{\pgf@marshal}
            \else
                \edef\pgf@marshal{
                    \noexpand\belongstocone
                    {\noexpand\pgf@sh@reanchor{simplechemicalmultimer}{center}}
                    {\rightintersection}
                    {\lowerrightjoin}
                    {\noexpand\pgfpoint{\the\@tempdima}{\the\@tempdimb}}
                }
                \pgf@process{\pgf@marshal}
                \if@tempswa
                    \edef\pgf@marshal{
                        \noexpand\intersectionlinecircle
                        {\noexpand\pgf@sh@reanchor{simplechemicalmultimer}{center}}
                        {\noexpand\pgfpoint{\the\@tempdima}{\the\@tempdimb}}
                        {\lowerrightcenter}
                        {\radius}
                        {2}
                    }
                    \pgf@process{\pgf@marshal}
                \else
                    \edef\pgf@marshal{
                        \noexpand\belongstocone
                        {\noexpand\pgf@sh@reanchor{simplechemicalmultimer}{center}}
                        {\lowerrightjoin}
                        {\lowerleftjoin}
                        {\noexpand\pgfpoint{\the\@tempdima}{\the\@tempdimb}}
                    }
                    \pgf@process{\pgf@marshal}
                    \if@tempswa
                        \edef\pgf@marshal{
                            \noexpand\pointborderrectanglecorners
                            {\noexpand\pgfpoint{\the\@tempdima}{\the\@tempdimb}}
                            {\noexpand\pgfpointadd{\middleleftjoin}{\noexpand\pgfpoint{0}{-\offset}}}
                            {\noexpand\pgfpointadd{\upperrightjoin}{\noexpand\pgfpoint{\offset}{0}}}
                        }
                        \pgf@process{\pgf@marshal}
                    \else
                        \edef\pgf@marshal{
                            \noexpand\belongstocone
                            {\noexpand\pgf@sh@reanchor{simplechemicalmultimer}{center}}
                            {\lowerleftjoin}
                            {\leftintersection}
                            {\noexpand\pgfpoint{\the\@tempdima}{\the\@tempdimb}}
                        }
                        \pgf@process{\pgf@marshal}
                        \if@tempswa
                            \pgf@sh@reanchor{simplechemicalmultimer}{center}
                            \ifdim\@tempdima>\pgf@x
                                \c@pgf@counta=2
                            \else
                                \c@pgf@counta=1
                            \fi
                            \edef\pgf@marshal{
                                \noexpand\intersectionlinecircle
                                {\noexpand\pgf@sh@reanchor{simplechemicalmultimer}{center}}
                                {\noexpand\pgfpoint{\the\@tempdima}{\the\@tempdimb}}
                                {\lowerleftcenter}
                                {\radius}
                                {\the\c@pgf@counta}
                            }
                            \pgf@process{\pgf@marshal}
                        \else
                            \edef\pgf@marshal{
                                \noexpand\intersectionlinecircle
                                {\noexpand\pgf@sh@reanchor{simplechemicalmultimer}{center}}
                                {\noexpand\pgfpoint{\the\@tempdima}{\the\@tempdimb}}
                                {\upperleftcenter}
                                {\radius}
                                {1}
                            }
                            \pgf@process{\pgf@marshal}
                        \fi
                    \fi
                \fi
            \fi
        \fi
    }

    \backgroundpath{
        \computecoordinates
        \pgfpathmoveto{\upperleftjoin}
        \pgfpathlineto{\upperrightjoin}
        \pgfpatharc{90}{-90}{\radius}
        \pgfpathlineto{\middleleftjoin}
        \pgfpatharc{90}{-90}{-\radius}
        \pgfpathclose

        \leftintersection
        \pgf@xc=\pgf@x
        \pgf@yc=\pgf@y
        \pgfpathmoveto{\pgfpoint{\pgf@x}{\pgf@y}}
        \pgf@process{\circlefindangle{\lowerleftcenter}{\radius}{\pgf@yc}{1}}
        \pgfpatharc{\pgf@x}{-90}{\radius}
        \pgfpathlineto{\lowerrightjoin}
        \rightintersection
        \pgf@yc=\pgf@y
        \pgf@process{\circlefindangle{\lowerrightcenter}{\radius}{\pgf@yc}{2}}
        \pgfpatharc{-90}{\pgf@x}{\radius}
        \pgf@process{\circlefindangle{\upperrightcenter}{\radius}{\pgf@yc}{2}}
        \pgfpatharc{\pgf@x}{-90}{\radius}
        \pgflineto{\middleleftjoin}
        \leftintersection
        \pgf@yc=\pgf@y
        \pgf@process{\circlefindangle{\upperleftcenter}{\radius}{\pgf@yc}{1}}
        \pgfpatharc{-90}{\pgf@x}{\radius}
        \pgfpathclose
    }

    \foregroundpath{
        \pgfkeysgetvalue{/pgf/clone}{\clone}
        \ifx\clone\true
            \def\cloneoffsetratio{0.25}
            \computecoordinates
            \newdimen\cloneoffset
            \pgfmathsetlength{\cloneoffset}{\cloneoffsetratio*2*\radius}
            \middleleftjoin
            \pgf@yc=\pgf@y
            \advance\pgf@yc by \cloneoffset
            \pgf@yb=\pgf@yc
            \pgf@process{\circlefindx{\upperleftcenter}{\radius}{\pgf@yc}{1}}
            \pgfpathmoveto{\pgfpoint{\pgf@x}{\pgf@yc}}
            \pgf@process{\circlefindx{\upperrightcenter}{\radius}{\pgf@yc}{2}}
            \pgfpathlineto{\pgfpoint{\pgf@x}{\pgf@yc}}
            \pgf@process{\circlefindangle{\upperrightcenter}{\radius}{\pgf@yc}{2}}
            \pgf@xc=\pgf@x
            \lowerrightjoin
            \pgf@yc=\pgf@y
            \advance\pgf@yc by \cloneoffset
            \pgf@process{\circlefindangle{\upperrightcenter}{\radius}{\pgf@yc}{2}}
            \pgfpatharc{\pgf@xc}{\pgf@x}{\radius}
            \pgf@process{\circlefindx{\lowerrightcenter}{\radius}{\pgf@yc}{2}}
            \pgfpathlineto{\pgfpoint{\pgf@x}{\pgf@yc}}
            \pgf@process{\circlefindangle{\lowerrightcenter}{\radius}{\pgf@yc}{2}}
            \pgfpatharc{\pgf@x}{-90}{\radius}
            \pgfpathlineto{\lowerleftjoin}
            \leftintersection
            \pgf@yc=\pgf@y
            \pgf@process{\circlefindangle{\lowerleftcenter}{\radius}{\pgf@yc}{1}}
            \pgfpatharc{-90}{\pgf@x}{\radius}
            \pgf@process{\circlefindangle{\upperleftcenter}{\radius}{\pgf@yc}{1}}
            \pgf@xc=\pgf@x
            \pgf@process{\circlefindangle{\upperleftcenter}{\radius}{\pgf@yb}{1}}
            \pgfpatharc{\pgf@xc}{\pgf@x}{\radius}
            % \pgfpathclose
            \pgfsetfillcolor{\tikz@strokecolor}
            \pgfusepath{stroke, fill}
        \fi
    }
}
\pgfdeclareshape{complexmultimer}{

    \inheritsavedanchors[from=rectangle] % this is nearly a rectangle

    \savedmacro{\scarceratio}{\def\scarceratio{0.09}}

    \savedmacro{\offsetratio}{\def\offsetratio{0.1}}

    \savedmacro\computecoordinates{%
        \pgf@yb = \ht\pgfnodeparttextbox
        \advance\pgf@yb by \dp\pgfnodeparttextbox
        \pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/pgf/inner ysep}}
        \advance\pgf@yb by 2\pgf@xa
        \pgfmathsetlength{\pgf@yb}{\pgf@yb/(1-\offsetratio)}
        \pgf@yc=\pgfkeysvalueof{/pgf/minimum height}
        \ifdim\pgf@yc>\pgf@yb
            \pgf@yb=\pgf@yc
        \fi
        \pgfmathsetlengthmacro\offset{\offsetratio*\pgf@yb}
        \addtosavedmacro\offset
        \pgf@xb=\wd\pgfnodeparttextbox
        \pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/pgf/inner xsep}}
        \advance\pgf@xb by 2\pgf@xa
        \pgf@xc=\pgfkeysvalueof{/pgf/minimum width}
        \advance\pgf@xb by \offset
        \ifdim\pgf@xc>\pgf@xb
            \pgf@xb=\pgf@xc
        \fi
        \advance\pgf@xb by -\offset
        \advance\pgf@yb by -\offset
        \ifdim\pgf@yb>\pgf@xb
            \pgfmathsetlengthmacro\scarceoffset{\scarceratio*\pgf@xb}
        \else
            \pgfmathsetlengthmacro\scarceoffset{\scarceratio*\pgf@yb}
        \fi
        \addtosavedmacro\scarceoffset
        \pgf@xa=-0.5\pgf@xb
        \advance\pgf@xa by 0.5\wd\pgfnodeparttextbox
        \pgf@xc=\pgf@xa %saving for later
        \pgf@ya=0.5\pgf@yb
        \advance\pgf@ya by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@ya by -0.5\dp\pgfnodeparttextbox
        \advance\pgf@ya by -\scarceoffset
        \pgfextract@process\upperwestnorthjoin{\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}
        \addtosavedmacro{\upperwestnorthjoin}
        \advance\pgf@ya by \scarceoffset
        \advance\pgf@xa by \scarceoffset
        \pgfextract@process\uppernorthwestjoin{\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}
        \addtosavedmacro{\uppernorthwestjoin}
        \advance\pgf@xa by \pgf@xb
        \pgfmathaddtolength{\pgf@xa}{-2*\scarceoffset}
        \pgfextract@process\uppernortheastjoin{\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}
        \addtosavedmacro{\uppernortheastjoin}
        \advance\pgf@ya by -\scarceoffset
        \advance\pgf@xa by \scarceoffset
        \pgfextract@process\uppereastnorthjoin{\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}
        \addtosavedmacro{\uppereastnorthjoin}
        \advance\pgf@ya by -\pgf@yb
        \pgfmathaddtolength{\pgf@ya}{2*\scarceoffset}
        \pgfextract@process\uppereastsouthjoin{\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}
        \addtosavedmacro{\uppereastsouthjoin}
        \advance\pgf@ya by -\scarceoffset
        \advance\pgf@xa by -\scarceoffset
        \pgfextract@process\uppersoutheastjoin{\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}
        \addtosavedmacro{\uppersoutheastjoin}
        \pgf@xa=\pgf@xc
        \advance\pgf@xa by \scarceoffset
        \pgfextract@process\uppersouthwestjoin{\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}
        \addtosavedmacro{\uppersouthwestjoin}
        \advance\pgf@xa by -\scarceoffset
        \advance\pgf@ya by \scarceoffset
        \pgfextract@process\upperwestsouthjoin{\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}
        \addtosavedmacro{\upperwestsouthjoin}
        \upperwestnorthjoin
        \advance\pgf@x by \offset
        \advance\pgf@y by -\offset
        \pgfextract@process\lowerwestnorthjoin{\pgfpoint{\the\pgf@x}{\the\pgf@y}}
        \addtosavedmacro{\lowerwestnorthjoin}
        \uppernorthwestjoin
        \advance\pgf@x by \offset
        \advance\pgf@y by -\offset
        \pgfextract@process\lowernorthwestjoin{\pgfpoint{\the\pgf@x}{\the\pgf@y}}
        \addtosavedmacro{\lowernorthwestjoin}
        \uppernortheastjoin
        \advance\pgf@x by \offset
        \advance\pgf@y by -\offset
        \pgfextract@process\lowernortheastjoin{\pgfpoint{\the\pgf@x}{\the\pgf@y}}
        \addtosavedmacro{\lowernortheastjoin}
        \uppereastnorthjoin
        \advance\pgf@x by \offset
        \advance\pgf@y by -\offset
        \pgfextract@process\lowereastnorthjoin{\pgfpoint{\the\pgf@x}{\the\pgf@y}}
        \addtosavedmacro{\lowereastnorthjoin}
        \uppereastsouthjoin
        \advance\pgf@x by \offset
        \advance\pgf@y by -\offset
        \pgfextract@process\lowereastsouthjoin{\pgfpoint{\the\pgf@x}{\the\pgf@y}}
        \addtosavedmacro{\lowereastsouthjoin}
        \uppersoutheastjoin
        \advance\pgf@x by \offset
        \advance\pgf@y by -\offset
        \pgfextract@process\lowersoutheastjoin{\pgfpoint{\the\pgf@x}{\the\pgf@y}}
        \addtosavedmacro{\lowersoutheastjoin}
        \uppersouthwestjoin
        \advance\pgf@x by \offset
        \advance\pgf@y by -\offset
        \pgfextract@process\lowersouthwestjoin{\pgfpoint{\the\pgf@x}{\the\pgf@y}}
        \addtosavedmacro{\lowersouthwestjoin}
        \upperwestsouthjoin
        \advance\pgf@x by \offset
        \advance\pgf@y by -\offset
        \pgfextract@process\lowerwestsouthjoin{\pgfpoint{\the\pgf@x}{\the\pgf@y}}
        \addtosavedmacro{\lowerwestsouthjoin}
        \pgf@xa=\offset
        \pgf@xb=\scarceoffset\relax
        \ifdim\pgf@xa>\pgf@xb
            \lowerwestsouthjoin
            \pgf@xc=\pgf@x
            \uppersouthwestjoin
            \pgfextract@process\leftintersection{\pgfpoint{\the\pgf@xc}{\the\pgf@y}}
            \addtosavedmacro{\leftintersection}
            \uppereastnorthjoin
            \pgf@xc=\pgf@x
            \lowernortheastjoin
            \pgfextract@process\rightintersection{\pgfpoint{\the\pgf@xc}{\the\pgf@y}}
            \addtosavedmacro{\rightintersection}
        \else
            \upperwestsouthjoin
            \pgf@xa=\pgf@x
            \pgf@ya=\pgf@y
            \uppersouthwestjoin
            \pgf@xb=\pgf@x
            \pgf@yb=\pgf@y
            \lowersouthwestjoin
            \pgfmathsetlength{\pgf@y}{((\pgf@yb-\pgf@ya)*\pgf@x+\pgf@ya*\pgf@xb-\pgf@yb*\pgf@xa)/(\pgf@xb-\pgf@xa)}
            \pgfextract@process\leftintersection{\pgfpoint{\the\pgf@x}{\the\pgf@y}}
            \addtosavedmacro{\leftintersection}
            \lowernortheastjoin
            \pgf@xa=\pgf@x
            \pgf@ya=\pgf@y
            \lowereastnorthjoin
            \pgf@xb=\pgf@x
            \pgf@yb=\pgf@y
            \uppereastnorthjoin
            \pgfmathsetlength{\pgf@y}{((\pgf@yb-\pgf@ya)*\pgf@x+\pgf@ya*\pgf@xb-\pgf@yb*\pgf@xa)/(\pgf@xb-\pgf@xa)}
            \pgfextract@process\rightintersection{\pgfpoint{\the\pgf@x}{\the\pgf@y}}
            \addtosavedmacro{\rightintersection}
        \fi
    }

    \inheritanchorborder[from=rectangle]

    \foreach \a in {center, north, south, west, east, south east, south west, north east, north west}
    {
        \inheritanchor[from=rectangle]{\a}
    }

    \backgroundpath{
        \computecoordinates
        \pgfpathmoveto{\uppernorthwestjoin}
        \pgfpathlineto{\uppernortheastjoin}
        \pgfpathlineto{\uppereastnorthjoin}
        \pgfpathlineto{\uppereastsouthjoin}
        \pgfpathlineto{\uppersoutheastjoin}
        \pgfpathlineto{\uppersouthwestjoin}
        \pgfpathlineto{\upperwestsouthjoin}
        \pgfpathlineto{\upperwestnorthjoin}
        \pgfpathclose

        \pgf@xa=\offset
        \pgf@xb=\scarceoffset
        \ifdim\pgf@xa>\pgf@xb
            \pgfpathmoveto{\leftintersection}
            \pgfpathlineto{\uppersoutheastjoin}
            \pgfpathlineto{\uppereastsouthjoin}
            \pgfpathlineto{\rightintersection}
            \pgfpathlineto{\lowernortheastjoin}
            \pgfpathlineto{\lowereastnorthjoin}
            \pgfpathlineto{\lowereastsouthjoin}
            \pgfpathlineto{\lowersoutheastjoin}
            \pgfpathlineto{\lowersouthwestjoin}
            \pgfpathlineto{\lowerwestsouthjoin}
            \pgfpathclose
        \else
            \pgfpathmoveto{\uppersouthwestjoin}
            \pgfpathlineto{\uppersoutheastjoin}
            \pgfpathlineto{\uppereastsouthjoin}
            \pgfpathlineto{\rightintersection}
            \pgfpathlineto{\lowereastnorthjoin}
            \pgfpathlineto{\lowereastsouthjoin}
            \pgfpathlineto{\lowersoutheastjoin}
            \pgfpathlineto{\lowersouthwestjoin}
            \pgfclosepath
        \fi
    }

    \foregroundpath{
        \pgfkeysgetvalue{/pgf/clone}{\clone}
        \ifx\clone\true
            \def\cloneoffsetratio{0.25}
            \computecoordinates
            \upperwestnorthjoin
            \pgf@xc=\pgf@x
            \pgf@ya=\pgf@y
            \uppersouthwestjoin
            \advance\pgf@ya by -\pgf@y
            \newdimen\cloneoffset
            \cloneoffset=\cloneoffsetratio\pgf@ya
            \pgf@yc=\pgf@y
            \advance\pgf@yc by \cloneoffset
            \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \uppereastnorthjoin
            \pgf@xc=\pgf@x
            \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \lowersoutheastjoin
            \pgf@yc=\pgf@y
            \advance\pgf@yc by \cloneoffset
            \pgf@xb=\offset
            \advance\pgf@xb by \scarceoffset\relax
            \ifdim\cloneoffset>\pgf@xb
                \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \else
                \pgfpathlineto{\uppereastsouthjoin}
                \uppersoutheastjoin
                \pgf@xa=\pgf@x
                \pgf@ya=\pgf@y
                \uppereastsouthjoin
                \pgf@xb=\pgf@x
                \pgf@yb=\pgf@y
                \pgfmathsetlength{\pgf@x}{(\pgf@yc*(\pgf@xb-\pgf@xa)+\pgf@yb*\pgf@xa-\pgf@ya*\pgf@xb)/(\pgf@yb-\pgf@ya)}
                \pgfpathlineto{\pgfpoint{\pgf@x}{\pgf@yc}}
            \fi
            \lowereastsouthjoin
            \pgf@xc=\pgf@x
            \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \pgfpathlineto{\lowereastsouthjoin}
            \pgfpathlineto{\lowersoutheastjoin}
            \pgfpathlineto{\lowersouthwestjoin}
            \pgf@xa=\offset
            \pgf@xb=\scarceoffset\relax
            \ifdim\pgf@xa>\pgf@xb
                \pgfpathlineto{\lowerwestsouthjoin}
                \pgfpathlineto{\leftintersection}
                \pgfpathlineto{\uppersouthwestjoin}
            \fi
            \pgfpathlineto{\upperwestsouthjoin}
            \pgfpathclose
            \pgfsetfillcolor{\tikz@strokecolor}
            \pgfusepath{fill, stroke}
        \fi

    }
}
\pgfdeclareshape{or}{

    \inheritsavedanchors[from=circle]
    \inheritanchorborder[from=circle]
    \foreach \a in {center, south east, south west, north east, north west}
    {
        \inheritanchor[from=circle]{\a}
    }

    \savedanchor\connectoreast{
        \pgfkeysgetvalue{/pgf/connectors}{\connectors}
        %compute width and height without taking into account outer sep
        \pgf@x=\wd\pgfnodeparttextbox
        \pgf@xc=\pgfkeysvalueof{/pgf/inner xsep}
        \advance\pgf@x by 2\pgf@xc
        \pgf@xc=\pgfkeysvalueof{/pgf/minimum width}
        \ifdim\pgf@xc>\pgf@x
            \pgf@x=\pgf@xc
        \fi
        \pgf@y=\ht\pgfnodeparttextbox
        \advance\pgf@y by \dp\pgfnodeparttextbox
        \pgf@yc=\pgfkeysvalueof{/pgf/inner ysep}
        \advance\pgf@y by 2\pgf@yc
        \pgf@yc=\pgfkeysvalueof{/pgf/minimum height}
        \ifdim\pgf@yc>\pgf@y
            \pgf@y=\pgf@yc
        \fi
        %store south west in xa,ya and north east in xb,yb
        \pgf@xa=-0.5\pgf@x
        \advance\pgf@xa by 0.5\wd\pgfnodeparttextbox
        \pgf@ya=-0.5\pgf@y
        \advance\pgf@ya by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@ya by -0.5\dp\pgfnodeparttextbox
        \pgf@xb=0.5\pgf@x
        \advance\pgf@xb by 0.5\wd\pgfnodeparttextbox
        \pgf@yb=0.5\pgf@y
        \advance\pgf@yb by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@yb by -0.5\dp\pgfnodeparttextbox
        %compute anchor
        \pgf@y=0.5\pgf@yb
        \advance\pgf@y by 0.5\pgf@ya
        \pgf@x=\pgf@xb
        \ifx\connectors\horizontal
            \pgfkeysgetvalue{/pgf/right connector length}{\lconnector}
            \advance\pgf@x by \lconnector
        \fi
    }

    \savedanchor\connectorwest{
        \pgfkeysgetvalue{/pgf/connectors}{\connectors}
        %compute width and height without taking into account outer sep
        \pgf@x=\wd\pgfnodeparttextbox
        \pgf@xc=\pgfkeysvalueof{/pgf/inner xsep}
        \advance\pgf@x by 2\pgf@xc
        \pgf@xc=\pgfkeysvalueof{/pgf/minimum width}
        \ifdim\pgf@xc>\pgf@x
            \pgf@x=\pgf@xc
        \fi
        \pgf@y=\ht\pgfnodeparttextbox
        \advance\pgf@y by \dp\pgfnodeparttextbox
        \pgf@yc=\pgfkeysvalueof{/pgf/inner ysep}
        \advance\pgf@y by 2\pgf@yc
        \pgf@yc=\pgfkeysvalueof{/pgf/minimum height}
        \ifdim\pgf@yc>\pgf@y
            \pgf@y=\pgf@yc
        \fi
        %store south west in xa,ya and north east in xb,yb
        \pgf@xa=-0.5\pgf@x
        \advance\pgf@xa by 0.5\wd\pgfnodeparttextbox
        \pgf@ya=-0.5\pgf@y
        \advance\pgf@ya by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@ya by -0.5\dp\pgfnodeparttextbox
        \pgf@xb=0.5\pgf@x
        \advance\pgf@xb by 0.5\wd\pgfnodeparttextbox
        \pgf@yb=0.5\pgf@y
        \advance\pgf@yb by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@yb by -0.5\dp\pgfnodeparttextbox
        %compute anchor
        \pgf@y=0.5\pgf@yb
        \advance\pgf@y by 0.5\pgf@ya
        \pgf@x=\pgf@xa
        \ifx\connectors\horizontal
            \pgfkeysgetvalue{/pgf/left connector length}{\lconnector}
            \advance\pgf@x by -\lconnector
        \fi
    }

    \savedanchor\connectornorth{
        \pgfkeysgetvalue{/pgf/connectors}{\connectors}
        %compute width and height without taking into account outer sep
        \pgf@x=\wd\pgfnodeparttextbox
        \pgf@xc=\pgfkeysvalueof{/pgf/inner xsep}
        \advance\pgf@x by 2\pgf@xc
        \pgf@xc=\pgfkeysvalueof{/pgf/minimum width}
        \ifdim\pgf@xc>\pgf@x
            \pgf@x=\pgf@xc
        \fi
        \pgf@y=\ht\pgfnodeparttextbox
        \advance\pgf@y by \dp\pgfnodeparttextbox
        \pgf@yc=\pgfkeysvalueof{/pgf/inner ysep}
        \advance\pgf@y by 2\pgf@yc
        \pgf@yc=\pgfkeysvalueof{/pgf/minimum height}
        \ifdim\pgf@yc>\pgf@y
            \pgf@y=\pgf@yc
        \fi
        %store south west in xa,ya and north east in xb,yb
        \pgf@xa=-0.5\pgf@x
        \advance\pgf@xa by 0.5\wd\pgfnodeparttextbox
        \pgf@ya=-0.5\pgf@y
        \advance\pgf@ya by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@ya by -0.5\dp\pgfnodeparttextbox
        \pgf@xb=0.5\pgf@x
        \advance\pgf@xb by 0.5\wd\pgfnodeparttextbox
        \pgf@yb=0.5\pgf@y
        \advance\pgf@yb by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@yb by -0.5\dp\pgfnodeparttextbox
        %compute anchor
        \pgf@x=0.5\pgf@xb
        \advance\pgf@x by 0.5\pgf@xa
        \pgf@y=\pgf@yb
        \ifx\connectors\vertical
            \pgfkeysgetvalue{/pgf/left connector length}{\lconnector}
            \advance\pgf@y by \lconnector
        \fi
    }

    \savedanchor\connectorsouth{
        \pgfkeysgetvalue{/pgf/connectors}{\lconnectors}
        %compute width and height without taking into account outer sep
        \pgf@x=\wd\pgfnodeparttextbox
        \pgf@xc=\pgfkeysvalueof{/pgf/inner xsep}
        \advance\pgf@x by 2\pgf@xc
        \pgf@xc=\pgfkeysvalueof{/pgf/minimum width}
        \ifdim\pgf@xc>\pgf@x
            \pgf@x=\pgf@xc
        \fi
        \pgf@y=\ht\pgfnodeparttextbox
        \advance\pgf@y by \dp\pgfnodeparttextbox
        \pgf@yc=\pgfkeysvalueof{/pgf/inner ysep}
        \advance\pgf@y by 2\pgf@yc
        \pgf@yc=\pgfkeysvalueof{/pgf/minimum height}
        \ifdim\pgf@yc>\pgf@y
            \pgf@y=\pgf@yc
        \fi
        %store south west in xa,ya and north east in xb,yb
        \pgf@xa=-0.5\pgf@x
        \advance\pgf@xa by 0.5\wd\pgfnodeparttextbox
        \pgf@ya=-0.5\pgf@y
        \advance\pgf@ya by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@ya by -0.5\dp\pgfnodeparttextbox
        \pgf@xb=0.5\pgf@x
        \advance\pgf@xb by 0.5\wd\pgfnodeparttextbox
        \pgf@yb=0.5\pgf@y
        \advance\pgf@yb by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@yb by -0.5\dp\pgfnodeparttextbox
        %compute anchor
        \pgf@x=0.5\pgf@xb
        \advance\pgf@x by 0.5\pgf@xa
        \pgf@y=\pgf@ya
        \ifx\connectors\vertical
            \pgfkeysgetvalue{/pgf/right connector length}{\lconnector}
            \advance\pgf@y by -\lconnector
        \fi
    }

    \anchor{west}{\connectorwest}
    \anchor{east}{\connectoreast}
    \anchor{north}{\connectornorth}
    \anchor{south}{\connectorsouth}

    \backgroundpath{
        \pgfpathcircle{\centerpoint}{\radius}
        \pgfkeysgetvalue{/pgf/connectors}{\connectors}
        \ifx\connectors\horizontal
            \pgfkeysgetvalue{/pgf/left connector length}{\lconnector}
            \pgfkeysgetvalue{/pgf/right connector length}{\rconnector}
            \pgf@process{\centerpoint}
            \pgf@xc=\pgf@x
            \pgf@yc=\pgf@y
            \pgf@xb = \radius
            \advance\pgf@xc by \pgf@xb
            \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@xc by \rconnector
            \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@xc by -\rconnector
            \advance\pgf@xc by -2\pgf@xb
            \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@xc by -\lconnector
            \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
        \fi
        \ifx\connectors\vertical
            \pgfkeysgetvalue{/pgf/left connector length}{\lconnector}
            \pgfkeysgetvalue{/pgf/right connector length}{\rconnector}
            \pgf@process{\centerpoint}
            \pgf@xc=\pgf@x
            \pgf@yc=\pgf@y
            \pgf@xb = \radius
            \advance\pgf@yc by \pgf@xb
            \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@yc by \lconnector
            \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@yc by -\lconnector
            \advance\pgf@yc by -2\pgf@xb
            \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@yc by -\rconnector
            \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
        \fi
    }

    \foregroundpath{
        \pgf@xa = \radius
        \advance\pgf@xa by -0.2\pgf@xa
        \pgftext{\fontsize{\pgf@xa}{\pgf@xa}\selectfont\sffamily\textcolor{\tikz@strokecolor}{OR}}
    }
}
\pgfdeclareshape{and}{

    \inheritsavedanchors[from=circle]
    \inheritanchorborder[from=circle]
    \foreach \a in {center, south east, south west, north east, north west}
    {
        \inheritanchor[from=circle]{\a}
    }

    \savedanchor\connectoreast{
        \pgfkeysgetvalue{/pgf/connectors}{\connectors}
        %compute width and height without taking into account outer sep
        \pgf@x=\wd\pgfnodeparttextbox
        \pgf@xc=\pgfkeysvalueof{/pgf/inner xsep}
        \advance\pgf@x by 2\pgf@xc
        \pgf@xc=\pgfkeysvalueof{/pgf/minimum width}
        \ifdim\pgf@xc>\pgf@x
            \pgf@x=\pgf@xc
        \fi
        \pgf@y=\ht\pgfnodeparttextbox
        \advance\pgf@y by \dp\pgfnodeparttextbox
        \pgf@yc=\pgfkeysvalueof{/pgf/inner ysep}
        \advance\pgf@y by 2\pgf@yc
        \pgf@yc=\pgfkeysvalueof{/pgf/minimum height}
        \ifdim\pgf@yc>\pgf@y
            \pgf@y=\pgf@yc
        \fi
        %store south west in xa,ya and north east in xb,yb
        \pgf@xa=-0.5\pgf@x
        \advance\pgf@xa by 0.5\wd\pgfnodeparttextbox
        \pgf@ya=-0.5\pgf@y
        \advance\pgf@ya by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@ya by -0.5\dp\pgfnodeparttextbox
        \pgf@xb=0.5\pgf@x
        \advance\pgf@xb by 0.5\wd\pgfnodeparttextbox
        \pgf@yb=0.5\pgf@y
        \advance\pgf@yb by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@yb by -0.5\dp\pgfnodeparttextbox
        %compute anchor
        \pgf@y=0.5\pgf@yb
        \advance\pgf@y by 0.5\pgf@ya
        \pgf@x=\pgf@xb
        \ifx\connectors\horizontal
            \pgfkeysgetvalue{/pgf/right connector length}{\lconnector}
            \advance\pgf@x by \lconnector
        \fi
    }

    \savedanchor\connectorwest{
        \pgfkeysgetvalue{/pgf/connectors}{\connectors}
        %compute width and height without taking into account outer sep
        \pgf@x=\wd\pgfnodeparttextbox
        \pgf@xc=\pgfkeysvalueof{/pgf/inner xsep}
        \advance\pgf@x by 2\pgf@xc
        \pgf@xc=\pgfkeysvalueof{/pgf/minimum width}
        \ifdim\pgf@xc>\pgf@x
            \pgf@x=\pgf@xc
        \fi
        \pgf@y=\ht\pgfnodeparttextbox
        \advance\pgf@y by \dp\pgfnodeparttextbox
        \pgf@yc=\pgfkeysvalueof{/pgf/inner ysep}
        \advance\pgf@y by 2\pgf@yc
        \pgf@yc=\pgfkeysvalueof{/pgf/minimum height}
        \ifdim\pgf@yc>\pgf@y
            \pgf@y=\pgf@yc
        \fi
        %store south west in xa,ya and north east in xb,yb
        \pgf@xa=-0.5\pgf@x
        \advance\pgf@xa by 0.5\wd\pgfnodeparttextbox
        \pgf@ya=-0.5\pgf@y
        \advance\pgf@ya by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@ya by -0.5\dp\pgfnodeparttextbox
        \pgf@xb=0.5\pgf@x
        \advance\pgf@xb by 0.5\wd\pgfnodeparttextbox
        \pgf@yb=0.5\pgf@y
        \advance\pgf@yb by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@yb by -0.5\dp\pgfnodeparttextbox
        %compute anchor
        \pgf@y=0.5\pgf@yb
        \advance\pgf@y by 0.5\pgf@ya
        \pgf@x=\pgf@xa
        \ifx\connectors\horizontal
            \pgfkeysgetvalue{/pgf/left connector length}{\lconnector}
            \advance\pgf@x by -\lconnector
        \fi
    }

    \savedanchor\connectornorth{
        \pgfkeysgetvalue{/pgf/connectors}{\connectors}
        %compute width and height without taking into account outer sep
        \pgf@x=\wd\pgfnodeparttextbox
        \pgf@xc=\pgfkeysvalueof{/pgf/inner xsep}
        \advance\pgf@x by 2\pgf@xc
        \pgf@xc=\pgfkeysvalueof{/pgf/minimum width}
        \ifdim\pgf@xc>\pgf@x
            \pgf@x=\pgf@xc
        \fi
        \pgf@y=\ht\pgfnodeparttextbox
        \advance\pgf@y by \dp\pgfnodeparttextbox
        \pgf@yc=\pgfkeysvalueof{/pgf/inner ysep}
        \advance\pgf@y by 2\pgf@yc
        \pgf@yc=\pgfkeysvalueof{/pgf/minimum height}
        \ifdim\pgf@yc>\pgf@y
            \pgf@y=\pgf@yc
        \fi
        %store south west in xa,ya and north east in xb,yb
        \pgf@xa=-0.5\pgf@x
        \advance\pgf@xa by 0.5\wd\pgfnodeparttextbox
        \pgf@ya=-0.5\pgf@y
        \advance\pgf@ya by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@ya by -0.5\dp\pgfnodeparttextbox
        \pgf@xb=0.5\pgf@x
        \advance\pgf@xb by 0.5\wd\pgfnodeparttextbox
        \pgf@yb=0.5\pgf@y
        \advance\pgf@yb by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@yb by -0.5\dp\pgfnodeparttextbox
        %compute anchor
        \pgf@x=0.5\pgf@xb
        \advance\pgf@x by 0.5\pgf@xa
        \pgf@y=\pgf@yb
        \ifx\connectors\vertical
            \pgfkeysgetvalue{/pgf/left connector length}{\lconnector}
            \advance\pgf@y by \lconnector
        \fi
    }

    \savedanchor\connectorsouth{
        \pgfkeysgetvalue{/pgf/connectors}{\lconnectors}
        %compute width and height without taking into account outer sep
        \pgf@x=\wd\pgfnodeparttextbox
        \pgf@xc=\pgfkeysvalueof{/pgf/inner xsep}
        \advance\pgf@x by 2\pgf@xc
        \pgf@xc=\pgfkeysvalueof{/pgf/minimum width}
        \ifdim\pgf@xc>\pgf@x
            \pgf@x=\pgf@xc
        \fi
        \pgf@y=\ht\pgfnodeparttextbox
        \advance\pgf@y by \dp\pgfnodeparttextbox
        \pgf@yc=\pgfkeysvalueof{/pgf/inner ysep}
        \advance\pgf@y by 2\pgf@yc
        \pgf@yc=\pgfkeysvalueof{/pgf/minimum height}
        \ifdim\pgf@yc>\pgf@y
            \pgf@y=\pgf@yc
        \fi
        %store south west in xa,ya and north east in xb,yb
        \pgf@xa=-0.5\pgf@x
        \advance\pgf@xa by 0.5\wd\pgfnodeparttextbox
        \pgf@ya=-0.5\pgf@y
        \advance\pgf@ya by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@ya by -0.5\dp\pgfnodeparttextbox
        \pgf@xb=0.5\pgf@x
        \advance\pgf@xb by 0.5\wd\pgfnodeparttextbox
        \pgf@yb=0.5\pgf@y
        \advance\pgf@yb by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@yb by -0.5\dp\pgfnodeparttextbox
        %compute anchor
        \pgf@x=0.5\pgf@xb
        \advance\pgf@x by 0.5\pgf@xa
        \pgf@y=\pgf@ya
        \ifx\connectors\vertical
            \pgfkeysgetvalue{/pgf/right connector length}{\lconnector}
            \advance\pgf@y by -\lconnector
        \fi
    }

    \anchor{west}{\connectorwest}
    \anchor{east}{\connectoreast}
    \anchor{north}{\connectornorth}
    \anchor{south}{\connectorsouth}

    \backgroundpath{
        \pgfpathcircle{\centerpoint}{\radius}
        \pgfkeysgetvalue{/pgf/connectors}{\connectors}
        \ifx\connectors\horizontal
            \pgfkeysgetvalue{/pgf/left connector length}{\lconnector}
            \pgfkeysgetvalue{/pgf/right connector length}{\rconnector}
            \pgf@process{\centerpoint}
            \pgf@xc=\pgf@x
            \pgf@yc=\pgf@y
            \pgf@xb = \radius
            \advance\pgf@xc by \pgf@xb
            \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@xc by \rconnector
            \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@xc by -\rconnector
            \advance\pgf@xc by -2\pgf@xb
            \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@xc by -\lconnector
            \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
        \fi
        \ifx\connectors\vertical
            \pgfkeysgetvalue{/pgf/left connector length}{\lconnector}
            \pgfkeysgetvalue{/pgf/right connector length}{\rconnector}
            \pgf@process{\centerpoint}
            \pgf@xc=\pgf@x
            \pgf@yc=\pgf@y
            \pgf@xb = \radius
            \advance\pgf@yc by \pgf@xb
            \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@yc by \lconnector
            \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@yc by -\lconnector
            \advance\pgf@yc by -2\pgf@xb
            \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@yc by -\rconnector
            \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
        \fi
    }

    \foregroundpath{
        \pgf@xa = \radius
        \advance\pgf@xa by -0.2\pgf@xa
        \pgftext{\fontsize{\pgf@xa}{\pgf@xa}\selectfont\sffamily\textcolor{\tikz@strokecolor}{AND}}
    }
}
\pgfdeclareshape{equivalence}{

    \inheritsavedanchors[from=circle]
    \inheritanchorborder[from=circle]
    \foreach \a in {center, south east, south west, north east, north west}
    {
        \inheritanchor[from=circle]{\a}
    }

    \savedanchor\connectoreast{
        \pgfkeysgetvalue{/pgf/connectors}{\connectors}
        %compute width and height without taking into account outer sep
        \pgf@x=\wd\pgfnodeparttextbox
        \pgf@xc=\pgfkeysvalueof{/pgf/inner xsep}
        \advance\pgf@x by 2\pgf@xc
        \pgf@xc=\pgfkeysvalueof{/pgf/minimum width}
        \ifdim\pgf@xc>\pgf@x
            \pgf@x=\pgf@xc
        \fi
        \pgf@y=\ht\pgfnodeparttextbox
        \advance\pgf@y by \dp\pgfnodeparttextbox
        \pgf@yc=\pgfkeysvalueof{/pgf/inner ysep}
        \advance\pgf@y by 2\pgf@yc
        \pgf@yc=\pgfkeysvalueof{/pgf/minimum height}
        \ifdim\pgf@yc>\pgf@y
            \pgf@y=\pgf@yc
        \fi
        %store south west in xa,ya and north east in xb,yb
        \pgf@xa=-0.5\pgf@x
        \advance\pgf@xa by 0.5\wd\pgfnodeparttextbox
        \pgf@ya=-0.5\pgf@y
        \advance\pgf@ya by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@ya by -0.5\dp\pgfnodeparttextbox
        \pgf@xb=0.5\pgf@x
        \advance\pgf@xb by 0.5\wd\pgfnodeparttextbox
        \pgf@yb=0.5\pgf@y
        \advance\pgf@yb by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@yb by -0.5\dp\pgfnodeparttextbox
        %compute anchor
        \pgf@y=0.5\pgf@yb
        \advance\pgf@y by 0.5\pgf@ya
        \pgf@x=\pgf@xb
        \ifx\connectors\horizontal
            \pgfkeysgetvalue{/pgf/right connector length}{\lconnector}
            \advance\pgf@x by \lconnector
        \fi
    }

    \savedanchor\connectorwest{
        \pgfkeysgetvalue{/pgf/connectors}{\connectors}
        %compute width and height without taking into account outer sep
        \pgf@x=\wd\pgfnodeparttextbox
        \pgf@xc=\pgfkeysvalueof{/pgf/inner xsep}
        \advance\pgf@x by 2\pgf@xc
        \pgf@xc=\pgfkeysvalueof{/pgf/minimum width}
        \ifdim\pgf@xc>\pgf@x
            \pgf@x=\pgf@xc
        \fi
        \pgf@y=\ht\pgfnodeparttextbox
        \advance\pgf@y by \dp\pgfnodeparttextbox
        \pgf@yc=\pgfkeysvalueof{/pgf/inner ysep}
        \advance\pgf@y by 2\pgf@yc
        \pgf@yc=\pgfkeysvalueof{/pgf/minimum height}
        \ifdim\pgf@yc>\pgf@y
            \pgf@y=\pgf@yc
        \fi
        %store south west in xa,ya and north east in xb,yb
        \pgf@xa=-0.5\pgf@x
        \advance\pgf@xa by 0.5\wd\pgfnodeparttextbox
        \pgf@ya=-0.5\pgf@y
        \advance\pgf@ya by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@ya by -0.5\dp\pgfnodeparttextbox
        \pgf@xb=0.5\pgf@x
        \advance\pgf@xb by 0.5\wd\pgfnodeparttextbox
        \pgf@yb=0.5\pgf@y
        \advance\pgf@yb by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@yb by -0.5\dp\pgfnodeparttextbox
        %compute anchor
        \pgf@y=0.5\pgf@yb
        \advance\pgf@y by 0.5\pgf@ya
        \pgf@x=\pgf@xa
        \ifx\connectors\horizontal
            \pgfkeysgetvalue{/pgf/left connector length}{\lconnector}
            \advance\pgf@x by -\lconnector
        \fi
    }

    \savedanchor\connectornorth{
        \pgfkeysgetvalue{/pgf/connectors}{\connectors}
        %compute width and height without taking into account outer sep
        \pgf@x=\wd\pgfnodeparttextbox
        \pgf@xc=\pgfkeysvalueof{/pgf/inner xsep}
        \advance\pgf@x by 2\pgf@xc
        \pgf@xc=\pgfkeysvalueof{/pgf/minimum width}
        \ifdim\pgf@xc>\pgf@x
            \pgf@x=\pgf@xc
        \fi
        \pgf@y=\ht\pgfnodeparttextbox
        \advance\pgf@y by \dp\pgfnodeparttextbox
        \pgf@yc=\pgfkeysvalueof{/pgf/inner ysep}
        \advance\pgf@y by 2\pgf@yc
        \pgf@yc=\pgfkeysvalueof{/pgf/minimum height}
        \ifdim\pgf@yc>\pgf@y
            \pgf@y=\pgf@yc
        \fi
        %store south west in xa,ya and north east in xb,yb
        \pgf@xa=-0.5\pgf@x
        \advance\pgf@xa by 0.5\wd\pgfnodeparttextbox
        \pgf@ya=-0.5\pgf@y
        \advance\pgf@ya by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@ya by -0.5\dp\pgfnodeparttextbox
        \pgf@xb=0.5\pgf@x
        \advance\pgf@xb by 0.5\wd\pgfnodeparttextbox
        \pgf@yb=0.5\pgf@y
        \advance\pgf@yb by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@yb by -0.5\dp\pgfnodeparttextbox
        %compute anchor
        \pgf@x=0.5\pgf@xb
        \advance\pgf@x by 0.5\pgf@xa
        \pgf@y=\pgf@yb
        \ifx\connectors\vertical
            \pgfkeysgetvalue{/pgf/left connector length}{\lconnector}
            \advance\pgf@y by \lconnector
        \fi
    }

    \savedanchor\connectorsouth{
        \pgfkeysgetvalue{/pgf/connectors}{\lconnectors}
        %compute width and height without taking into account outer sep
        \pgf@x=\wd\pgfnodeparttextbox
        \pgf@xc=\pgfkeysvalueof{/pgf/inner xsep}
        \advance\pgf@x by 2\pgf@xc
        \pgf@xc=\pgfkeysvalueof{/pgf/minimum width}
        \ifdim\pgf@xc>\pgf@x
            \pgf@x=\pgf@xc
        \fi
        \pgf@y=\ht\pgfnodeparttextbox
        \advance\pgf@y by \dp\pgfnodeparttextbox
        \pgf@yc=\pgfkeysvalueof{/pgf/inner ysep}
        \advance\pgf@y by 2\pgf@yc
        \pgf@yc=\pgfkeysvalueof{/pgf/minimum height}
        \ifdim\pgf@yc>\pgf@y
            \pgf@y=\pgf@yc
        \fi
        %store south west in xa,ya and north east in xb,yb
        \pgf@xa=-0.5\pgf@x
        \advance\pgf@xa by 0.5\wd\pgfnodeparttextbox
        \pgf@ya=-0.5\pgf@y
        \advance\pgf@ya by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@ya by -0.5\dp\pgfnodeparttextbox
        \pgf@xb=0.5\pgf@x
        \advance\pgf@xb by 0.5\wd\pgfnodeparttextbox
        \pgf@yb=0.5\pgf@y
        \advance\pgf@yb by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@yb by -0.5\dp\pgfnodeparttextbox
        %compute anchor
        \pgf@x=0.5\pgf@xb
        \advance\pgf@x by 0.5\pgf@xa
        \pgf@y=\pgf@ya
        \ifx\connectors\vertical
            \pgfkeysgetvalue{/pgf/right connector length}{\lconnector}
            \advance\pgf@y by -\lconnector
        \fi
    }

    \anchor{west}{\connectorwest}
    \anchor{east}{\connectoreast}
    \anchor{north}{\connectornorth}
    \anchor{south}{\connectorsouth}

    \backgroundpath{
        \pgfpathcircle{\centerpoint}{\radius}
        \pgfkeysgetvalue{/pgf/connectors}{\connectors}
        \ifx\connectors\horizontal
            \pgfkeysgetvalue{/pgf/left connector length}{\lconnector}
            \pgfkeysgetvalue{/pgf/right connector length}{\rconnector}
            \pgf@process{\centerpoint}
            \pgf@xc=\pgf@x
            \pgf@yc=\pgf@y
            \pgf@xb = \radius
            \advance\pgf@xc by \pgf@xb
            \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@xc by \rconnector
            \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@xc by -\rconnector
            \advance\pgf@xc by -2\pgf@xb
            \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@xc by -\lconnector
            \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
        \fi
        \ifx\connectors\vertical
            \pgfkeysgetvalue{/pgf/left connector length}{\lconnector}
            \pgfkeysgetvalue{/pgf/right connector length}{\rconnector}
            \pgf@process{\centerpoint}
            \pgf@xc=\pgf@x
            \pgf@yc=\pgf@y
            \pgf@xb = \radius
            \advance\pgf@yc by \pgf@xb
            \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@yc by \lconnector
            \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@yc by -\lconnector
            \advance\pgf@yc by -2\pgf@xb
            \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@yc by -\rconnector
            \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
        \fi
    }

    \foregroundpath{
        \pgf@xa = \radius
        \advance\pgf@xa by 0.4\pgf@xa
        \pgftext{\fontsize{\pgf@xa}{\pgf@xa}\selectfont\sffamily\textcolor{\tikz@strokecolor}{$\Xi$}}
    }
}
\pgfdeclareshape{omittedprocess}{
    % \savedmacro\lanchor{0.75}
    \inheritsavedanchors[from=rectangle]
    \inheritanchorborder[from=rectangle]
    \foreach \a in {center, south east, south west, north east, north west}
    {
        \inheritanchor[from=rectangle]{\a}
    }

    \savedanchor\connectoreast{
        \pgfkeysgetvalue{/pgf/connectors}{\connectors}
        %compute width and height without taking into account outer sep
        \pgf@x=\wd\pgfnodeparttextbox
        \pgf@xc=\pgfkeysvalueof{/pgf/inner xsep}
        \advance\pgf@x by 2\pgf@xc
        \pgf@xc=\pgfkeysvalueof{/pgf/minimum width}
        \ifdim\pgf@xc>\pgf@x
            \pgf@x=\pgf@xc
        \fi
        \pgf@y=\ht\pgfnodeparttextbox
        \advance\pgf@y by \dp\pgfnodeparttextbox
        \pgf@yc=\pgfkeysvalueof{/pgf/inner ysep}
        \advance\pgf@y by 2\pgf@yc
        \pgf@yc=\pgfkeysvalueof{/pgf/minimum height}
        \ifdim\pgf@yc>\pgf@y
            \pgf@y=\pgf@yc
        \fi
        %store south west in xa,ya and north east in xb,yb
        \pgf@xa=-0.5\pgf@x
        \advance\pgf@xa by 0.5\wd\pgfnodeparttextbox
        \pgf@ya=-0.5\pgf@y
        \advance\pgf@ya by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@ya by -0.5\dp\pgfnodeparttextbox
        \pgf@xb=0.5\pgf@x
        \advance\pgf@xb by 0.5\wd\pgfnodeparttextbox
        \pgf@yb=0.5\pgf@y
        \advance\pgf@yb by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@yb by -0.5\dp\pgfnodeparttextbox
        %compute anchor
        \pgf@y=0.5\pgf@yb
        \advance\pgf@y by 0.5\pgf@ya
        \pgf@x=\pgf@xb
        \ifx\connectors\horizontal
            \pgfkeysgetvalue{/pgf/right connector length}{\lconnector}
            \advance\pgf@x by \lconnector
        \fi
    }

    \savedanchor\connectorwest{
        \pgfkeysgetvalue{/pgf/connectors}{\connectors}
        %compute width and height without taking into account outer sep
        \pgf@x=\wd\pgfnodeparttextbox
        \pgf@xc=\pgfkeysvalueof{/pgf/inner xsep}
        \advance\pgf@x by 2\pgf@xc
        \pgf@xc=\pgfkeysvalueof{/pgf/minimum width}
        \ifdim\pgf@xc>\pgf@x
            \pgf@x=\pgf@xc
        \fi
        \pgf@y=\ht\pgfnodeparttextbox
        \advance\pgf@y by \dp\pgfnodeparttextbox
        \pgf@yc=\pgfkeysvalueof{/pgf/inner ysep}
        \advance\pgf@y by 2\pgf@yc
        \pgf@yc=\pgfkeysvalueof{/pgf/minimum height}
        \ifdim\pgf@yc>\pgf@y
            \pgf@y=\pgf@yc
        \fi
        %store south west in xa,ya and north east in xb,yb
        \pgf@xa=-0.5\pgf@x
        \advance\pgf@xa by 0.5\wd\pgfnodeparttextbox
        \pgf@ya=-0.5\pgf@y
        \advance\pgf@ya by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@ya by -0.5\dp\pgfnodeparttextbox
        \pgf@xb=0.5\pgf@x
        \advance\pgf@xb by 0.5\wd\pgfnodeparttextbox
        \pgf@yb=0.5\pgf@y
        \advance\pgf@yb by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@yb by -0.5\dp\pgfnodeparttextbox
        %compute anchor
        \pgf@y=0.5\pgf@yb
        \advance\pgf@y by 0.5\pgf@ya
        \pgf@x=\pgf@xa
        \ifx\connectors\horizontal
            \pgfkeysgetvalue{/pgf/left connector length}{\lconnector}
            \advance\pgf@x by -\lconnector
        \fi
    }

    \savedanchor\connectornorth{
        \pgfkeysgetvalue{/pgf/connectors}{\connectors}
        %compute width and height without taking into account outer sep
        \pgf@x=\wd\pgfnodeparttextbox
        \pgf@xc=\pgfkeysvalueof{/pgf/inner xsep}
        \advance\pgf@x by 2\pgf@xc
        \pgf@xc=\pgfkeysvalueof{/pgf/minimum width}
        \ifdim\pgf@xc>\pgf@x
            \pgf@x=\pgf@xc
        \fi
        \pgf@y=\ht\pgfnodeparttextbox
        \advance\pgf@y by \dp\pgfnodeparttextbox
        \pgf@yc=\pgfkeysvalueof{/pgf/inner ysep}
        \advance\pgf@y by 2\pgf@yc
        \pgf@yc=\pgfkeysvalueof{/pgf/minimum height}
        \ifdim\pgf@yc>\pgf@y
            \pgf@y=\pgf@yc
        \fi
        %store south west in xa,ya and north east in xb,yb
        \pgf@xa=-0.5\pgf@x
        \advance\pgf@xa by 0.5\wd\pgfnodeparttextbox
        \pgf@ya=-0.5\pgf@y
        \advance\pgf@ya by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@ya by -0.5\dp\pgfnodeparttextbox
        \pgf@xb=0.5\pgf@x
        \advance\pgf@xb by 0.5\wd\pgfnodeparttextbox
        \pgf@yb=0.5\pgf@y
        \advance\pgf@yb by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@yb by -0.5\dp\pgfnodeparttextbox
        %compute anchor
        \pgf@x=0.5\pgf@xb
        \advance\pgf@x by 0.5\pgf@xa
        \pgf@y=\pgf@yb
        \ifx\connectors\vertical
            \pgfkeysgetvalue{/pgf/left connector length}{\lconnector}
            \advance\pgf@y by \lconnector
        \fi
    }

    \savedanchor\connectorsouth{
        \pgfkeysgetvalue{/pgf/connectors}{\connectors}
        %compute width and height without taking into account outer sep
        \pgf@x=\wd\pgfnodeparttextbox
        \pgf@xc=\pgfkeysvalueof{/pgf/inner xsep}
        \advance\pgf@x by 2\pgf@xc
        \pgf@xc=\pgfkeysvalueof{/pgf/minimum width}
        \ifdim\pgf@xc>\pgf@x
            \pgf@x=\pgf@xc
        \fi
        \pgf@y=\ht\pgfnodeparttextbox
        \advance\pgf@y by \dp\pgfnodeparttextbox
        \pgf@yc=\pgfkeysvalueof{/pgf/inner ysep}
        \advance\pgf@y by 2\pgf@yc
        \pgf@yc=\pgfkeysvalueof{/pgf/minimum height}
        \ifdim\pgf@yc>\pgf@y
            \pgf@y=\pgf@yc
        \fi
        %store south west in xa,ya and north east in xb,yb
        \pgf@xa=-0.5\pgf@x
        \advance\pgf@xa by 0.5\wd\pgfnodeparttextbox
        \pgf@ya=-0.5\pgf@y
        \advance\pgf@ya by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@ya by -0.5\dp\pgfnodeparttextbox
        \pgf@xb=0.5\pgf@x
        \advance\pgf@xb by 0.5\wd\pgfnodeparttextbox
        \pgf@yb=0.5\pgf@y
        \advance\pgf@yb by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@yb by -0.5\dp\pgfnodeparttextbox
        %compute anchor
        \pgf@x=0.5\pgf@xb
        \advance\pgf@x by 0.5\pgf@xa
        \pgf@y=\pgf@ya
        \ifx\connectors\vertical
            \pgfkeysgetvalue{/pgf/right connector length}{\lconnector}
            \advance\pgf@y by -\lconnector
        \fi
    }

    \anchor{west}{\connectorwest}
    \anchor{east}{\connectoreast}
    \anchor{north}{\connectornorth}
    \anchor{south}{\connectorsouth}

    \backgroundpath{
        \pgfpathrectanglecorners{\southwest}{\northeast}
        \pgfkeysgetvalue{/pgf/connectors}{\connectors}
        \ifx\connectors\horizontal
            \pgfkeysgetvalue{/pgf/left connector length}{\lconnector}
            \pgfkeysgetvalue{/pgf/right connector length}{\rconnector}
            \pgf@process{\southwest}
            \pgf@xa = \pgf@x
            \pgf@ya = \pgf@y
            \pgf@process{\northeast}
            \pgf@xb = \pgf@x
            \pgf@yb = \pgf@y
            \pgf@xc=\pgf@x
            \pgf@yc=\pgf@y
            \advance\pgf@yc by -0.5\pgf@yb
            \advance\pgf@yc by 0.5\pgf@ya
            \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@xc by \rconnector
            \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \pgf@xc=\pgf@xa
            \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@xc by -\lconnector
            \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
        \fi
        \ifx\connectors\vertical
            \pgfkeysgetvalue{/pgf/left connector length}{\lconnector}
            \pgfkeysgetvalue{/pgf/right connector length}{\rconnector}
            \pgf@process{\southwest}
            \pgf@xa = \pgf@x
            \pgf@ya = \pgf@y
            \pgf@process{\northeast}
            \pgf@xb = \pgf@x
            \pgf@yb = \pgf@y
            \pgf@xc=\pgf@x
            \pgf@yc=\pgf@y
            \advance\pgf@xc by -0.5\pgf@xb
            \advance\pgf@xc by 0.5\pgf@xa
            \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@yc by \rconnector
            \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \pgf@yc=\pgf@ya
            \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@yc by -\lconnector
            \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
        \fi
    }

    \foregroundpath{
        \pgf@process{\southwest}
        \pgf@xa = \pgf@x
        \pgf@ya = \pgf@y
        \pgf@process{\northeast}
        \pgf@xb = \pgf@x
        \pgf@yb = \pgf@y
        \advance\pgf@yb by -0.1\pgf@yb
        \advance\pgf@yb by 0.1\pgf@ya
        \advance\pgf@ya by -0.1\pgf@ya
        \advance\pgf@ya by 0.1\pgf@y
        \pgf@xc = \pgf@xa
        \advance\pgf@xc by 0.25\pgf@xb
        \advance\pgf@xc by -0.25\pgf@xa
        \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yb}}
        \advance\pgf@xc by 0.25\pgf@xb
        \advance\pgf@xc by -0.25\pgf@xa
        \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@ya}}
        \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yb}}
        \advance\pgf@xc by 0.25\pgf@xb
        \advance\pgf@xc by -0.25\pgf@xa
        \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@ya}}
    }
}
\pgfdeclareshape{macromolecule}{

    \savedmacro{\scarceratio}{\def\scarceratio{0.15}}

    \savedmacro\computecoordinates{%
        \pgf@yb = \ht\pgfnodeparttextbox
        \advance\pgf@yb by \dp\pgfnodeparttextbox
        \pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/pgf/inner ysep}}
        \advance\pgf@yb by 2\pgf@xa
        \pgf@yc=\pgfkeysvalueof{/pgf/minimum height}
        \ifdim\pgf@yc>\pgf@yb
            \pgf@yb=\pgf@yc
        \fi
        \pgf@xb=\wd\pgfnodeparttextbox
        \pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/pgf/inner xsep}}
        \advance\pgf@xb by 2\pgf@xa
        \pgf@xc=\pgfkeysvalueof{/pgf/minimum width}
        \ifdim\pgf@xc>\pgf@xb
            \pgf@xb=\pgf@xc
        \fi
        \ifdim\pgf@yb>\pgf@xb
            \pgfmathsetlengthmacro\scarceoffset{\scarceratio*\pgf@xb}
        \else
            \pgfmathsetlengthmacro\scarceoffset{\scarceratio*\pgf@yb}
        \fi
        \addtosavedmacro\scarceoffset
        \pgf@xa=-0.5\pgf@xb
        \advance\pgf@xa by 0.5\wd\pgfnodeparttextbox
        \pgf@xc=\pgf@xa %saving for later
        \pgf@ya=0.5\pgf@yb
        \advance\pgf@ya by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@ya by -0.5\dp\pgfnodeparttextbox
        \advance\pgf@ya by -\scarceoffset
        \pgfextract@process\westnorthjoin{\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}
        \addtosavedmacro{\westnorthjoin}
        \advance\pgf@ya by \scarceoffset
        \advance\pgf@xa by \scarceoffset
        \pgfextract@process\northwestjoin{\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}
        \addtosavedmacro{\northwestjoin}
        \advance\pgf@xa by \pgf@xb
        \pgfmathaddtolength{\pgf@xa}{-2*\scarceoffset}
        \pgfextract@process\northeastjoin{\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}
        \addtosavedmacro{\northeastjoin}
        \advance\pgf@ya by -\scarceoffset
        \advance\pgf@xa by \scarceoffset
        \pgfextract@process\eastnorthjoin{\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}
        \addtosavedmacro{\eastnorthjoin}
        \advance\pgf@ya by -\pgf@yb
        \pgfmathaddtolength{\pgf@ya}{2*\scarceoffset}
        \pgfextract@process\eastsouthjoin{\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}
        \addtosavedmacro{\eastsouthjoin}
        \advance\pgf@ya by -\scarceoffset
        \advance\pgf@xa by -\scarceoffset
        \pgfextract@process\southeastjoin{\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}
        \addtosavedmacro{\southeastjoin}
        \pgf@xa=\pgf@xc
        \advance\pgf@xa by \scarceoffset
        \pgfextract@process\southwestjoin{\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}
        \addtosavedmacro{\southwestjoin}
        \advance\pgf@xa by -\scarceoffset
        \advance\pgf@ya by \scarceoffset
        \pgfextract@process\westsouthjoin{\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}
        \addtosavedmacro{\westsouthjoin}
    }

    \savedanchor{\southwest}{
        \westnorthjoin
        \pgf@xc=\pgf@x
        \southwestjoin
        \pgf@x=\pgf@xc
    }

    \savedanchor{\northeast}{
        \eastnorthjoin
        \pgf@xc=\pgf@x
        \northeastjoin
        \pgf@x=\pgf@xc
    }

    \anchor{south west}{
        \southwest
    }

    \anchor{north east}{
        \northeast
    }


    \anchor{south east}{
        \northeast
        \pgf@xc=\pgf@x
        \southwest
        \pgf@x=\pgf@xc
    }

    \anchor{north west}{
        \southwest
        \pgf@xc=\pgf@x
        \northeast
        \pgf@x=\pgf@xc
    }

    \inheritanchorborder[from=rectangle]

    \foreach \a in {center, north, south, west, east}
    {
        \inheritanchor[from=rectangle]{\a}
    }

    \backgroundpath{
        \pgfpathmoveto{\northwestjoin}
        \pgfpathlineto{\northeastjoin}
        \pgfpatharc{90}{0}{\scarceoffset}
        \pgfpathlineto{\eastsouthjoin}
        \pgfpatharc{0}{-90}{\scarceoffset}
        \pgfpathlineto{\southwestjoin}
        \pgfpatharc{-90}{-180}{\scarceoffset}
        \pgfpathlineto{\westnorthjoin}
        \pgfpatharc{-180}{-270}{\scarceoffset}
        \pgfpathclose
    }

    \foregroundpath{
        \pgfkeysgetvalue{/pgf/clone}{\clone}
        \ifx\clone\true
            \def\cloneoffsetratio{0.25}
            \computecoordinates
            \northwestjoin
            \pgf@ya=\pgf@y
            \southwestjoin
            \advance\pgf@ya by -\pgf@y
            \newdimen\cloneoffset
            \cloneoffset=\cloneoffsetratio\pgf@ya
            \pgf@yc=\pgf@y
            \advance\pgf@yc by \cloneoffset
            \westsouthjoin
            \pgf@xc=\pgf@x
            \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \eastnorthjoin
            \pgf@xc=\pgf@x
            \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \pgfpathlineto{\eastsouthjoin}
            \pgfpatharc{0}{-90}{\scarceoffset}
            \pgfpathlineto{\southwestjoin}
            \pgfpatharc{-90}{-180}{\scarceoffset}
            \pgfpathclose
            \pgfsetfillcolor{\tikz@strokecolor}
            \pgfusepath{fill, stroke}
        \fi
    }
}
\pgfdeclareshape{delay}{

    \inheritsavedanchors[from=circle]
    \inheritanchorborder[from=circle]
    \foreach \a in {center, south east, south west, north east, north west}
    {
        \inheritanchor[from=circle]{\a}
    }

    \savedanchor\connectoreast{
        \pgfkeysgetvalue{/pgf/connectors}{\connectors}
        %compute width and height without taking into account outer sep
        \pgf@x=\wd\pgfnodeparttextbox
        \pgf@xc=\pgfkeysvalueof{/pgf/inner xsep}
        \advance\pgf@x by 2\pgf@xc
        \pgf@xc=\pgfkeysvalueof{/pgf/minimum width}
        \ifdim\pgf@xc>\pgf@x
            \pgf@x=\pgf@xc
        \fi
        \pgf@y=\ht\pgfnodeparttextbox
        \advance\pgf@y by \dp\pgfnodeparttextbox
        \pgf@yc=\pgfkeysvalueof{/pgf/inner ysep}
        \advance\pgf@y by 2\pgf@yc
        \pgf@yc=\pgfkeysvalueof{/pgf/minimum height}
        \ifdim\pgf@yc>\pgf@y
            \pgf@y=\pgf@yc
        \fi
        %store south west in xa,ya and north east in xb,yb
        \pgf@xa=-0.5\pgf@x
        \advance\pgf@xa by 0.5\wd\pgfnodeparttextbox
        \pgf@ya=-0.5\pgf@y
        \advance\pgf@ya by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@ya by -0.5\dp\pgfnodeparttextbox
        \pgf@xb=0.5\pgf@x
        \advance\pgf@xb by 0.5\wd\pgfnodeparttextbox
        \pgf@yb=0.5\pgf@y
        \advance\pgf@yb by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@yb by -0.5\dp\pgfnodeparttextbox
        %compute anchor
        \pgf@y=0.5\pgf@yb
        \advance\pgf@y by 0.5\pgf@ya
        \pgf@x=\pgf@xb
        \ifx\connectors\horizontal
            \pgfkeysgetvalue{/pgf/right connector length}{\lconnector}
            \advance\pgf@x by \lconnector
        \fi
    }

    \savedanchor\connectorwest{
        \pgfkeysgetvalue{/pgf/connectors}{\connectors}
        %compute width and height without taking into account outer sep
        \pgf@x=\wd\pgfnodeparttextbox
        \pgf@xc=\pgfkeysvalueof{/pgf/inner xsep}
        \advance\pgf@x by 2\pgf@xc
        \pgf@xc=\pgfkeysvalueof{/pgf/minimum width}
        \ifdim\pgf@xc>\pgf@x
            \pgf@x=\pgf@xc
        \fi
        \pgf@y=\ht\pgfnodeparttextbox
        \advance\pgf@y by \dp\pgfnodeparttextbox
        \pgf@yc=\pgfkeysvalueof{/pgf/inner ysep}
        \advance\pgf@y by 2\pgf@yc
        \pgf@yc=\pgfkeysvalueof{/pgf/minimum height}
        \ifdim\pgf@yc>\pgf@y
            \pgf@y=\pgf@yc
        \fi
        %store south west in xa,ya and north east in xb,yb
        \pgf@xa=-0.5\pgf@x
        \advance\pgf@xa by 0.5\wd\pgfnodeparttextbox
        \pgf@ya=-0.5\pgf@y
        \advance\pgf@ya by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@ya by -0.5\dp\pgfnodeparttextbox
        \pgf@xb=0.5\pgf@x
        \advance\pgf@xb by 0.5\wd\pgfnodeparttextbox
        \pgf@yb=0.5\pgf@y
        \advance\pgf@yb by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@yb by -0.5\dp\pgfnodeparttextbox
        %compute anchor
        \pgf@y=0.5\pgf@yb
        \advance\pgf@y by 0.5\pgf@ya
        \pgf@x=\pgf@xa
        \ifx\connectors\horizontal
            \pgfkeysgetvalue{/pgf/left connector length}{\lconnector}
            \advance\pgf@x by -\lconnector
        \fi
    }

    \savedanchor\connectornorth{
        \pgfkeysgetvalue{/pgf/connectors}{\connectors}
        %compute width and height without taking into account outer sep
        \pgf@x=\wd\pgfnodeparttextbox
        \pgf@xc=\pgfkeysvalueof{/pgf/inner xsep}
        \advance\pgf@x by 2\pgf@xc
        \pgf@xc=\pgfkeysvalueof{/pgf/minimum width}
        \ifdim\pgf@xc>\pgf@x
            \pgf@x=\pgf@xc
        \fi
        \pgf@y=\ht\pgfnodeparttextbox
        \advance\pgf@y by \dp\pgfnodeparttextbox
        \pgf@yc=\pgfkeysvalueof{/pgf/inner ysep}
        \advance\pgf@y by 2\pgf@yc
        \pgf@yc=\pgfkeysvalueof{/pgf/minimum height}
        \ifdim\pgf@yc>\pgf@y
            \pgf@y=\pgf@yc
        \fi
        %store south west in xa,ya and north east in xb,yb
        \pgf@xa=-0.5\pgf@x
        \advance\pgf@xa by 0.5\wd\pgfnodeparttextbox
        \pgf@ya=-0.5\pgf@y
        \advance\pgf@ya by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@ya by -0.5\dp\pgfnodeparttextbox
        \pgf@xb=0.5\pgf@x
        \advance\pgf@xb by 0.5\wd\pgfnodeparttextbox
        \pgf@yb=0.5\pgf@y
        \advance\pgf@yb by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@yb by -0.5\dp\pgfnodeparttextbox
        %compute anchor
        \pgf@x=0.5\pgf@xb
        \advance\pgf@x by 0.5\pgf@xa
        \pgf@y=\pgf@yb
        \ifx\connectors\vertical
            \pgfkeysgetvalue{/pgf/left connector length}{\lconnector}
            \advance\pgf@y by \lconnector
        \fi
    }

    \savedanchor\connectorsouth{
        \pgfkeysgetvalue{/pgf/connectors}{\lconnectors}
        %compute width and height without taking into account outer sep
        \pgf@x=\wd\pgfnodeparttextbox
        \pgf@xc=\pgfkeysvalueof{/pgf/inner xsep}
        \advance\pgf@x by 2\pgf@xc
        \pgf@xc=\pgfkeysvalueof{/pgf/minimum width}
        \ifdim\pgf@xc>\pgf@x
            \pgf@x=\pgf@xc
        \fi
        \pgf@y=\ht\pgfnodeparttextbox
        \advance\pgf@y by \dp\pgfnodeparttextbox
        \pgf@yc=\pgfkeysvalueof{/pgf/inner ysep}
        \advance\pgf@y by 2\pgf@yc
        \pgf@yc=\pgfkeysvalueof{/pgf/minimum height}
        \ifdim\pgf@yc>\pgf@y
            \pgf@y=\pgf@yc
        \fi
        %store south west in xa,ya and north east in xb,yb
        \pgf@xa=-0.5\pgf@x
        \advance\pgf@xa by 0.5\wd\pgfnodeparttextbox
        \pgf@ya=-0.5\pgf@y
        \advance\pgf@ya by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@ya by -0.5\dp\pgfnodeparttextbox
        \pgf@xb=0.5\pgf@x
        \advance\pgf@xb by 0.5\wd\pgfnodeparttextbox
        \pgf@yb=0.5\pgf@y
        \advance\pgf@yb by 0.5\ht\pgfnodeparttextbox
        \advance\pgf@yb by -0.5\dp\pgfnodeparttextbox
        %compute anchor
        \pgf@x=0.5\pgf@xb
        \advance\pgf@x by 0.5\pgf@xa
        \pgf@y=\pgf@ya
        \ifx\connectors\vertical
            \pgfkeysgetvalue{/pgf/right connector length}{\lconnector}
            \advance\pgf@y by -\lconnector
        \fi
    }

    \anchor{west}{\connectorwest}
    \anchor{east}{\connectoreast}
    \anchor{north}{\connectornorth}
    \anchor{south}{\connectorsouth}

    \backgroundpath{
        \pgfpathcircle{\centerpoint}{\radius}
        \pgfkeysgetvalue{/pgf/connectors}{\connectors}
        \ifx\connectors\horizontal
            \pgfkeysgetvalue{/pgf/left connector length}{\lconnector}
            \pgfkeysgetvalue{/pgf/right connector length}{\rconnector}
            \pgf@process{\centerpoint}
            \pgf@xc=\pgf@x
            \pgf@yc=\pgf@y
            \pgf@xb = \radius
            \advance\pgf@xc by \pgf@xb
            \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@xc by \rconnector
            \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@xc by -\rconnector
            \advance\pgf@xc by -2\pgf@xb
            \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@xc by -\lconnector
            \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
        \fi
        \ifx\connectors\vertical
            \pgfkeysgetvalue{/pgf/left connector length}{\lconnector}
            \pgfkeysgetvalue{/pgf/right connector length}{\rconnector}
            \pgf@process{\centerpoint}
            \pgf@xc=\pgf@x
            \pgf@yc=\pgf@y
            \pgf@xb = \radius
            \advance\pgf@yc by \pgf@xb
            \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@yc by \lconnector
            \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@yc by -\lconnector
            \advance\pgf@yc by -2\pgf@xb
            \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc}}
            \advance\pgf@yc by -\rconnector
            \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
        \fi
    }

    \foregroundpath{
        \pgf@xa = \radius
        \advance\pgf@xa by 0.4\pgf@xa
        \pgftext{\fontsize{\pgf@xa}{\pgf@xa}\selectfont\sffamily\textcolor{\tikz@strokecolor}{$\tau$}}
    }
}



